Edge-covering plane-filling curves on grid colorings: a pedestrian approach

We describe families of plane-filling curves on any edge-to-edge tiling of the plane with regular polygons and finitely many classes of edges. It is shown how to partition the minimal number of edge classes from the group G of symmetries of the tiling into refined colorings of the tiling, corresponding to finite subgroups of G. All of these colorings correspond to families of plane-filling curves which we call curve-sets. Our exposition is driven by illustrated examples.

==> figures/33333-motif-col-it1.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=3 -T='A+B,A0A,A-C,B+C,B0B,B-A,C+A,C0C,C-B' -a='A+B+C' -m='A ABACA  B BABCB  C CC' -w=15 -A -L=0.4 -l=,A,B,C -e=0.15 -i=1
%% zrender -d=3 -T='A+B,A0A,A-C,B+C,B0B,B-A,C+A,C0C,C-B' -a='A+B+C' -m='A ABACA  B BABCB  C CC' -w=15 -A -L=0.4 -l=,A,B,C -e=0.15 -i=2
%%
%% zrender -d=3 -a='A+B+C' -m='A A+B-C-A+B  B C-A+B+C-A  C B0C' -w=15 -A -L=0.4 -l=,A,B,C -e=0.15 -i=1
%% zrender -d=3 -a='A+B+C' -m='A A+B-C-A+B  B C-A+B+C-A  C B0C' -w=15 -A -L=0.4 -l=,A,B,C -e=0.15 -i=2
%%
\begin{center}
%
{\includegraphics*[width=25mm, viewport={100 320 495 660}]{33333-motif-col-it1-rotational.pdf}}%
{\includegraphics*[width=39mm, viewport={70 380 525 720}]{33333-motif-col-it1-rotational-it2.pdf}}%
\hspace*{0mm}% layout
{\includegraphics*[width=25mm, viewport={100 320 495 660}]{33333-motif-col-it1-star.pdf}}%
{\includegraphics*[width=39mm, viewport={70 345 525 715}]{33333-motif-col-it1-star-it2.pdf}}%
%
\end{center}
\caption{\label{fig:33333-motif-col-it1}
%
First and second iterates of the CCW tiles of the same shape but
with transitions for different grid colorings.
Note the different sequences of letters.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/33333-motif-col-itx.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=3 -T='A+B,A0A,A-C,B+C,B0B,B-A,C+A,C0C,C-B' -a='A+B+C' -m='A ABACA  B BABCB  C CC' -l=,A,B,C -i=7 -J='*3'
%%
%% zrender -d=3 -a='A+B+C' -m='A A+B-C-A+B  B C-A+B+C-A  C B0C' -l=,A,B,C -i=7 -J='*3'
%% zrender -d=3 -a='A-B-C' -m='A A+B-C-A+B  B C-A+B+C-A  C B0C' -l=,A,B,C -i=7 -J='*3'
%%
\begin{center}
%
\begin{subfigure}[b]{38mm}
{\includegraphics*[width=37mm, viewport={20 247 575 842}]{33333-motif-col-itx-rotational.pdf}}%
\vspace*{1mm}% V
\end{subfigure}%
%
{\includegraphics*[width=50mm, viewport={17 300 570 770}]{33333-motif-col-itx-star.pdf}}%
{\includegraphics*[width=35mm, viewport={80 257 535 815}]{33333-motif-col-itx-star-minus.pdf}}%
%
\end{center}
\caption{\label{fig:33333-motif-col-itx}
%
The CCW tile using the grid coloring in this section (left).
The CCW (middle) and CW (right) tile using
the grid coloring from Section~\ref{sect:col-333333-star}.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-3366-grid-graph.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-333333-3366.txt
%%
%% zrender -a='(3,+A+C)' -d=6 -m='A ACABD-ECABABD+ECD0EBD-ECACACD+EBABA  B BACD0EBD-EBAB  C CACD0ECD+EBAC  D D-EBD0ECD+EBABABD  E ECACACD-EBD0ECD+E ' -T='A+C,A-B,B-A,B++D,C+A,C--D,D0E,D--E,D++E,E--C,E++B' -e=0 -i=0 -@=2 --zoom=5 -L=0.4 -A=0.2,0.1 --no-text -l --colors-pick=1,12 -w=10
%%
%% zrender -a='(3,+A+C)' -d=6 -m='A ACABD-ECABABD+ECD0EBD-ECACACD+EBABA  B BACD0EBD-EBAB  C CACD0ECD+EBAC  D D-EBD0ECD+EBABABD  E ECACACD-EBD0ECD+E ' -T='A+C,A-B,B-A,B++D,C+A,C--D,D0E,D--E,D++E,E--C,E++B' -e=0 -w=1 -i=0 -@=2 --zoom=5 -L=0.4 --no-text -l --colors-pick=1,12 -J='A,6,6;B,3,6;C,6,3;D,3,3;E,3,3;'
%%
%%
\begin{center}
%
\fbox{\includegraphics*[width=64mm, viewport={0 400 595 782}]{333333-3366-grid-graph.pdf}}%
\hspace*{1.5mm}% layout
\fbox{\includegraphics*[width=64mm, viewport={0 400 595 782}]{333333-3366-grid-graph-solid.pdf}}%
%
\end{center}
\caption{\label{fig:333333-3366-grid-graph}
%
Grid-graph of the $(3^6; 3.3.6.6)$-grid (left) and
an area drawing of the same (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-3366-r16-var0-curve-decomp.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -@=1 -a='0A' -l --colors-pick=1,12 -d=6 -m='A ABACACACD+ECABABABD+ECD+EBA  B BABD-EBD-EBD-ECAB  C CACD+ECD+ECD+EBAC  D D+ECD0EBD-EBABABD  E ECACACD+ECD0EBD-E ' -T='A+C,A-B,B-A,B++D,C+A,C--D,D0E,D--E,D++E,E--C,E++B' -e=0.1 -w=15 -L=0.4 -A --arrow-offset=0.1 -i=0 --zoom=0.9
%% zrender -@=1 -a='0A' -l --colors-pick=1,12 -d=6 -m='A ABACACACD+ECABABABD+ECD+EBA  B BABD-EBD-EBD-ECAB  C CACD+ECD+ECD+EBAC  D D+ECD0EBD-EBABABD  E ECACACD+ECD0EBD-E ' -T='A+C,A-B,B-A,B++D,C+A,C--D,D0E,D--E,D++E,E--C,E++B' -e=0 -w=1 -i=3 -J='A,6,6;B,3,6;C,6,3;D,3,3;E,3,3;'
%%
%% zrender -@=1 -a='-B' -l --colors-pick=1,12 -d=6 -m='A ABACACACD+ECABABABD+ECD+EBA  B BABD-EBD-EBD-ECAB  C CACD+ECD+ECD+EBAC  D D+ECD0EBD-EBABABD  E ECACACD+ECD0EBD-E ' -T='A+C,A-B,B-A,B++D,C+A,C--D,D0E,D--E,D++E,E--C,E++B' -e=0.1 -w=15 -L=0.4 -A --arrow-offset=0.1 -i=0
%% zrender -@=1 -a='-B' -l --colors-pick=1,12 -d=6 -m='A ABACACACD+ECABABABD+ECD+EBA  B BABD-EBD-EBD-ECAB  C CACD+ECD+ECD+EBAC  D D+ECD0EBD-EBABABD  E ECACACD+ECD0EBD-E ' -T='A+C,A-B,B-A,B++D,C+A,C--D,D0E,D--E,D++E,E--C,E++B' -e=0 -w=1 -i=3 -J='A,6,6;B,3,6;C,6,3;D,3,3;E,3,3;'
%%
%% zrender -@=1 -a='+C' -l --colors-pick=1,12 -d=6 -m='A ABACACACD+ECABABABD+ECD+EBA  B BABD-EBD-EBD-ECAB  C CACD+ECD+ECD+EBAC  D D+ECD0EBD-EBABABD  E ECACACD+ECD0EBD-E ' -T='A+C,A-B,B-A,B++D,C+A,C--D,D0E,D--E,D++E,E--C,E++B' -e=0.1 -w=15 -L=0.4 -A --arrow-offset=0.1 -i=0
%% zrender -@=1 -a='+C' -l --colors-pick=1,12 -d=6 -m='A ABACACACD+ECABABABD+ECD+EBA  B BABD-EBD-EBD-ECAB  C CACD+ECD+ECD+EBAC  D D+ECD0EBD-EBABABD  E ECACACD+ECD0EBD-E ' -T='A+C,A-B,B-A,B++D,C+A,C--D,D0E,D--E,D++E,E--C,E++B' -e=0 -w=1 -i=3 -J='A,6,6;B,3,6;C,6,3;D,3,3;E,3,3;'
%%
%% zrender -@=1 -a='!D' -l --colors-pick=1,12 -d=6 -m='A ABACACACD+ECABABABD+ECD+EBA  B BABD-EBD-EBD-ECAB  C CACD+ECD+ECD+EBAC  D D+ECD0EBD-EBABABD  E ECACACD+ECD0EBD-E ' -T='A+C,A-B,B-A,B++D,C+A,C--D,D0E,D--E,D++E,E--C,E++B' -e=0.1 -w=15 -L=0.4 -A --arrow-offset=0.1 -i=0
%% zrender -@=1 -a='!D' -l --colors-pick=1,12 -d=6 -m='A ABACACACD+ECABABABD+ECD+EBA  B BABD-EBD-EBD-ECAB  C CACD+ECD+ECD+EBAC  D D+ECD0EBD-EBABABD  E ECACACD+ECD0EBD-E ' -T='A+C,A-B,B-A,B++D,C+A,C--D,D0E,D--E,D++E,E--C,E++B' -e=0 -w=1 -i=3 -J='A,6,6;B,3,6;C,6,3;D,3,3;E,3,3;'
%%
%% zrender -@=1 -a='!E' -l --colors-pick=1,12 -d=6 -m='A ABACACACD+ECABABABD+ECD+EBA  B BABD-EBD-EBD-ECAB  C CACD+ECD+ECD+EBAC  D D+ECD0EBD-EBABABD  E ECACACD+ECD0EBD-E ' -T='A+C,A-B,B-A,B++D,C+A,C--D,D0E,D--E,D++E,E--C,E++B' -e=0.1 -w=15 -L=0.4 -A --arrow-offset=0.1 -i=0
%% zrender -@=1 -a='!E' -l --colors-pick=1,12 -d=6 -m='A ABACACACD+ECABABABD+ECD+EBA  B BABD-EBD-EBD-ECAB  C CACD+ECD+ECD+EBAC  D D+ECD0EBD-EBABABD  E ECACACD+ECD0EBD-E ' -T='A+C,A-B,B-A,B++D,C+A,C--D,D0E,D--E,D++E,E--C,E++B' -e=0 -w=1 -i=3 -J='A,6,6;B,3,6;C,6,3;D,3,3;E,3,3;'
%%
%%
\begin{center}
%
{\includegraphics*[width=31mm, viewport={0 247 595 842}]{333333-3366-r16-var0-curve-decomp-A-lines.pdf}}%
{\includegraphics*[width=31mm, viewport={0 247 595 842}]{333333-3366-r16-var0-curve-decomp-A-solid.pdf}}%
%
\hspace*{1mm}% layout
%
{\includegraphics*[width=31mm, viewport={0 247 595 842}]{333333-3366-r16-var0-curve-decomp-B-lines.pdf}}%
{\includegraphics*[width=31mm, viewport={0 247 595 842}]{333333-3366-r16-var0-curve-decomp-B-solid.pdf}}
%
%
{\includegraphics*[width=31mm, viewport={0 247 595 842}]{333333-3366-r16-var0-curve-decomp-C-lines.pdf}}%
{\includegraphics*[width=31mm, viewport={0 247 595 842}]{333333-3366-r16-var0-curve-decomp-C-solid.pdf}}%
%
\hspace*{1mm}% layout
%
{\includegraphics*[width=31mm, viewport={0 247 595 842}]{333333-3366-r16-var0-curve-decomp-D-lines.pdf}}%
{\includegraphics*[width=31mm, viewport={0 247 595 842}]{333333-3366-r16-var0-curve-decomp-D-solid.pdf}}
%
\hspace*{63mm}% layout
%
{\includegraphics*[width=31mm, viewport={0 290 595 822}]{333333-3366-r16-var0-curve-decomp-E-lines.pdf}}%
{\includegraphics*[width=31mm, viewport={0 290 595 822}]{333333-3366-r16-var0-curve-decomp-E-solid.pdf}}
%
%
\end{center}
\caption{\label{fig:333333-3366-r16-var0-curve-decomp}
Mutual self-similarity of the curves (left to right, top to bottom):
\texttt{A} (small copies blue),
\texttt{B} (small copies red),
\texttt{C} (small copies green),
\texttt{D} (small copies pale pink), and
\texttt{E} (small copies olive).\IMAGENAME%
%\texttt{A},
%\texttt{B},
%\texttt{C},
%\texttt{D}, and
%\texttt{E}.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-3366-r16-var0-tiles-plus.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%% zrender -@=1 -a='(3,A+C+)' -l='AC,BDE' --colors-pick=1,12 -d=6 -m='A ABACACACD+ECABABABD+ECD+EBA  B BABD-EBD-EBD-ECAB  C CACD+ECD+ECD+EBAC  D D+ECD0EBD-EBABABD  E ECACACD+ECD0EBD-E ' -T='A+C,A-B,B-A,B++D,C+A,C--D,D0E,D--E,D++E,E--C,E++B' -e=0 -w=1 -i=2 -J
%% zrender -@=1 -a='-(1,B++D++E)' -l='AC,BDE' --colors-pick=1,12 -d=6 -m='A ABACACACD+ECABABABD+ECD+EBA  B BABD-EBD-EBD-ECAB  C CACD+ECD+ECD+EBAC  D D+ECD0EBD-EBABABD  E ECACACD+ECD0EBD-E ' -T='A+C,A-B,B-A,B++D,C+A,C--D,D0E,D--E,D++E,E--C,E++B' -e=0 -w=1 -i=2 -J
%%
%% zrender -@=1 -a='(3,A+C+)' -l='A,C,B,D,E' --colors-pick=1,12 -d=6 -m='A ABACACACD+ECABABABD+ECD+EBA  B BABD-EBD-EBD-ECAB  C CACD+ECD+ECD+EBAC  D D+ECD0EBD-EBABABD  E ECACACD+ECD0EBD-E ' -T='A+C,A-B,B-A,B++D,C+A,C--D,D0E,D--E,D++E,E--C,E++B' -e=0 -w=1 -i=2 -J
%% zrender -@=1 -a='-(1,B++D++E)' -l='A,C,B,D,E' --colors-pick=1,12 -d=6 -m='A ABACACACD+ECABABABD+ECD+EBA  B BABD-EBD-EBD-ECAB  C CACD+ECD+ECD+EBAC  D D+ECD0EBD-EBABABD  E ECACACD+ECD0EBD-E ' -T='A+C,A-B,B-A,B++D,C+A,C--D,D0E,D--E,D++E,E--C,E++B' -e=0 -w=1 -i=2 -J
%%
%%
\begin{center}
%
{\includegraphics*[width=32mm, viewport={0 270 595 790}]{333333-3366-r16-var0-tiles-plus-AC3.pdf}}%
{\includegraphics*[width=32mm, viewport={0 270 595 790}]{333333-3366-r16-var0-tiles-plus-BDE.pdf}}%
\hspace*{1mm}%
{\includegraphics*[width=32mm, viewport={0 270 595 790}]{333333-3366-r16-var0-tiles-plus-AC3-curves.pdf}}%
{\includegraphics*[width=32mm, viewport={0 270 595 790}]{333333-3366-r16-var0-tiles-plus-BDE-curves.pdf}}%
%
\end{center}
\caption{\label{fig:333333-3366-r16-var0-tiles-plus}
%
Mutual self-similarity of the CCW prototiles
\tileS{A+C+}{3} (left, small copies blue) and \tileS{B++D++E++}{1} (small copies red).
Note that all but one of the prototiles \tileS{B++D++E++}{1} appear in (triangular) clusters of three.
The two images colored by curves (right) may help to see the structure.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-3366-r16-var0-tiling.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -@=1 -a='(3,A+C+)' -l --colors-pick=1,12 -d=6 -m='A ABACACACD+ECABABABD+ECD+EBA  B BABD-EBD-EBD-ECAB  C CACD+ECD+ECD+EBAC  D D+ECD0EBD-EBABABD  E ECACACD+ECD0EBD-E ' -T='A+C,A-B,B-A,B++D,C+A,C--D,D0E,D--E,D++E,E--C,E++B' -e=0 -w=1 -i=2 -J='A,6,6;B,3,6;C,6,3;D,3,3;E,3,3;' -@=2 --zoom=4
%%
%%
\begin{center}
%
\fbox{\includegraphics*[width=100mm, viewport={0 497 595 842}]{333333-3366-r16-var0-tiling.pdf}}%
%
\end{center}
\caption{\label{fig:333333-3366-r16-var0-tiling}
%
Tiling the plane with the curve-set, coloring as in grid.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-3366-trans-r13-15-curve-decomp.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -a='F' -d=3 -m='F F+F0F0F-F-F+F0F+F+F-F0F-F ' -e=0 -w=3 -@=1 -i=3 -k=-1 -J -r=-120
%%
%%% same look, but bigger:
%%% zrender -a='A' -d=6 -m='A ABD+ECABD0ECABD0ECABD-ECABD-ECABD+ECABD0ECABD+ECABD+ECABD-ECABD0ECABD-ECA  B B  C C  D D  E E  ' -T='A+C,A-B,B-A,B++D,C+A,C--D,D0E,D--E,D++E,E--C,E++B' -e=0.1 -w=5 -@=1 -i=3 -k=-1 -A -J --margin=0.01 -r=-120
%%

%%
\begin{center}
%
%\fbox{\includegraphics*[width=64.5mm, viewport={0 247 595 842}]{333333-3366-trans-r13-15-curve-decomp-it4.pdf}}%
%{\includegraphics*[width=84.5mm, viewport={0 332 595 752}]{333333-3366-trans-r13-15-curve-decomp-it4.pdf}}%
{\includegraphics*[width=90mm, viewport={0 342 595 730}]{333333-3366-trans-r13-15-curve-decomp-it4.pdf}}%
%\fbox{\includegraphics*[width=64.5mm, viewport={0 247 595 842}]{333333-3366-trans-r13-15-curve-from-it4.pdf}}%
\hspace*{0mm}% layout
%
%\begin{subfigure}[b]{21mm}
%\fbox{\includegraphics*[width=20mm, viewport={0 247 595 842}]{333333-3366-trans-r13-15-curve-decomp.pdf}}
%\vspace*{12mm}% V
%\end{subfigure}
%
\end{center}
\caption{\label{fig:333333-3366-trans-r13-15-curve-decomp}
%
Self-similarity of the curve for the letter \texttt{A}.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-3366-trans-r13-15-tiles-plus.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -a='(3,A+C+)' -d=6 -m='A ABD+ECABD0ECABD0ECABD-ECABD-ECABD+ECABD0ECABD+ECABD+ECABD-ECABD0ECABD-ECA  B B  C C  D D  E E  ' -T='A+C,A-B,B-A,B++D,C+A,C--D,D0E,D--E,D++E,E--C,E++B' -e=0.1 -w=5 -@=1 -i=0 -k=+6 -A -L=0 -J
%%
%% zrender -a='(3,A+C+)' -d=6 -m='A ABD+ECABD0ECABD0ECABD-ECABD-ECABD+ECABD0ECABD+ECABD+ECABD-ECABD0ECABD-ECA  B B  C C  D D  E E  ' -T='A+C,A-B,B-A,B++D,C+A,C--D,D0E,D--E,D++E,E--C,E++B' -e=0.1 -w=5 -@=1 -i=1 -k=+6 -A -J
%%
%% zrender -a='(3,A+C+)' -d=6 -m='A ABD+ECABD0ECABD0ECABD-ECABD-ECABD+ECABD0ECABD+ECABD+ECABD-ECABD0ECABD-ECA  B B  C C  D D  E E  ' -T='A+C,A-B,B-A,B++D,C+A,C--D,D0E,D--E,D++E,E--C,E++B' -e=0.1 -w=5 -@=1 -i=2 -k=+6 -A -J
%%
%%
\begin{center}
%
%\fbox{\includegraphics*[width=43mm, viewport={0 247 595 842}]{333333-3366-trans-r13-15-tiles-plus-it1.pdf}}%
%\fbox{\includegraphics*[width=43mm, viewport={0 247 595 842}]{333333-3366-trans-r13-15-tiles-plus-it2.pdf}}%
%\fbox{\includegraphics*[width=43mm, viewport={0 247 595 842}]{333333-3366-trans-r13-15-tiles-plus-it3.pdf}}%
%
{\includegraphics*[width=60mm, viewport={0 267 595 802}]{333333-3366-trans-r13-15-tiles-plus-it1.pdf}}%
\hspace*{4mm}%
{\includegraphics*[width=60mm, viewport={0 267 595 802}]{333333-3366-trans-r13-15-tiles-plus-it2.pdf}}%
%
\end{center}
\caption{\label{fig:333333-3366-trans-r13-15-tiles-plus}
%
Area drawings for the first (left) and second (right) iterates
of the tile \tileS{A+C+}{3}.
Coloring by the letters and their orientation in the first iterate.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-3366-trans-r13-15.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -a='~A' -d=6 -m='A ABD+ECABD0ECABD0ECABD-ECABD-ECABD+ECABD0ECABD+ECABD+ECABD-ECABD0ECABD-ECA  B B  C C  D D  E E  ' -T='A+C,A-B,B-A,B++D,C+A,C--D,D0E,D--E,D++E,E--C,E++B' -e=0.15 -w=10 -@=1 -i=0 -t=A -L=0.4 -A
%%
%% zrender -a='~A' -d=6 -m='A ABD+ECABD0ECABD0ECABD-ECABD-ECABD+ECABD0ECABD+ECABD+ECABD-ECABD0ECABD-ECA  B B  C C  D D  E E  ' -T='A+C,A-B,B-A,B++D,C+A,C--D,D0E,D--E,D++E,E--C,E++B' -e=0.2 -w=5 -@=1 -i=1 -t=A -r=-60
%%
%% zrender -a='F' -d=3 -m='F F+F0F0F-F-F+F0F+F+F-F0F-F ' -e=0.15 -w=7 -@=1 -i=1 -k=-1 -r=-60
%%
\begin{center}
%
%{\includegraphics*[width=40mm, viewport={90 247 505 842}]{333333-3366-trans-r13-15-from.pdf}}%
{\includegraphics*[width=40mm, viewport={90 247 505 842}]{333333-3366-trans-r13-15-to.pdf}}%
%
{\includegraphics*[width=42mm, viewport={85 247 505 825}]{333333-3366-trans-r13-15-to-it2.pdf}}%
{\includegraphics*[width=42mm, viewport={85 247 505 825}]{333333-3366-trans-r13-15-from-it2.pdf}}%
%
\end{center}
\caption{\label{fig:333333-3366-trans-r13-15}
%
First (left) and second iterate (middle) of the curve for the letter \texttt{A} (left),
a similarly looking curve on the triangle grid (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-R25-544.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=3 -a='(3,F+)' -m='F F0F+F+F-F-F0F-F0F+F+F-F-F0F-F0F+F+F-F0F0F+F-F+F0F' --id='R25-544' -i=3 -k=+1 -w=3 -J
%% zrender -d=3 -a='(3,F-)' -m='F F0F+F+F-F-F0F-F0F+F+F-F-F0F-F0F+F+F-F0F0F+F-F+F0F' --id='R25-544' -i=3 -k=+1 -w=3 -J
%%
\begin{center}
%
{\includegraphics*[width=60mm, viewport={0 247 595 822}]{333333-R25-544-tile-plus.pdf}}%
\hspace*{3mm}% layout
{\includegraphics*[width=60mm, viewport={0 247 595 822}]{333333-R25-544-tile-minus.pdf}}%
%
\end{center}
\caption{\label{fig:333333-R25-544}
%
Third iterates of the tiles \tileS{F+}{3} (left) and \tileS{F-}{3} (right) of a curve of order 25.
Both have reflection symmetry.
Coloring by orientation of curves.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-bizarro-curve-r9-var0-it.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=3 -T='A+A,A0B,A-C, B+C,B0A,B-B, C+D,C0D,C-D, D+B,D0C,D-A' -m='A A+A-C-D0C+D+B-B0A  B B+C-D-A0B+C+D-A0B  C C+D-A-C0D+B+C-D+B-B-B0A+A+A-C  D D0C0D' --colors-pick=1,4 -l -i=3 -J -B=7,0.7 -a='A[]+A-C-D0C+D+B[]-B0A'
%%
%% zrender -d=3 -T='A+A,A0B,A-C, B+C,B0A,B-B, C+D,C0D,C-D, D+B,D0C,D-A' -m='A A+A-C-D0C+D+B-B0A  B B+C-D-A0B+C+D-A0B  C C+D-A-C0D+B+C-D+B-B-B0A+A+A-C  D D0C0D' --colors-pick=1,4 -l -i=3 -J -B=7,0.7 -a='B+C-D-A0B+C+D-A0B'
%%
%% zrender -d=3 -T='A+A,A0B,A-C, B+C,B0A,B-B, C+D,C0D,C-D, D+B,D0C,D-A' -m='A A+A-C-D0C+D+B-B0A  B B+C-D-A0B+C+D-A0B  C C+D-A-C0D+B+C-D+B-B-B0A+A+A-C  D D0C0D' --colors-pick=1,4 -l -i=3 -J -B=7,0.7 -a='C+D-A-C0D+B+C-D+B[]-B-B0A[]+A[]+A-C'
%%
%% zrender -d=3 -T='A+A,A0B,A-C, B+C,B0A,B-B, C+D,C0D,C-D, D+B,D0C,D-A' -m='A A+A-C-D0C+D+B-B0A  B B+C-D-A0B+C+D-A0B  C C+D-A-C0D+B+C-D+B-B-B0A+A+A-C  D D0C0D' --colors-pick=1,4 -l -i=3 -J -B=7,0.7 -a='D0C0D'
%%
\begin{center}
%
{\includegraphics*[width=30mm, viewport={0 300 595 742}]{333333-bizarro-curve-r9-var0-it-A.pdf}}%
\hspace*{3mm}%
{\includegraphics*[width=30mm, viewport={0 300 595 742}]{333333-bizarro-curve-r9-var0-it-B.pdf}}%
\hspace*{3mm}%
{\includegraphics*[width=30mm, viewport={0 300 595 772}]{333333-bizarro-curve-r9-var0-it-C.pdf}}%
\hspace*{3mm}%
{\includegraphics*[width=30mm, viewport={0 300 595 742}]{333333-bizarro-curve-r9-var0-it-D.pdf}}%
%\hspace*{0mm}% layout
%
%
\end{center}
\caption{\label{fig:333333-bizarro-curve-r9-var0-it}
From left to right:
Third iterates of the curves
\texttt{A} (small copies blue),
\texttt{B} (small copies red),
\texttt{C} (small copies green), and
\texttt{D} (small copies pale pink).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-bizarro-curve-r9-var0-it1.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=3 -T='A+A,A0B,A-C, B+C,B0A,B-B, C+D,C0D,C-D, D+B,D0C,D-A' -m='A A+A-C-D0C+D+B-B0A  B B+C-D-A0B+C+D-A0B  C C+D-A-C0D+B+C-D+B-B-B0A+A+A-C  D D0C0D' --colors-pick=1,4 -l -L -A -w=20 -e=0.12 -@=1 -i=0 --zoom=1.4 -a=A
%%
%%
%%
\begin{center}
%
{\includegraphics*[width=30mm, viewport={0 347 595 742}]{333333-bizarro-curve-r9-var0-it1-A.pdf}}%
\hspace*{3mm}%
{\includegraphics*[width=30mm, viewport={0 347 595 742}]{333333-bizarro-curve-r9-var0-it1-B.pdf}}%
\hspace*{3mm}%
{\includegraphics*[width=30mm, viewport={0 347 595 742}]{333333-bizarro-curve-r9-var0-it1-C.pdf}}%
\hspace*{3mm}%
{\includegraphics*[width=30mm, viewport={0 347 595 742}]{333333-bizarro-curve-r9-var0-it1-D.pdf}}%
%\hspace*{0mm}% layout
%
%
\end{center}
\caption{\label{fig:333333-bizarro-curve-r9-var0-it1}
From left to right:
motifs of the curves
\texttt{A}, \texttt{B}, \texttt{C}, and \texttt{D}.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-bizarro-curve-r9-var0-tiling.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=3 -T='A+A,A0B,A-C, B+C,B0A,B-B, C+D,C0D,C-D, D+B,D0C,D-A' -a='A' -m='A A+A-C-D0C+D+B-B0A  B B+C-D-A0B+C+D-A0B  C C+D-A-C0D+B+C-D+B-B-B0A+A+A-C  D D0C0D' --colors-pick=1,4 -l -@=1 -i=3 -J --grid=3 --no-text --zoom=2 --shift-y=-0.08
%%
%%
%%
\begin{center}
%
\fbox{\includegraphics*[width=100mm, viewport={0 400 595 822}]{333333-bizarro-curve-r9-var0-tiling.pdf}}%
\hspace*{0mm}% layout
%
%
\end{center}
\caption{\label{fig:333333-bizarro-curve-r9-var0-tiling}
Tiling of the plane with our curves.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-bizarro-grid.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=3 -a='A' -T='A+A,A0B,A-C, B+C,B0A,B-B, C+D,C0D,C-D, D+B,D0C,D-A' --const-maps --grid=12 -l=',A,B,C,D' -A=0.25,0.1 -L=0.4 -w=10 --zoom=1.7
%%
%% zrender -d=3 -T='A+A,A0B,A-C, B+C,B0A,B-B, C+D,C0D,C-D, D+B,D0C,D-A' -a='(3,A+)' --const-maps -l=',A,B,C,D' -A=0.2,0.1 -L=0.4 -w=30
%% zrender -d=3 -T='A+A,A0B,A-C, B+C,B0A,B-B, C+D,C0D,C-D, D+B,D0C,D-A' -a='(1,B+C+D+)' --const-maps -l=',A,B,C,D' -A=0.2,0.1 -L=0.4 -w=30
%%
%% zrender -d=3 -T='A+A,A0B,A-C, B+C,B0A,B-B, C+D,C0D,C-D, D+B,D0C,D-A' -a='(3,B-)' --const-maps -l=',A,B,C,D' -A=0.2,0.1 -L=0.4 -w=30
%% zrender -d=3 -T='A+A,A0B,A-C, B+C,B0A,B-B, C+D,C0D,C-D, D+B,D0C,D-A' -a='(1,A-C-D-)' --const-maps -l=',A,B,C,D' -A=0.2,0.1 -L=0.4 -w=30
%%
\begin{center}
%
\fbox{\includegraphics*[width=75mm, viewport={100 490 555 790}]{333333-bizarro-grid.pdf}}%
\hspace*{0mm}% layout
%
\hspace*{7mm}% H
\begin{subfigure}[b]{15mm}
{\includegraphics*[width=15mm, viewport={100 247 490 842}]{333333-bizarro-grid-tilep-A3.pdf}}
{\includegraphics*[width=15mm, viewport={100 247 490 842}]{333333-bizarro-grid-tilep-BCD.pdf}}
%\vspace*{2mm}% V
\end{subfigure}%
%
\hspace*{5mm}% H
\begin{subfigure}[b]{15mm}
{\includegraphics*[width=15mm, viewport={100 247 490 842}]{333333-bizarro-grid-tilem-B3.pdf}}
{\includegraphics*[width=15mm, viewport={100 247 490 842}]{333333-bizarro-grid-tilem-ACD.pdf}}
%\vspace*{2mm}% V
\end{subfigure}%
%
\end{center}
\caption{\label{fig:333333-bizarro-grid}
A coloring of the triangle grid with four colors (left),
its CCW tiles \tileS{A+}{3} and \tileS{B-C-D-}{1} (middle),
and
its CW tiles \tileS{B-}{3} and \tileS{A-C-D-}{1} (right).\IMAGENAME%
%obtained by dropping all edges \texttt{A}
%in the $(3^6;\, 3.3.6.6)$-grid.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-curve-r13-1-solid.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -i=0 -m='F F0F+F0F0F-F+F-F-F0F+F+F-F' -a='F' -@=1 -d=3  -e=0.1 -k=-1 -w=15 --id='R13-1' --arrows=0.15 --zoom=0.9 -J='*3'
%% zrender -i=1 -m='F F0F+F0F0F-F+F-F-F0F+F+F-F' -a='F' -@=1 -d=3  -e=0 -k=-1 -w=2 --id='R13-1'  -r=-46.6 -J='*3' # rot!
%% zrender -i=2 -m='F F0F+F0F0F-F+F-F-F0F+F+F-F' -a='F' -@=1 -d=3  -e=0 -k=-1 -w=2 --id='R13-1'  -r=-93.3 -J='*3' # rot!
%%
\begin{center}
%
\begin{subfigure}[b]{41mm}
{\includegraphics*[width=40mm, viewport={50 237 545 842}]{333333-curve-r13-1-solid-it1.pdf}}
\vspace*{4mm}% V
\end{subfigure}
%
\hspace*{2mm}% layout
{\includegraphics*[width=40mm, viewport={100 247 480 842}]{333333-curve-r13-1-solid-it2.pdf}}
%
\hspace*{2mm}% layout
{\includegraphics*[width=40mm, viewport={100 247 480 842}]{333333-curve-r13-1-solid-it3.pdf}}
%
\end{center}
\caption{\label{fig:333333-curve-r13-1-solid}
First (left), second (middle), and third (right) iterate of a curve,
rendered as area drawings.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-curve-r13-1.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -i=0 -m='F F0F+F0F0F-F+F-F-F0F+F+F-F' -a='F' -@=1 -d=3  -e=0.12 -k=-1 -w=15 --id='R13-1' --letters --arrows=0.15 --zoom=0.9
%% zrender -i=0 -m='F F0F+F0F0F-F+F-F-F0F+F+F-F' -a='F' -@=1 -d=3 -e=0.15 -k=-1 -w=7 --id='R13-1' -A=0.2,0.1 -i=1
%% zrender -i=3 -m='F F0F+F0F0F-F+F-F-F0F+F+F-F' -a='F' -@=1 -d=3  -e=0 -k=-1 -w=2 --id='R13-1' -r=-140 -J='*3' # rot!
%%
\begin{center}
%
\begin{subfigure}[b]{40mm}
{\includegraphics*[width=40mm, viewport={0 247 595 842}]{333333-curve-r13-1-it1.pdf}}
\vspace*{2mm}% V
\end{subfigure}
%
\hspace*{0mm}% layout
\begin{subfigure}[b]{45mm}
{\includegraphics*[width=45mm, viewport={0 247 595 842}]{333333-curve-r13-1-it2.pdf}}
\vspace*{2mm}% V
\end{subfigure}
%
%\hspace*{2mm}% layout
{\includegraphics*[width=35mm, viewport={100 247 480 815}]{333333-curve-r13-1-it4.pdf}}
%
\end{center}
\caption{\label{fig:333333-curve-r13-1}
First iterate (left),
second iterate (middle),
and fourth iterate (right)
of a curve corresponding to the word \texttt{F0F+F0F0F-F+F-F-F0F+F+F-F}.
This curve lives on the triangle grid.
Coloring by edges of the motif.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-rotational-grid-graph.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -T='A0A,B0B,C0C, A+B,B+C,C+A, A-C,B-A,C-B' -d=3 --const-maps -w=11 -a=A -l=',A,B,C' -L -A=0.2,0.1 --grid=10 --zoom=2
%% zrender -T='A0A,B0B,C0C, A+B,B+C,C+A, A-C,B-A,C-B' -d=3 --const-maps -w=30 -a=A+B+C -l=',A,B,C' -L -A=0.15,0.05 --zoom=0.8
%% zrender -T='A0A,B0B,C0C, A+B,B+C,C+A, A-C,B-A,C-B' -d=3 --const-maps -w=30 -a=A-C-B -l=',A,B,C' -L -A=0.15,0.05 --zoom=0.8
%%
%%
\begin{center}
%
\hspace*{0mm}% layout
\fbox{\includegraphics*[width=65mm, viewport={0 417 595 832}]{333333-rotational-grid-graph.pdf}}%
\hspace*{7mm}% layout
\begin{subfigure}[b]{41mm}
{\includegraphics*[width=20mm, viewport={0 247 595 842}]{333333-rotational-grid-graph-tile-ABC.pdf}}%
{\includegraphics*[width=20mm, viewport={0 247 595 842}]{333333-rotational-grid-graph-tile-ACB.pdf}}%
\vspace*{4mm}% V
\end{subfigure}
%
\end{center}
\caption{\label{fig:333333-rotational-grid-graph}
%
A coloring of the triangle grid (left)
and its two prototiles \tileS{A+B+C+}{1} and \tileS{A-C-B-}{1} (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-rotational-keili-it.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=3 -T='A0A,B0B,C0C, A+B,B+C,C+A, A-C,B-A,C-B' -m='A AABA  B BABCB  C CACCBABCC ' -e=0.15 -w=5 -a=A+B+C+ -k=+3 -i=7 -l=',A,B,C' -J -r=-60
%%
\begin{center}
%
{\includegraphics*[width=128mm, viewport={25 520 575 550}]{333333-rotational-keili-it7.pdf}}%
\hspace*{0mm}% layout
%
\end{center}
\caption{\label{fig:333333-rotational-keili-it}
%
Seventh iterate of the CCW prototile.\IMAGENAME%
%The uneven growth becomes obvious.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-rotational-keili.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=3 -T='A0A,B0B,C0C, A+B,B+C,C+A, A-C,B-A,C-B' -m='A AABA  B BABCB  C CACCBABCC ' -e=0.12 -w=15 -a=A+B+C+ -k=+3 -i=1 -l=',A,B,C' -A=0.2,0.1 -L=0.4 --fancy-print-maps
%% zrender -d=3 -T='A0A,B0B,C0C, A+B,B+C,C+A, A-C,B-A,C-B' -m='A AABA  B BABCB  C CACCBABCC ' -e=0.12 -w=10 -a=A+B+C+ -k=+3 -i=2 -l=',A,B,C' -A=0.2,0.1
%% zrender -d=3 -T='A0A,B0B,C0C, A+B,B+C,C+A, A-C,B-A,C-B' -m='A AABA  B BABCB  C CACCBABCC ' -e=0.15 -w=5 -a=A+B+C+ -k=+3 -i=3 -l=',A,B,C'
%%
\begin{center}
%
{\includegraphics*[width=40mm, viewport={0 267 595 822}]{333333-rotational-keili-it1.pdf}}%
{\includegraphics*[width=40mm, viewport={0 267 595 822}]{333333-rotational-keili-it2.pdf}}%
{\includegraphics*[width=40mm, viewport={0 257 595 812}]{333333-rotational-keili-it3.pdf}}%
\hspace*{0mm}% layout
%
%\begin{subfigure}[b]{21mm}
%\fbox{\includegraphics*[width=20mm, viewport={0 247 595 842}]{333333-rotational-keili.pdf}}
%\vspace*{12mm}% V
%\end{subfigure}
%%
%\begin{subfigure}[b]{20mm}
%\fbox{\includegraphics*[width=20mm, viewport={0 247 595 842}]{333333-rotational-keili.pdf}}
%\fbox{\includegraphics*[width=20mm, viewport={0 247 595 842}]{333333-rotational-keili.pdf}}
%\end{subfigure}
%
\end{center}
\caption{\label{fig:333333-rotational-keili}
%
First (left), second (middle), and third (right) iterate
of the CCW prototile.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-rotational-manta-t-36-decomp.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=3 -m='1 121212121333331313131222211111  2 232323232111112121212333322222  3 313131313232321213122223232323131312123211133333  ' -e=0 -w=2 -a='@1' -i=2 -k=+3 -J='*3'
%% zrender -d=3 -m='1 121212121333331313131222211111  2 232323232111112121212333322222  3 313131313232321213122223232323131312123211133333  ' -e=0 -w=2 -a='@2' -i=2 -k=+3 -J='*3'
%% zrender -d=3 -m='1 121212121333331313131222211111  2 232323232111112121212333322222  3 313131313232321213122223232323131312123211133333  ' -e=0 -w=2 -a='@3' -i=2 -k=+3 -J='*3'
%%
%% zrender -T='A0A,B0B,C0C, A+B,B+C,C+A, A-C,B-A,C-B' -d=3 -m='A ABABABABACCCCCACACACABBBBAAAAA  B BCBCBCBCBAAAAABABABABCCCCBBBBB  C CACACACACBCBCBABACABBBBCBCBCBCACACABABCBAAACCCCC ' -e=0 -w=2 -a='0@A' -i=2 -l=,A,B,C -J='*3'
%% zrender -T='A0A,B0B,C0C, A+B,B+C,C+A, A-C,B-A,C-B' -d=3 -m='A ABABABABACCCCCACACACABBBBAAAAA  B BCBCBCBCBAAAAABABABABCCCCBBBBB  C CACACACACBCBCBABACABBBBCBCBCBCACACABABCBAAACCCCC ' -e=0 -w=2 -a='+@B' -i=2 -l=,A,B,C -J='*3'
%% zrender -T='A0A,B0B,C0C, A+B,B+C,C+A, A-C,B-A,C-B' -d=3 -m='A ABABABABACCCCCACACACABBBBAAAAA  B BCBCBCBCBAAAAABABABABCCCCBBBBB  C CACACACACBCBCBABACABBBBCBCBCBCACACABABCBAAACCCCC ' -e=0 -w=2 -a='-@C' -i=2 -l=,A,B,C -J='*3'
%%
\begin{center}
%
{\includegraphics*[width=65mm, viewport={0 237 595 820}]{333333-rotational-manta-t-36-decomp-1.pdf}}%
\hspace*{0mm}% layout
{\includegraphics*[width=65mm, viewport={0 277 595 795}]{333333-rotational-manta-t-36-decomp-2.pdf}}
%
\hspace*{0mm}% layout
{\includegraphics*[width=65mm, viewport={0 310 595 765}]{333333-rotational-manta-t-36-decomp-3.pdf}}
%
\end{center}
\caption{\label{fig:333333-rotational-manta-t-36-decomp}
%
Mutual self-similarity of the curves
\texttt{A} (top left),
\texttt{B} (top right), and
\texttt{C} (bottom).\IMAGENAME%
%
% just two:
%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-rotational-manta-t-36-tile-decomp.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%% manta-t-36-set
%%
%% zrender -T='A0A,B0B,C0C, A+B,B+C,C+A, A-C,B-A,C-B' -d=3 -m='A ABABABABACCCCCACACACABBBBAAAAA  B BCBCBCBCBAAAAABABABABCCCCBBBBB  C CACACACACBCBCBABACABBBBCBCBCBCACACABABCBAAACCCCC ' -e=0.15 -w=10 -a='(1,A+B+C)' -@=0 --colors-pick=1,3 -i=1 -l -L -A=0.3,0.1
%%
%% zrender -T='A0A,B0B,C0C, A+B,B+C,C+A, A-C,B-A,C-B' -d=3 -m='A ABABABABACCCCCACACACABBBBAAAAA  B BCBCBCBCBAAAAABABABABCCCCBBBBB  C CACACACACBCBCBABACABBBBCBCBCBCACACABABCBAAACCCCC ' -e=0 -w=2 -a='(1,A+B+C)' -@=1 --colors-pick=1,3 -i=2 -J='*3' -t='0,-'
%%
%%
\begin{center}
%
{\includegraphics*[width=50mm, viewport={50 285 545 790}]{333333-rotational-manta-t-36-tile-decomp-crv.pdf}}%
\hspace*{5mm}% H
%
{\includegraphics*[width=60mm, viewport={25 285 568 790}]{333333-rotational-manta-t-36-tile-decomp.pdf}}%
%
\end{center}
\caption{\label{fig:333333-rotational-manta-t-36-tile-decomp}
%
The CCW tile \tileS{A+B+C+}{1}:
first iterate, decomposed into curves (left)
and
its self-similarity (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-star-grid-graph.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=3 -a='A+B+C' -m='A A0B0C+A+B-C+A-B-C+A-B0C-A-B+C+A0B+C-A  B B0C+A+B-C-A+B-C0A-B-C+A+B0C+A-B  C C0A-B+C+A-B+C+A-B+C-A-B+C-A0B-C-A+B+C0A+B-C ' -e=0 -l=',A,B,C' -w=10 --arrows  --arrow-offset=0.1 --letters=0.3 -@=2 -i=0 --zoom=4
%%
%% zrender -d=3 -a='A+B+C' -m='A A0B0C+A+B-C+A-B-C+A-B0C-A-B+C+A0B+C-A  B B0C+A+B-C-A+B-C0A-B-C+A+B0C+A-B  C C0A-B+C+A-B+C+A-B+C-A-B+C-A0B-C-A+B+C0A+B-C ' -e=0 -l=',A,B,C' --arrows=0.15 --arrow-offset=0.1 --letters=0.3 -i=0 --zoom=0.8 -w=40
%% zrender -d=3 -a='A-B-C' -m='A A0B0C+A+B-C+A-B-C+A-B0C-A-B+C+A0B+C-A  B B0C+A+B-C-A+B-C0A-B-C+A+B0C+A-B  C C0A-B+C+A-B+C+A-B+C-A-B+C-A0B-C-A+B+C0A+B-C ' -e=0 -l=',A,B,C' --arrows=0.15 --arrow-offset=0.1 --letters=0.3 -i=0 --zoom=0.8 -w=40
%%
%% zrender -d=3 -a='A+B+C-A-B' -m='A A0B0C+A+B-C+A-B-C+A-B0C-A-B+C+A0B+C-A  B B0C+A+B-C-A+B-C0A-B-C+A+B0C+A-B  C C0A-B+C+A-B+C+A-B+C-A-B+C-A0B-C-A+B+C0A+B-C ' -e=0.1 -l=',A,B,C' --arrows=0.15 --arrow-offset=0.1 --letters=0.3 -i=0 --zoom=0.8 -w=20
%%
\begin{center}
%
%\fbox{\includegraphics*[width=60mm, viewport={100 377 595 730}]{333333-star-grid-graph.pdf}}%
\fbox{\includegraphics*[width=75mm, viewport={0 377 595 730}]{333333-star-grid-graph.pdf}}%
%
\hspace*{15mm}% H
\begin{subfigure}[b]{15mm}
{\includegraphics*[width=15mm, viewport={0 247 595 842}]{333333-star-prototile-plus-it0.pdf}}
{\includegraphics*[width=15mm, viewport={0 247 595 842}]{333333-star-prototile-minus-it0.pdf}}
\vspace*{2mm}% V
\end{subfigure}%
%
%\hspace*{8mm}% H
%\begin{subfigure}[b]{30mm}
%{\includegraphics*[width=30mm, viewport={0 247 595 842}]{333333-star-infinity-figure.pdf}}
%\vspace*{2mm}% V
%\end{subfigure}%
%
\end{center}
\caption{\label{fig:333333-star-grid-graph}
%
Coloring of the triangle grid (left),
its two prototiles \tileS{A+B+C+}{1} and \tileS{A-B-C-}{1} (right).
Both prototiles appear in three orientations.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% filled:
%% zrender -d=3 -a='A+B+C' -m='A A0B0C+A+B-C+A-B-C+A-B0C-A-B+C+A0B+C-A  B B0C+A+B-C-A+B-C0A-B-C+A+B0C+A-B  C C0A-B+C+A-B+C+A-B+C-A-B+C-A0B-C-A+B+C0A+B-C ' -e=0 -l=',A,B,C' -w=10 -@=2 -i=0 --zoom=4 -J='*3'

%% zrender -d=3 -a='(3,F+)' -m='F F+F-H+H-G-F0G+G0H0F  G G-F+F-H+H+H-G+G+G-F0G-F0G-F-H+H+H0F0G  H H-G+G-F+F-H+H+H0F0G-F0G+G0H-G-F+F-H+H ' -e=0 -w=10 -i=3 --letters --arrows=0.1 --arrow-offset=0.1 --zoom=10 --no-text
%%%% color version:
%% zrender -d=3 -a='_(4,(4,FGH)+(4,H+H-G+G-F+F-)H-G(4,HFG)+(4,G+G-F+F-H+H-)G-) ' -m='F F  G G  H H  t t' -e=0 -w=10 -i=0 -l --arrows=0.1 --letters --arrow-offset=0.1 --zoom=2
%%
%% zrender -d=3 -m='F F  G G  H H ' -e=0 -w=15 -a='_(3,F+)' -i=2 --zoom=0.5 --no-text --arrows=0.15 --arrow-offset=0.1 --letters -l
%% zrender -d=3 -m='F F  G G  H H ' -e=0 -w=15 -a='_(3,G+)' -i=2 --zoom=0.5 --no-text --arrows=0.15 --arrow-offset=0.1 --letters -l
%% zrender -d=3 -m='F F  G G  H H ' -e=0 -w=15 -a='_(3,H+)' -i=2 --zoom=0.5 --no-text --arrows=0.15 --arrow-offset=0.1 --letters -l
%% zrender -d=3 -m='F F  G G  H H ' -e=0 -w=15 -a='_F-H-G-' -i=2 --zoom=0.5 --no-text --arrows=0.15 --arrow-offset=0.1 --letters -l
%%
%% zrender -d=3 -a='_F+F0G+G0H+H+H-G-F' -m='F F0G0H0F  G G0H0F0G  H H0F0G0H ' -e=0.1 -l -w=15 --arrows --letters -i=0 --no-text



%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-star-lattice-tiles-outline.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-translational-x3-hex.txt  curve-set r16-hex-var-1
%%
%% zrender -d=3 -@=0 -a='(3,A+B+C-)' -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0.1 -l=',A,B,C' -w=20 -A=0.17 -L -i=0
%% zrender -d=3 -@=0 -a='(3,B+C+A-)' -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0.1 -l=',A,B,C' -w=20 -A=0.17 -L -i=0
%% zrender -d=3 -@=0 -a='(3,C+A+B-)' -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0.1 -l=',A,B,C' -w=20 -A=0.17 -L -i=0
%%
%% zrender -d=3 -@=0 -a='(3,A-B-C+)' -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0.1 -l=',A,B,C' -w=20 -A=0.17 -L -i=0
%% zrender -d=3 -@=0 -a='(3,B-C-A+)' -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0.1 -l=',A,B,C' -w=20 -A=0.17 -L -i=0
%% zrender -d=3 -@=0 -a='(3,C-A-B+)' -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0.1 -l=',A,B,C' -w=20 -A=0.17 -L -i=0
%%
%%
%% zrender -d=3 -@=0 -a='(3,A+B+C-)' -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0.1 -l=',A,B,C' -w=20 -A=0.17 -J='*3' -i=0
%% zrender -d=3 -@=0 -a='(3,B+C+A-)' -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0.1 -l=',A,B,C' -w=20 -A=0.17 -J='*3' -i=0
%% zrender -d=3 -@=0 -a='(3,C+A+B-)' -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0.1 -l=',A,B,C' -w=20 -A=0.17 -J='*3' -i=0
%%
%% zrender -d=3 -@=0 -a='(3,A-B-C+)' -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0.1 -l=',A,B,C' -w=20 -A=0.17 -J='*3' -i=0
%% zrender -d=3 -@=0 -a='(3,B-C-A+)' -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0.1 -l=',A,B,C' -w=20 -A=0.17 -J='*3' -i=0
%% zrender -d=3 -@=0 -a='(3,C-A-B+)' -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0.1 -l=',A,B,C' -w=20 -A=0.17 -J='*3' -i=0
%%
\begin{center}
%
%{\includegraphics*[width=43mm, viewport={0 247 595 842}]{333333-star-lattice-tiles-outline-plusABC3.pdf}}%
%{\includegraphics*[width=43mm, viewport={0 247 595 842}]{333333-star-lattice-tiles-outline-plusBCA3.pdf}}%
%{\includegraphics*[width=43mm, viewport={0 247 595 842}]{333333-star-lattice-tiles-outline-plusCAB3.pdf}}
%%
%{\includegraphics*[width=43mm, viewport={0 247 595 842}]{333333-star-lattice-tiles-outline-minusABC3.pdf}}%
%{\includegraphics*[width=43mm, viewport={0 247 595 842}]{333333-star-lattice-tiles-outline-minusBCA3.pdf}}%
%{\includegraphics*[width=43mm, viewport={0 247 595 842}]{333333-star-lattice-tiles-outline-minusCAB3.pdf}}
%
{\includegraphics*[width=21.5mm, viewport={0 247 595 842}]{333333-star-lattice-tiles-outline-plusABC3.pdf}}%
{\includegraphics*[width=21.5mm, viewport={0 247 595 842}]{333333-star-lattice-tiles-outline-plusBCA3.pdf}}%
{\includegraphics*[width=21.5mm, viewport={0 247 595 842}]{333333-star-lattice-tiles-outline-plusCAB3.pdf}}%
%
{\includegraphics*[width=21.5mm, viewport={0 247 595 842}]{333333-star-lattice-tiles-outline-minusABC3.pdf}}%
{\includegraphics*[width=21.5mm, viewport={0 247 595 842}]{333333-star-lattice-tiles-outline-minusBCA3.pdf}}%
{\includegraphics*[width=21.5mm, viewport={0 247 595 842}]{333333-star-lattice-tiles-outline-minusCAB3.pdf}}
%
%
{\includegraphics*[width=21.5mm, viewport={0 227 595 842}]{333333-star-lattice-tiles-outline-plusABC3-filled.pdf}}%
{\includegraphics*[width=21.5mm, viewport={0 227 595 842}]{333333-star-lattice-tiles-outline-plusBCA3-filled.pdf}}%
{\includegraphics*[width=21.5mm, viewport={0 227 595 842}]{333333-star-lattice-tiles-outline-plusCAB3-filled.pdf}}%
%
{\includegraphics*[width=21.5mm, viewport={0 247 595 842}]{333333-star-lattice-tiles-outline-minusABC3-filled.pdf}}%
{\includegraphics*[width=21.5mm, viewport={0 247 595 842}]{333333-star-lattice-tiles-outline-minusBCA3-filled.pdf}}%
{\includegraphics*[width=21.5mm, viewport={0 247 595 842}]{333333-star-lattice-tiles-outline-minusCAB3-filled.pdf}}
%
\end{center}
\caption{\label{fig:333333-star-lattice-tiles-outline}
%
Left to right: the lattice tiles
(\texttt{A+B+C-})$^3$,
(\texttt{B+C+A-})$^3$,
(\texttt{C+A+B-})$^3$,
(\texttt{A-B-C+})$^3$,
(\texttt{B-C-A+})$^3$, and
(\texttt{C-A-B+})$^3$.
The bottom row shows the corresponding area drawings.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-star-lattice-tiles.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-translational-x3-hex.txt  curve-set r16-hex-var-1
%%
%% zrender -d=3 -@=0 -a='(3,A+B+C-)' -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0 -l=',A,B,C' -w=1 -i=3 -J='*3'
%% zrender -d=3 -@=0 -a='(3,B+C+A-)' -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0 -l=',A,B,C' -w=1 -i=3 -J='*3'
%% zrender -d=3 -@=0 -a='(3,C+A+B-)' -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0 -l=',A,B,C' -w=1 -i=3 -J='*3'
%%
%% zrender -d=3 -@=0 -a='(3,A-B-C+)' -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0 -l=',A,B,C' -w=1 -i=3 -J='*3'
%% zrender -d=3 -@=0 -a='(3,B-C-A+)' -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0 -l=',A,B,C' -w=1 -i=3 -J='*3'
%% zrender -d=3 -@=0 -a='(3,C-A-B+)' -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0 -l=',A,B,C' -w=1 -i=3 -J='*3'
%%
\begin{center}
%
{\includegraphics*[width=43mm, viewport={0 247 595 812}]{333333-star-lattice-tiles-plusABC3.pdf}}%
{\includegraphics*[width=43mm, viewport={0 247 595 812}]{333333-star-lattice-tiles-plusBCA3.pdf}}%
{\includegraphics*[width=43mm, viewport={0 247 595 812}]{333333-star-lattice-tiles-plusCAB3.pdf}}
%
{\includegraphics*[width=43mm, viewport={0 260 595 822}]{333333-star-lattice-tiles-minusABC3.pdf}}%
{\includegraphics*[width=43mm, viewport={0 260 595 822}]{333333-star-lattice-tiles-minusBCA3.pdf}}%
{\includegraphics*[width=43mm, viewport={0 260 595 822}]{333333-star-lattice-tiles-minusCAB3.pdf}}
%
\end{center}
\caption{\label{fig:333333-star-lattice-tiles}
%
Third iterates of the lattice tiles.
Top row, left to right:
(\texttt{A+B+C-})$^3$,
(\texttt{B+C+A-})$^3$, and
(\texttt{C+A+B-})$^3$.
Bottom row, left to right:
(\texttt{A-B-C+})$^3$,
(\texttt{B-C-A+})$^3$, and
(\texttt{C-A-B+})$^3$.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-star-r16-manta-decomp.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-star-x3.txt , curve-set r16-manta
%%
%% zrender -d=3 -a='A' -m='A A0B+C-A-B0C+A+B-C+A0B-C-A+B-C0A0B+C+A-B+C-A  B B0C0A+B0C-A-B+C-A0B0C+A+B-C+A-B  C C0A0B+C-A-B0C+A+B-C ' -e=0.15 -l=',A,B,C' -w=1 -i=0 -@=1 -w=20 -L=0.4 -A --fancy-print-maps -r=i0
%% zrender -d=3 -a='B' -m='A A0B+C-A-B0C+A+B-C+A0B-C-A+B-C0A0B+C+A-B+C-A  B B0C0A+B0C-A-B+C-A0B0C+A+B-C+A-B  C C0A0B+C-A-B0C+A+B-C ' -e=0.15 -l=',A,B,C' -w=1 -i=0 -@=1 -w=20 -L=0.4 -A --fancy-print-maps -r=i1
%% zrender -d=3 -a='C' -m='A A0B+C-A-B0C+A+B-C+A0B-C-A+B-C0A0B+C+A-B+C-A  B B0C0A+B0C-A-B+C-A0B0C+A+B-C+A-B  C C0A0B+C-A-B0C+A+B-C ' -e=0.15 -l=',A,B,C' -w=1 -i=0 -@=1 -w=20 -L=0.4 -A --fancy-print-maps -r=i2
%%
%% zrender -d=3 -a='A' -m='A A0B+C-A-B0C+A+B-C+A0B-C-A+B-C0A0B+C+A-B+C-A  B B0C0A+B0C-A-B+C-A0B0C+A+B-C+A-B  C C0A0B+C-A-B0C+A+B-C ' -e=0 -l=',A,B,C' -w=1 -i=3 -@=1 -w=5 -J='*3'  --fancy-print-maps -r=i0
%% zrender -d=3 -a='B' -m='A A0B+C-A-B0C+A+B-C+A0B-C-A+B-C0A0B+C+A-B+C-A  B B0C0A+B0C-A-B+C-A0B0C+A+B-C+A-B  C C0A0B+C-A-B0C+A+B-C ' -e=0 -l=',A,B,C' -w=1 -i=3 -@=1 -w=5 -J='*3'  --fancy-print-maps -r=i1
%% zrender -d=3 -a='C' -m='A A0B+C-A-B0C+A+B-C+A0B-C-A+B-C0A0B+C+A-B+C-A  B B0C0A+B0C-A-B+C-A0B0C+A+B-C+A-B  C C0A0B+C-A-B0C+A+B-C ' -e=0 -l=',A,B,C' -w=1 -i=3 -@=1 -w=5 -J='*3'  --fancy-print-maps -r=i2
%%
%%
\begin{center}
%% small version:
%{\includegraphics*[width=43mm, viewport={0 247 595 842}]{333333-star-manta-decomp-A-it1.pdf}}%
%{\includegraphics*[width=43mm, viewport={0 247 595 842}]{333333-star-manta-decomp-B-it1.pdf}}%
%{\includegraphics*[width=43mm, viewport={0 247 595 842}]{333333-star-manta-decomp-C-it1.pdf}}
%%
%{\includegraphics*[width=43mm, viewport={0 247 595 822}]{333333-star-manta-decomp-A-it4.pdf}}%
%{\includegraphics*[width=43mm, viewport={0 247 595 822}]{333333-star-manta-decomp-B-it4.pdf}}%
%{\includegraphics*[width=43mm, viewport={0 247 595 822}]{333333-star-manta-decomp-C-it4.pdf}}
%
%% big version:
\begin{subfigure}[b]{51mm}
{\includegraphics*[width=50mm, viewport={0 247 595 842}]{333333-star-manta-decomp-A-it1.pdf}}
\vspace*{6mm}% V
\end{subfigure}%
{\includegraphics*[width=70mm, viewport={0 247 595 822}]{333333-star-manta-decomp-A-it4.pdf}}
%
\begin{subfigure}[b]{51mm}
{\includegraphics*[width=50mm, viewport={0 247 595 842}]{333333-star-manta-decomp-B-it1.pdf}}%
\vspace*{6mm}% V
\end{subfigure}%
{\includegraphics*[width=70mm, viewport={0 247 595 822}]{333333-star-manta-decomp-B-it4.pdf}}
%
\begin{subfigure}[b]{51mm}
{\includegraphics*[width=50mm, viewport={0 247 595 842}]{333333-star-manta-decomp-C-it1.pdf}}%
\vspace*{6mm}% V
\end{subfigure}%
{\includegraphics*[width=70mm, viewport={0 247 595 822}]{333333-star-manta-decomp-C-it4.pdf}}
%
%
\end{center}
\caption{\label{fig:333333-star-r16-manta-decomp}
%
Mutual self-similarity of a curve-set where all curves have reflection symmetry.
First (left) and fourth (right) iterates.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-star-r16-manta-grid.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=3 -a='A' -m='A A0B+C-A-B0C+A+B-C+A0B-C-A+B-C0A0B+C+A-B+C-A  B B0C0A+B0C-A-B+C-A0B0C+A+B-C+A-B  C C0A0B+C-A-B0C+A+B-C' -e=0 -l=',A,B,C' -w=2 -i=2 -J='*3' --grid=10,10 --zoom=1.3 --shift-y=-0.05
%%
\begin{center}
%
\fbox{\includegraphics*[width=129mm, viewport={0 447 595 842}]{333333-star-r16-manta-grid.pdf}}%
\hspace*{0mm}% layout
%
%
\end{center}
\caption{\label{fig:333333-star-r16-manta-grid}
%
Second iterates of the curves on the grid.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-star-r16-var1-it1.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=3 -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0.15 -l=',A,B,C' -w=15 -A -L -i=0 -@=1 -a='0A'
%% zrender -d=3 -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0.15 -l=',A,B,C' -w=15 -A -L -i=0 -@=1 -a='+B'
%% zrender -d=3 -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0.15 -l=',A,B,C' -w=15 -A -L -i=0 -@=1 -a='-C'
%%
\begin{center}
%
{\includegraphics*[width=42mm, viewport={0 255 595 780}]{333333-star-r16-var1-it1-A.pdf}}%
\hspace*{0mm}% layout
{\includegraphics*[width=40mm, viewport={0 255 595 815}]{333333-star-r16-var1-it1-B.pdf}}%
\hspace*{0mm}% layout
{\includegraphics*[width=40mm, viewport={0 255 595 822}]{333333-star-r16-var1-it1-C.pdf}}%
%
\end{center}
\caption{\label{fig:333333-star-r16-var1-it1}
%
Motifs of the curves
\texttt{A} (left), \texttt{B} (middle), and \texttt{C} (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-star-tile-minus.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-translational-x3-hex.txt  curve-set r16-hex-var-1
%%
%% zrender -d=3 -a='A-B-C' -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0 -l=',A,B,C' -w=1 -i=3 -J='*3' --fancy-print-maps
%% zrender -d=3 -a='A-B-C' -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0 -t='+,0' --colors-pick=1,3  -w=1 -@=1 -i=3 -J='*3'
%%
\begin{center}
%
{\includegraphics*[width=50mm, viewport={0 255 595 819}]{333333-star-tile-minus.pdf}}%
\hspace*{10mm}% layout
{\includegraphics*[width=50mm, viewport={0 255 595 819}]{333333-star-tile-minus-decomp.pdf}}%
%
\end{center}
\caption{\label{fig:333333-star-tile-minus}
%
The CW prototile \tileS{A-B-C-}{1} split into curves (left) and
its decomposition showing its self-similarity (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-star-tile-plus.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-translational-x3-hex.txt  curve-set r16-hex-var-1
%%
%% zrender -d=3 -a='A+B+C' -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0 -l=',A,B,C' -w=1 -i=3 -J='*3' --fancy-print-maps
%% zrender -d=3 -a='A+B+C' -m='A A+B-C+A-B-C0A+B0C-A-B+C-A+B+C0A0B+C-A  B B+C-A+B-C-A0B+C-A+B+C0A-B-C+A-B0C+A+B-C+A0B-C-A+B  C C0A0B0C ' -e=0 -t='-,0' --colors-pick=1,3  -w=1 -@=1 -i=3 -J='*3'
%%
\begin{center}
%
{\includegraphics*[width=50mm, viewport={0 255 595 816}]{333333-star-tile-plus.pdf}}%
\hspace*{10mm}% layout
{\includegraphics*[width=50mm, viewport={0 255 595 816}]{333333-star-tile-plus-decomp.pdf}}%
%
\end{center}
\caption{\label{fig:333333-star-tile-plus}
%
The CCW prototile \tileS{A+B+C+}{1} split into curves (left) and
its decomposition into smaller copies of itself showing its self-similarity (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-translational-grid-graph.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=3 -a='_(4,(4,FGH)+(4,H+H-G+G-F+F-)H-G(4,HFG)+(4,G+G-F+F-H+H-)G-) ' -m='F F  G G  H H  t t' -e=0 -w=10 -i=0 -l --arrows=0.1 --letters --arrow-offset=0.1 --zoom=2
%%
%% zrender -d=3 -m='F F  G G  H H ' -e=0 -w=40 -a='_(3,F+)' -i=2 --zoom=0.8 --arrows=0.15 --arrow-offset=0.1 --letters -l
%% zrender -d=3 -m='F F  G G  H H ' -e=0 -w=40 -a='_(3,G+)' -i=2 --zoom=0.8 --arrows=0.15 --arrow-offset=0.1 --letters -l
%% zrender -d=3 -m='F F  G G  H H ' -e=0 -w=40 -a='_(3,H+)' -i=2 --zoom=0.8 --arrows=0.15 --arrow-offset=0.1 --letters -l
%% zrender -d=3 -m='F F  G G  H H ' -e=0 -w=40 -a='_F-H-G-' -i=2 --zoom=0.8 --arrows=0.15 --arrow-offset=0.1 --letters -l
%%
%% zrender -d=3 -a='_F+F0G+G0H+H+H-G-F' -m='F F0G0H0F  G G0H0F0G  H H0F0G0H ' -e=0.1 -l -w=20 --arrows --letters -i=0 --no-text
%%
\begin{center}
%{\includegraphics*[width=60mm, viewport={0 377 595 802}]{333333-translational-grid-graph.pdf}}%
\fbox{\includegraphics*[width=60mm, viewport={100 377 595 730}]{333333-translational-grid-graph.pdf}}%
%
\hspace{10mm}% layout
\begin{subfigure}[b]{18mm}
{\includegraphics*[width=17mm, viewport={0 247 595 842}]{333333-translational-prototile-F3-it0.pdf}}
{\includegraphics*[width=17mm, viewport={0 247 595 842}]{333333-translational-prototile-H3-it0.pdf}}
\vspace*{0mm}% V
\end{subfigure}%
%
\begin{subfigure}[b]{18mm}
{\includegraphics*[width=17mm, viewport={0 247 595 842}]{333333-translational-prototile-G3-it0.pdf}}
{\includegraphics*[width=17mm, viewport={0 247 595 842}]{333333-translational-prototile-FHG-it0.pdf}}
\vspace*{0mm}% V
\end{subfigure}%
%\hspace{1mm}% layout
%\begin{subfigure}[b]{30mm}
%{\includegraphics*[width=30mm, viewport={0 80 595 842}]{333333-translational-infinity-figure.pdf}}
%%\vspace*{0mm}% V
%\end{subfigure}%
%
\end{center}
\caption{\label{fig:333333-translational-grid-graph}
%
A coloring of the triangle grid with three colors (left)
and its four prototiles
\tileS{F+}{3},
\tileS{G+}{3},
\tileS{H+}{3}, and
\tileS{F-H-G-}{1} (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-translational-minus-tile-self-similarity.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=3 -a='(1,@F-@H-@G)' -m='F F+F-H+H-G-F0G+G0H0F  G G-F+F-H+H+H-G+G+G-F0G-F0G-F-H+H+H0F0G  H H-G+G-F+F-H+H+H0F0G-F0G+G0H-G-F+F-H+H ' -e=0 -w=5 -i=3 --colors-pick='1,3' -t='0,+' -J='F,3,3;G,3,3;H,3,3;'
%%
%% zrender -d=3 -a='(1,F-H-G)+(1,G-F-H)+(1,H-G-F)' -m='F F+F-H+H-G-F0G+G0H0F  G G-F+F-H+H+H-G+G+G-F0G-F0G-F-H+H+H0F0G  H H-G+G-F+F-H+H+H0F0G-F0G+G0H-G-F+F-H+H ' -e=0 -w=5 -i=3 --colors-pick='1,3' -t='0,+' -J='F,3,3;G,3,3;H,3,3;'
%%
\begin{center}
%
{\includegraphics*[width=65mm, viewport={0 247 595 822}]{333333-translational-minus-tile-self-similarity.pdf}}%
\hspace*{0mm}% layout
%
{\includegraphics*[width=65mm, viewport={0 247 595 822}]{333333-translational-minus-tile-self-similarity-three.pdf}}
%
\end{center}
\caption{\label{fig:333333-translational-minus-tile-self-similarity}
%
Self-similarity of the CW prototile \tileS{F-H-G-}{1} (left).
The prototile tiles the plane, appearing in three orientations.
The arrangement of three prototiles (right) is a lattice tile.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-translational-plus-tiles-self-similarity.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%% note the ordering!
%% zrender -d=3 -a='_(3,@F+)' -m='F F+F-H+H-G-F0G+G0H0F  G G-F+F-H+H+H-G+G+G-F0G-F0G-F-H+H+H0F0G  H H-G+G-F+F-H+H+H0F0G-F0G+G0H-G-F+F-H+H ' -e=0 -w=12 -i=2 -l -J
%% zrender -d=3 -a='_(3,@G+)' -m='F F+F-H+H-G-F0G+G0H0F  G G-F+F-H+H+H-G+G+G-F0G-F0G-F-H+H+H0F0G  H H-G+G-F+F-H+H+H0F0G-F0G+G0H-G-F+F-H+H ' -e=0 -w=7 -i=2 -l -J
%% zrender -d=3 -a='_(3,@H+)' -m='F F+F-H+H-G-F0G+G0H0F  G G-F+F-H+H+H-G+G+G-F0G-F0G-F-H+H+H0F0G  H H-G+G-F+F-H+H+H0F0G-F0G+G0H-G-F+F-H+H ' -e=0 -w=6 -i=2 -l -J
%%
%% zrender -d=3 -a='_(3,F+)--(3,H+)--(3,G+)' -m='F F+F-H+H-G-F0G+G0H0F  G G-F+F-H+H+H-G+G+G-F0G-F0G-F-H+H+H0F0G  H H-G+G-F+F-H+H+H0F0G-F0G+G0H-G-F+F-H+H ' -e=0 -w=5 -i=3 -l -J='F,3,3;G,3,3;H,3,3;'
%%
\begin{center}
%
\begin{subfigure}[b]{55mm}
{\includegraphics*[width=55mm, viewport={20 247 595 822}]{333333-translational-plus-tiles-self-similarity-F.pdf}}
{\includegraphics*[width=55mm, viewport={20 247 595 822}]{333333-translational-plus-tiles-self-similarity-H.pdf}}
\end{subfigure}
%
\hspace*{4mm}% layout
\begin{subfigure}[b]{55mm}
{\includegraphics*[width=55mm, viewport={20 247 595 822}]{333333-translational-plus-tiles-self-similarity-G.pdf}}
{\includegraphics*[width=55mm, viewport={20 247 595 822}]{333333-translational-plus-tiles-self-similarity-FGH.pdf}}
\end{subfigure}
%
\end{center}
\caption{\label{fig:333333-translational-plus-tiles-self-similarity}
%
Mutual self-similarity of the CCW prototiles
\tileS{F+}{3} (upper left),
\tileS{G+}{3} (upper right), and
\tileS{H+}{3} (lower left).
Each is composed of smaller copies of all three of the prototiles.
The arrangement of three prototiles (lower right) is a lattice tile.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/333333-translational-r25-motifs.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
% zrender -d=3 -a='F' -m='F F+F-H+H-G-F0G+G0H0F  G G-F+F-H+H+H-G+G+G-F0G-F0G-F-H+H+H0F0G  H H-G+G-F+F-H+H+H0F0G-F0G+G0H-G-F+F-H+H ' -e=0 -w=18 -i=0 -@=1 -l=,F,G,H -L=0.4 -A=0.2,0.1 -e=0.12
% zrender -d=3 -a='G' -m='F F+F-H+H-G-F0G+G0H0F  G G-F+F-H+H+H-G+G+G-F0G-F0G-F-H+H+H0F0G  H H-G+G-F+F-H+H+H0F0G-F0G+G0H-G-F+F-H+H ' -e=0 -w=18 -i=0 -@=1 -l=,F,G,H -L=0.4 -A=0.2,0.1 -e=0.12
% zrender -d=3 -a='H' -m='F F+F-H+H-G-F0G+G0H0F  G G-F+F-H+H+H-G+G+G-F0G-F0G-F-H+H+H0F0G  H H-G+G-F+F-H+H+H0F0G-F0G+G0H-G-F+F-H+H ' -e=0 -w=18 -i=0 -@=1 -l=,F,G,H -L=0.4 -A=0.2,0.1 -e=0.12

%%
%%
\begin{center}
%
{\includegraphics*[width=38mm, viewport={80 400 525 705}]{333333-translational-r25-motifs-F.pdf}}%
{\includegraphics*[width=38mm, viewport={50 380 525 715}]{333333-translational-r25-motifs-G.pdf}}%
{\includegraphics*[width=42mm, viewport={40 298 575 790}]{333333-translational-r25-motifs-H.pdf}}%
%
\end{center}
\caption{\label{fig:333333-translational-r25-motifs}
%
Motifs for the curves of a curve-set of order 25.
From left to right,
motifs for curve \texttt{F}, \texttt{G}, and \texttt{H}.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3446-3464-curve-set-var-2-motifs.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -m='A A++A++A---B---F+++E+++F---D---A---B++++C--E--C++++D---A++A++A  B B  C C  D D  E E  F F---D++++B---F---D++++B---F+++E--C++++D++++B---F+++E--C--E--C--E--C++++D++++B---F ' -l -w=18 -i=0 -@=1 -e=0.15 -L=0.5 -A=0.3,0.1 -a=_A
%% zrender -d=12 -m='A A++A++A---B---F+++E+++F---D---A---B++++C--E--C++++D---A++A++A  B B  C C  D D  E E  F F---D++++B---F---D++++B---F+++E--C++++D++++B---F+++E--C--E--C--E--C++++D++++B---F ' -l -w=18 -i=0 -@=1 -e=0.15 -L=0.5 -A=0.3,0.1 -a=_F
%%
\begin{center}
%
{\includegraphics*[width=40mm, viewport={0 277 595 785}]{3446-3464-curve-set-var-2-motifs-A.pdf}}%
\hspace*{5mm}% layout
{\includegraphics*[width=40mm, viewport={0 277 595 785}]{3446-3464-curve-set-var-2-motifs-F.pdf}}%
%
\end{center}
\caption{\label{fig:3446-3464-curve-set-var-2-motifs}
%
Motifs for the curves \texttt{A} (left) and \texttt{F} (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3446-3464-curve-set-var-2-prototile-A6.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -a='(6,A++)' -m='A A++A++A---B---F+++E+++F---D---A---B++++C--E--C++++D---A++A++A  B B  C C  D D  E E  F F---D++++B---F---D++++B---F+++E--C++++D++++B---F+++E--C--E--C--E--C++++D++++B---F ' -k=-12 -w=10 -i=1 -e=0.15 -L=0.4 -A=0.3 # grows
%%
%% zrender -d=12 -a='(6,A++)' -m='A A++A++A---B---F+++E+++F---D---A---B++++C--E--C++++D---A++A++A  B B  C C  D D  E E  F F---D++++B---F---D++++B---F+++E--C++++D++++B---F+++E--C--E--C--E--C++++D++++B---F ' -k=-12 -e=0 -w=12 -i=4 -J
%%
%%
\begin{center}
%
{\includegraphics*[width=54.5mm, viewport={0 247 595 832}]{3446-3464-curve-set-var-2-prototile-A6-it1.pdf}}%
\hspace*{0mm}% layout
{\includegraphics*[width=64.5mm, viewport={0 257 595 815}]{3446-3464-curve-set-var-2-prototile-A6-it.pdf}}%
%
\end{center}
\caption{\label{fig:3446-3464-curve-set-var-2-prototile-A6}
%
First (left) and fourth (right) iterate of the prototile \tileS{A++}{6}.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3446-3464-curve-set-var-2-prototile-ABFD1.tex <==
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -a='(1,A---B---F---D)' -m='A A++A++A---B---F+++E+++F---D---A---B++++C--E--C++++D---A++A++A  B B  C C  D D  E E  F F---D++++B---F---D++++B---F+++E--C++++D++++B---F+++E--C--E--C--E--C++++D++++B---F ' -k=-12 -w=10 -i=1 -e=0.15 -L=0.4 -A=0.3 # grows
%%
%% zrender -d=12 -a='(1,A---B---F---D)' -m='A A++A++A---B---F+++E+++F---D---A---B++++C--E--C++++D---A++A++A  B B  C C  D D  E E  F F---D++++B---F---D++++B---F+++E--C++++D++++B---F+++E--C--E--C--E--C++++D++++B---F ' -k=-12 -e=0 -w=12 -i=5 -J
%%
%%
\begin{center}
%
{\includegraphics*[width=52mm, viewport={0 247 595 822}]{3446-3464-curve-set-var-2-prototile-ABFD1-it1.pdf}}%
\hspace*{3mm}% layout
{\includegraphics*[width=55mm, viewport={0 267 595 812}]{3446-3464-curve-set-var-2-prototile-ABFD1-it.pdf}}%
%
\end{center}
\caption{\label{fig:3446-3464-curve-set-var-2-prototile-ABFD1}
%
First (left) and fifth (right) iterate of
the prototile \tileS{A---B---F---D---}{1}.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3446-3464-curve-set-var-2-prototile-EF2.tex <==
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -a='(2,E+++F+++)' -m='A A++A++A---B---F+++E+++F---D---A---B++++C--E--C++++D---A++A++A  B B  C C  D D  E E  F F---D++++B---F---D++++B---F+++E--C++++D++++B---F+++E--C--E--C--E--C++++D++++B---F ' -k=-12 -w=10 -i=1 -e=0.15 -L=0.4 -A=0.3 -r=A
%%
%% zrender -d=12 -a='(2,E+++F+++)' -m='A A++A++A---B---F+++E+++F---D---A---B++++C--E--C++++D---A++A++A  B B  C C  D D  E E  F F---D++++B---F---D++++B---F+++E--C++++D++++B---F+++E--C--E--C--E--C++++D++++B---F ' -k=-12 -e=0 -w=12 -i=5 -J -r=A
%%
%%
\begin{center}
%
{\includegraphics*[width=50mm, viewport={0 247 595 842}]{3446-3464-curve-set-var-2-prototile-EF2-it1.pdf}}%
\hspace*{5mm}% layout
{\includegraphics*[width=50mm, viewport={0 247 595 842}]{3446-3464-curve-set-var-2-prototile-EF2-it.pdf}}%
%
\end{center}
\caption{\label{fig:3446-3464-curve-set-var-2-prototile-EF2}
%
First (left) and fifth (right) iterate of the prototile \tileS{E+++F+++}{2}.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3446-3464-decomp-var-2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% coloring by hand:
%% zrender -d=12 -a='A++__A++__A---B---__F+++E+++_F---D---_A---B++++C--E--C++++D---__A++~~A++~~~~~~~~A' -m='A A++A++A---B---F+++E+++F---D---A---B++++C--E--C++++D---A++A++A  B B  C C  D D  E E  F F---D++++B---F---D++++B---F+++E--C++++D++++B---F+++E--C--E--C--E--C++++D++++B---F ' -e=0 -w=4 -i=4 -J='A,6,4;B,3,4;C,3,6;D,3,4;E,4,6;F,4,4;'
%%
%% zrender -d=12 -a='@F' -m='A A++A++A---B---F+++E+++F---D---A---B++++C--E--C++++D---A++A++A  B B  C C  D D  E E  F F---D++++B---F---D++++B---F+++E--C++++D++++B---F+++E--C--E--C--E--C++++D++++B---F ' -k=-12 -e=0 -w=4 -i=4 -J='A,6,4;B,3,4;C,3,6;D,3,4;E,4,6;F,4,4;'
%%
\begin{center}
{\includegraphics*[width=70mm, viewport={0 260 595 800}]{3446-3464-decomp-var-2-A.pdf}}%
\hspace*{0mm}% layout
{\includegraphics*[width=44mm, viewport={100 247 500 822}]{3446-3464-decomp-var-2-F.pdf}}%
\end{center}
\caption{\label{fig:3446-3464-decomp-var-2}
%
Mutual self-similarity of curves \texttt{A} (left)
and \texttt{F} (right).
Coloring by curves and orientation.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%% zrender -d=12 -a='@A' -m='A A++A++A---B---F+++E+++F---D---A---B++++C--E--C++++D---A++A++A  B B  C C  D D  E E  F F---D++++B---F---D++++B---F+++E--C++++D++++B---F+++E--C--E--C--E--C++++D++++B---F ' -k=-12 -e=0 -w=2 -i=4

%% mental model for curve F:
%% zrender -i=5 -m='A A+A---A+A+A' -a='(6,A+)' -d=6 -e=0 -k=+6 -w=1
%% completed to Gosper island:
%% zrender -i=5 -m='A A+A+A---A-A+A+A' -a='(6,A+)' -d=6 -e=0 -k=+6 -w=1
%% alternatively:
%% zrender -i=5 -m='A A+A-A---A+A+A+A' -a='(6,A+)' -d=6 -e=0 -k=+6 -w=1


%% nice stuff:

%% zrender -d=12 -a='(6,X++__)' -m='A A++A++A---B---F+++E+++F---D---A---B++++C--E--C++++D---A++A++A  B B  C C  D D  E E  F F---D++++B---F---D++++B---F+++E--C++++D++++B---F+++E--C--E--C--E--C++++D++++B---F  X A++__A++__A---B---__F+++E+++_F---D---_A---B++++C--E--C++++D---__A++~~A++~~~~~~~~A ' -e=0 -w=1 -i=5

%% inside:
%% zrender -d=12 -a='(6,@B---@F---@D++++_)' -m='A A++A++A---B---F+++E+++F---D---A---B++++C--E--C++++D---A++A++A  B B  C C  D D  E E  F F---D++++B---F---D++++B---F+++E--C++++D++++B---F+++E--C--E--C--E--C++++D++++B---F ' -k=-12 -e=0 -w=2 -i=4
%% outside
%% zrender -d=12 -a='(6,@B---@F---@D----_)' -m='A A++A++A---B---F+++E+++F---D---A---B++++C--E--C++++D---A++A++A  B B  C C  D D  E E  F F---D++++B---F---D++++B---F+++E--C++++D++++B---F+++E--C--E--C--E--C++++D++++B---F ' -k=-12 -e=0 -w=2 -i=4

%% Gosper island:
%% zrender -d=12 -a='(6,@X++)-----(6,@B---@F---@D++++_)' -m='A A++A++A---B---F+++E+++F---D---A---B++++C--E--C++++D---A++A++A  B B  C C  D D  E E  F F---D++++B---F---D++++B---F+++E--C++++D++++B---F+++E--C--E--C--E--C++++D++++B---F  X A++__A++__A---B---__F+++E+++_F---D---_A---B++++C--E--C++++D---__A++~~A++~~~~~~~~A' -k=-12 -e=0 -w=1 -i=4

%% zrender -d=12 -a='(6,@X++)-----(6,@B---@F---@D++++)' -m='A A++A++A---B---F+++E+++F---D---A---B++++C--E--C++++D---A++A++A  B B  C C  D D  E E  F F---D++++B---F---D++++B---F+++E--C++++D++++B---F+++E--C--E--C--E--C++++D++++B---F  X A++A++A---B---F+++E+++F---D---A---B++++C--E--C++++D---A++A++A' -l -e=0 -w=1 -i=4



%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3446-3464-grid-graph-repeat.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -a='_(6,@@A++)' -m='A A---B++++C++++D---A++A---B---F+++E+++F---D---A---B++++C--E--C--E--C++++D++++B---F+++E+++F---D---A---B++++C++++D---A++A  B B  C C  D D  E E  F F---D++++B---F+++E--C--E+++F ' -e=0 -w=10 -i=0 --arrows=0.15 --arrow-offset=0.1 --letters=0.45 --zoom=2.7 -l
%%
%% zrender -d=12 -a='_(6,A++)' -m='A A  B B  C C  D D  E E  F F ' -e=0 -w=30 -i=0 --arrows=0.2 --arrow-offset=0.1 --letters=0.6 -l --zoom=0.9
%% zrender -d=12 -a='_(1,B++++C++++D)' -m='A A  B B  C C  D D  E E  F F ' -e=0 -w=30 -i=0 --arrows=0.2 --arrow-offset=0.1 --letters=0.35 -l --zoom=0.8
%% zrender -d=12 -a='_(2,E+++F+++)' -m='A A  B B  C C  D D  E E  F F ' -e=0 -w=30 -i=0 --arrows=0.2 --arrow-offset=0.1 --letters=0.35 -l --zoom=0.7
%% zrender -d=12 -a='_(1,A---B---F---D)' -m='A A  B B  C C  D D  E E  F F ' -e=0 -w=30 -i=0 --arrows=0.2 --arrow-offset=0.1 --letters=0.35 -l --zoom=0.7
%% zrender -d=12 -a='_(3,C--E--)' -m='A A  B B  C C  D D  E E  F F ' -e=0 -w=30 -i=0 --arrows=0.2 --arrow-offset=0.1 --letters=0.5 -l --zoom=0.9 -r=i2
%%
\begin{center}
\fbox{\includegraphics*[width=80mm, viewport={0 447 595 802}]{3446-3464-grid-graph.pdf}}%
\hspace*{5mm}% layout
\begin{subfigure}[b]{15mm}
{\includegraphics*[width=15mm, viewport={0 247 595 852}]{3446-3464-grid-graph-prototile-A6.pdf}}
{\includegraphics*[width=15mm, viewport={0 247 595 852}]{3446-3464-grid-graph-prototile-BCD.pdf}}
{\includegraphics*[width=15mm, viewport={0 247 595 852}]{3446-3464-grid-graph-prototile-EFEF.pdf}}
\end{subfigure}
\hspace*{5mm}% layout
\begin{subfigure}[b]{15mm}
{\includegraphics*[width=15mm, viewport={0 247 595 852}]{3446-3464-grid-graph-prototile-ABFD.pdf}}
{\includegraphics*[width=15mm, viewport={0 247 595 852}]{3446-3464-grid-graph-prototile-CECE.pdf}}
\end{subfigure}
\end{center}
\caption{\label{fig:3446-3464-grid-graph-repeat}
Grid-graph for the $(3.4.4.6; 3.4.6.4)$-grid (left)
and its CCW (middle) and CW (right) prototiles.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3446-3464-grid-graph.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -a='_(6,@@A++)' -m='A A---B++++C++++D---A++A---B---F+++E+++F---D---A---B++++C--E--C--E--C++++D++++B---F+++E+++F---D---A---B++++C++++D---A++A  B B  C C  D D  E E  F F---D++++B---F+++E--C--E+++F ' -e=0 -w=10 -i=0 --arrows=0.15 --arrow-offset=0.1 --letters=0.45 --zoom=2.7 -l
%%
%% zrender -d=12 -a='_(6,A++)' -m='A A  B B  C C  D D  E E  F F ' -e=0 -w=30 -i=0 --arrows=0.2 --arrow-offset=0.1 --letters=0.6 -l --zoom=0.9
%% zrender -d=12 -a='_(1,B++++C++++D)' -m='A A  B B  C C  D D  E E  F F ' -e=0 -w=30 -i=0 --arrows=0.2 --arrow-offset=0.1 --letters=0.35 -l --zoom=0.8
%% zrender -d=12 -a='_(2,E+++F+++)' -m='A A  B B  C C  D D  E E  F F ' -e=0 -w=30 -i=0 --arrows=0.2 --arrow-offset=0.1 --letters=0.35 -l --zoom=0.7
%% zrender -d=12 -a='_(1,A---B---F---D)' -m='A A  B B  C C  D D  E E  F F ' -e=0 -w=30 -i=0 --arrows=0.2 --arrow-offset=0.1 --letters=0.35 -l --zoom=0.7
%% zrender -d=12 -a='_(3,C--E--)' -m='A A  B B  C C  D D  E E  F F ' -e=0 -w=30 -i=0 --arrows=0.2 --arrow-offset=0.1 --letters=0.5 -l --zoom=0.9 -r=i2
%%
\begin{center}
\fbox{\includegraphics*[width=80mm, viewport={0 447 595 802}]{3446-3464-grid-graph.pdf}}%
\hspace*{5mm}% layout
\begin{subfigure}[b]{15mm}
{\includegraphics*[width=15mm, viewport={0 247 595 852}]{3446-3464-grid-graph-prototile-A6.pdf}}
{\includegraphics*[width=15mm, viewport={0 247 595 852}]{3446-3464-grid-graph-prototile-BCD.pdf}}
{\includegraphics*[width=15mm, viewport={0 247 595 852}]{3446-3464-grid-graph-prototile-EFEF.pdf}}
\end{subfigure}
\hspace*{5mm}% layout
\begin{subfigure}[b]{15mm}
{\includegraphics*[width=15mm, viewport={0 247 595 852}]{3446-3464-grid-graph-prototile-ABFD.pdf}}
{\includegraphics*[width=15mm, viewport={0 247 595 852}]{3446-3464-grid-graph-prototile-CECE.pdf}}
\end{subfigure}
\end{center}
\caption{\label{fig:3446-3464-grid-graph}
The $(3.4.4.6; 3.4.6.4)$-grid (left)
and its CCW (middle)
and CW (right) prototiles.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3446-3464-grid-mod-180deg.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%% zrender -d=12 -a='(6,A++)' --const-maps -T='A++A,A---B,B++++C,B---F,C++++D,C--E,D++++B,D---A,E+++F,E--C,F+++E,F---D' -e=0 -w=10 -A=0.2,0.1 -L=0.4 --colors-pick='1,6' --fancy-print-maps --no-text --zoom=2 -k=+6 --grid=20 -r=-30 --shift-y=-0.11
%%
%%
\begin{center}
%
\fbox{\includegraphics*[width=90mm, viewport={0 460 595 842}]{3446-3464-grid-mod-180deg.pdf}}%
\hspace*{0mm}% layout
%
\end{center}
\caption{\label{fig:3446-3464-grid-mod-180deg}
Grid with edges colored by rotation modulo 180 degrees.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3446-3464-r31-var0-motifs.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%  zrender -d=12 -a=':A:' -@=1 -m='A ABCDAABFEFDABCECECDBFEFDABCECDBFDBFDBCEFDBCECEFDABCDA  B BFEFDBFECECECDBFDAAAABCDAAB  C CEFDABCEFEFDAABCDAAABFEC  D DBFDAAAAAABFDBCECECEFEFD  E ECDABFECDBFDBFEFDBCECECDABCDAABFDBFE  F FECECECDBFEFDABCDABFEF ' -T='A++A,A---B,B++++C,B---F,C++++D,C--E,D++++B,D---A,E+++F,E--C,F+++E,F---D' -e=0.15 -w=15 -i=0 --colors-pick='1,12' --fancy-print-maps -l -A=0.2,0.1 -L=0.5
%%
%%
\begin{center}
%
{\includegraphics*[width=40mm, viewport={0 247 595 802}]{3446-3464-r31-var0-motifs-A.pdf}}%
{\includegraphics*[width=40mm, viewport={0 247 595 802}]{3446-3464-r31-var0-motifs-B.pdf}}%
{\includegraphics*[width=40mm, viewport={0 247 595 802}]{3446-3464-r31-var0-motifs-C.pdf}}%
\hspace*{0mm}% layout
%

{\includegraphics*[width=40mm, viewport={0 277 595 802}]{3446-3464-r31-var0-motifs-D.pdf}}%
{\includegraphics*[width=40mm, viewport={0 277 595 802}]{3446-3464-r31-var0-motifs-E.pdf}}%
{\includegraphics*[width=40mm, viewport={0 277 595 802}]{3446-3464-r31-var0-motifs-F.pdf}}%
%
\begin{subfigure}[b]{20mm}
%\fbox{\includegraphics*[width=20mm, viewport={0 247 595 842}]{3446-3464-r31-var0-motifs.pdf}}
%\fbox{\includegraphics*[width=20mm, viewport={0 247 595 842}]{3446-3464-r31-var0-motifs.pdf}}
\end{subfigure}
%
\end{center}
\caption{\label{fig:3446-3464-r31-var0-motifs}
Top to bottom, left to right:
motifs of
\texttt{A},
\texttt{B},
\texttt{C},
\texttt{D},
\texttt{E}, and
\texttt{F}.
Start and end marked for each curve.
Coloring by letters.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3446-3464-r31-var0-tiles-minus-2.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-3446-3464.txt
%%
%%
%% zrender -d=12 -a='(1,A---B---F---D)' -@=1  -m='A ABCDAABFEFDABCECECDBFEFDABCECDBFDBFDBCEFDBCECEFDABCDA  B BFEFDBFECECECDBFDAAAABCDAAB  C CEFDABCEFEFDAABCDAAABFEC  D DBFDAAAAAABFDBCECECEFEFD  E ECDABFECDBFDBFEFDBCECECDABCDAABFDBFE  F FECECECDBFEFDABCDABFEF ' -T='A++A,A---B,B++++C,B---F,C++++D,C--E,D++++B,D---A,E+++F,E--C,F+++E,F---D' -e=0.1 -w=10 -i=0 --colors-pick='1,6' --fancy-print-maps  -l='ABFD,CE' -A=0.2,0.1 -L=0.5 -k=+6 -r=-30
%%
%% zrender -d=12 -a='+++(3,C--E--)' -@=1  -m='A ABCDAABFEFDABCECECDBFEFDABCECDBFDBFDBCEFDBCECEFDABCDA  B BFEFDBFECECECDBFDAAAABCDAAB  C CEFDABCEFEFDAABCDAAABFEC  D DBFDAAAAAABFDBCECECEFEFD  E ECDABFECDBFDBFEFDBCECECDABCDAABFDBFE  F FECECECDBFEFDABCDABFEF ' -T='A++A,A---B,B++++C,B---F,C++++D,C--E,D++++B,D---A,E+++F,E--C,F+++E,F---D' -e=0.1 -w=10 -i=0 --colors-pick='1,6' --fancy-print-maps -l='ABFD,CE' -A=0.2,0.1 -L=0.5 -k=+6 -r=-30
%%
%%
%% zrender -d=12 -a='(1,A---B---F---D)' -@=1  -m='A ABCDAABFEFDABCECECDBFEFDABCECDBFDBFDBCEFDBCECEFDABCDA  B BFEFDBFECECECDBFDAAAABCDAAB  C CEFDABCEFEFDAABCDAAABFEC  D DBFDAAAAAABFDBCECECEFEFD  E ECDABFECDBFDBFEFDBCECECDABCDAABFDBFE  F FECECECDBFEFDABCDABFEF ' -T='A++A,A---B,B++++C,B---F,C++++D,C--E,D++++B,D---A,E+++F,E--C,F+++E,F---D' -e=0 -w=3 -i=2 --colors-pick='1,6' --fancy-print-maps -J='A,6,4;B,3,4;C,3,6;D,3,4;E,4,6;F,4,4;'  -l='ABFD,CE' -k=+6 -r=-20
%%
%% zrender -d=12 -a='+++(3,C--E--)' -@=1  -m='A ABCDAABFEFDABCECECDBFEFDABCECDBFDBFDBCEFDBCECEFDABCDA  B BFEFDBFECECECDBFDAAAABCDAAB  C CEFDABCEFEFDAABCDAAABFEC  D DBFDAAAAAABFDBCECECEFEFD  E ECDABFECDBFDBFEFDBCECECDABCDAABFDBFE  F FECECECDBFEFDABCDABFEF ' -T='A++A,A---B,B++++C,B---F,C++++D,C--E,D++++B,D---A,E+++F,E--C,F+++E,F---D' -e=0 -w=3 -i=2 --colors-pick='1,6' --fancy-print-maps -J='A,6,4;B,3,4;C,3,6;D,3,4;E,4,6;F,4,4;'  -l='ABFD,CE' -k=+6 -r=-20
%%
%%
\begin{center}
%
{\includegraphics*[width=59mm, viewport={70 260 595 810}]{3446-3464-r31-var0-tiles-minus-2-ABFD-lines.pdf}}%
{\includegraphics*[width=64mm, viewport={40 260 595 790}]{3446-3464-r31-var0-tiles-minus-2-CE3-lines.pdf}}
%
%\hspace*{0mm}% layout
{\includegraphics*[width=59mm, viewport={30 255 555 815}]{3446-3464-r31-var0-tiles-minus-2-ABFD-solid.pdf}}%
%\hspace*{20mm}% layout
{\includegraphics*[width=64mm, viewport={28 270 570 798}]{3446-3464-r31-var0-tiles-minus-2-CE3-solid.pdf}}
%
%\begin{subfigure}[b]{20mm}
%\end{subfigure}
%
\end{center}
\caption{\label{fig:3446-3464-r31-var0-tiles-minus-2}
First iterates of the CW prototiles
\tileS{A---B---F---D---}{1} (top left) and
\tileS{C--E--}{3} (to right).
Third iterates of the same at the bottom.
Coloring by orientation modulo 180 degrees.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3446-3464-r31-var0-tiles-plus.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-3446-3464.txt
%%
%% zrender -d=12 -a='(6,A++)' -@=1 -m='A ABCDAABFEFDABCECECDBFEFDABCECDBFDBFDBCEFDBCECEFDABCDA  B BFEFDBFECECECDBFDAAAABCDAAB  C CEFDABCEFEFDAABCDAAABFEC  D DBFDAAAAAABFDBCECECEFEFD  E ECDABFECDBFDBFEFDBCECECDABCDAABFDBFE  F FECECECDBFEFDABCDABFEF ' -T='A++A,A---B,B++++C,B---F,C++++D,C--E,D++++B,D---A,E+++F,E--C,F+++E,F---D' -e=0.15 -w=10 -i=0 --colors-pick='1,12' --fancy-print-maps -l='A,BCD,EF' -A=0.2,0.1 -L=0.5
%%
%% zrender -d=12 -a='(6,A++)' -@=1 -m='A ABCDAABFEFDABCECECDBFEFDABCECDBFDBFDBCEFDBCECEFDABCDA  B BFEFDBFECECECDBFDAAAABCDAAB  C CEFDABCEFEFDAABCDAAABFEC  D DBFDAAAAAABFDBCECECEFEFD  E ECDABFECDBFDBFEFDBCECECDABCDAABFDBFE  F FECECECDBFEFDABCDABFEF ' -T='A++A,A---B,B++++C,B---F,C++++D,C--E,D++++B,D---A,E+++F,E--C,F+++E,F---D' -e=0 -w=3 -i=2  --colors-pick='1,12' --fancy-print-maps -J='A,6,4;B,3,4;C,3,6;D,3,4;E,4,6;F,4,4;' -l='A,BCD,EF'
%%
%%
%% zrender -d=12 -a='---(1,B++++C++++D)' -@=1 -m='A ABCDAABFEFDABCECECDBFEFDABCECDBFDBFDBCEFDBCECEFDABCDA  B BFEFDBFECECECDBFDAAAABCDAAB  C CEFDABCEFEFDAABCDAAABFEC  D DBFDAAAAAABFDBCECECEFEFD  E ECDABFECDBFDBFEFDBCECECDABCDAABFDBFE  F FECECECDBFEFDABCDABFEF ' -T='A++A,A---B,B++++C,B---F,C++++D,C--E,D++++B,D---A,E+++F,E--C,F+++E,F---D' -e=0.15 -w=15 -i=0 --colors-pick='1,12' --fancy-print-maps -l='A,BCD,EF' -A=0.2,0.1 -L=0.5
%%
%% zrender -d=12 -a='---(1,B++++C++++D)' -@=1 -m='A ABCDAABFEFDABCECECDBFEFDABCECDBFDBFDBCEFDBCECEFDABCDA  B BFEFDBFECECECDBFDAAAABCDAAB  C CEFDABCEFEFDAABCDAAABFEC  D DBFDAAAAAABFDBCECECEFEFD  E ECDABFECDBFDBFEFDBCECECDABCDAABFDBFE  F FECECECDBFEFDABCDABFEF ' -T='A++A,A---B,B++++C,B---F,C++++D,C--E,D++++B,D---A,E+++F,E--C,F+++E,F---D' -e=0 -w=3 -i=2  --colors-pick='1,12' --fancy-print-maps -J='A,6,4;B,3,4;C,3,6;D,3,4;E,4,6;F,4,4;' -l='A,BCD,EF'
%%
%%
%% zrender -d=12 -a='+++(2,E+++F+++)' -@=1 -m='A ABCDAABFEFDABCECECDBFEFDABCECDBFDBFDBCEFDBCECEFDABCDA  B BFEFDBFECECECDBFDAAAABCDAAB  C CEFDABCEFEFDAABCDAAABFEC  D DBFDAAAAAABFDBCECECEFEFD  E ECDABFECDBFDBFEFDBCECECDABCDAABFDBFE  F FECECECDBFEFDABCDABFEF ' -T='A++A,A---B,B++++C,B---F,C++++D,C--E,D++++B,D---A,E+++F,E--C,F+++E,F---D' -e=0.15 -w=10 -i=0 --colors-pick='1,12' --fancy-print-maps -l='A,BCD,EF' -A=0.2,0.1 -L=0.5
%%
%% zrender -d=12 -a='+++(2,E+++F+++)' -@=1 -m='A ABCDAABFEFDABCECECDBFEFDABCECDBFDBFDBCEFDBCECEFDABCDA  B BFEFDBFECECECDBFDAAAABCDAAB  C CEFDABCEFEFDAABCDAAABFEC  D DBFDAAAAAABFDBCECECEFEFD  E ECDABFECDBFDBFEFDBCECECDABCDAABFDBFE  F FECECECDBFEFDABCDABFEF ' -T='A++A,A---B,B++++C,B---F,C++++D,C--E,D++++B,D---A,E+++F,E--C,F+++E,F---D' -e=0 -w=3 -i=2  --colors-pick='1,12' --fancy-print-maps -J='A,6,4;B,3,4;C,3,6;D,3,4;E,4,6;F,4,4;' -l='A,BCD,EF'
%%
%%
%%
\begin{center}
%
{\includegraphics*[width=64.5mm, viewport={0 267 595 792}]{3446-3464-r31-var0-tiles-plus-A6-lines.pdf}}%
%\hspace*{0mm}% layout
{\includegraphics*[width=64.5mm, viewport={0 267 595 792}]{3446-3464-r31-var0-tiles-plus-A6-solid.pdf}}
%
{\includegraphics*[width=44.5mm, viewport={0 247 595 842}]{3446-3464-r31-var0-tiles-plus-BCD-lines.pdf}}%
\hspace*{20mm}% layout
{\includegraphics*[width=44.5mm, viewport={0 247 595 842}]{3446-3464-r31-var0-tiles-plus-BCD-solid.pdf}}
%
{\includegraphics*[width=64.5mm, viewport={0 322 595 762}]{3446-3464-r31-var0-tiles-plus-EF2-lines.pdf}}%
%\hspace*{0mm}% layout
{\includegraphics*[width=64.5mm, viewport={0 322 595 762}]{3446-3464-r31-var0-tiles-plus-EF2-solid.pdf}}
%
%\begin{subfigure}[b]{20mm}
%\end{subfigure}
%
\end{center}
\caption{\label{fig:3446-3464-r31-var0-tiles-plus}
Mutual self-similarity of the CCW prototiles
\tileS{A++}{6} (top, small copies blue),
\tileS{B++++C++++D++++}{1} (middle, small copies red), and
\tileS{E+++F+++}{2} (bottom, small copies green).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-curve-r39-hex-var1-tiles-plus.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-3464.txt
%%
%% zrender -d=12 -m='A AABAAAAAABBABBABBABAAAABBBABAABBAAAAAABA   B BBAAABABBABBBABBBAB,BBAAABABBABBBABBBAB ' -T='A++A,B++++B,A---B,B---A' -e=0.1 -w=2 -a='(6,A++)' -k=-12 -i=1 -@=1 -J -l=',A,B'
%%
%% zrender -d=12 -m='A AABAAAAAABBABBABBABAAAABBBABAABBAAAAAABA   B BBAAABABBABBBABBBAB,BBAAABABBABBBABBBAB ' -T='A++A,B++++B,A---B,B---A' -e=0.1 -w=2 -a='(3,B++++)' -k=-12 -i=1 -@=1 -J -l=',A,B'
%%
\begin{center}
%
{\includegraphics*[width=79mm, viewport={0 287 595 782}]{3464-curve-r39-hex-var1-tiles-plus-A6.pdf}}%
\begin{subfigure}[b]{50.5mm}
{\includegraphics*[width=50mm, viewport={0 247 595 842}]{3464-curve-r39-hex-var1-tiles-plus-B3.pdf}}%
\vspace*{5mm}% V
\end{subfigure}%
%\hspace*{0mm}% layout
%
\end{center}
\caption{\label{fig:3464-curve-r39-hex-var1-tiles-plus}
Mutual self-similarity of the prototiles
\tileS{A}{6} (left, small copies blue) and
\tileS{B}{3} (right, small copies red)
of a curve-set of order 39.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-curve-r9-var1-koch-tiles-decomp.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
% VARIANT 1: R9-var-1
%%
%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0 -w=6 -a='(6,@A++)' -l -i=3 --colors-pick=1,2 -J='A,6,4;B,3,4;'
%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0 -w=8 -a='(3,@B++++)' -l -i=3 -r=+90 --zoom=0.8 --colors-pick=1,2 -J='A,6,4;B,3,4;'
%
\begin{center}
{\includegraphics*[width=60mm, viewport={0 255 595 820}]{3464-curve-r9-var1-koch-tiles-decomp-A.pdf}}%
\hspace*{3mm}% layout
{\includegraphics*[width=60mm, viewport={0 255 595 820}]{3464-curve-r9-var1-koch-tiles-decomp-B.pdf}}%
\end{center}
\caption{\label{fig:3464-curve-r9-var1-koch-tiles-decomp}
%
Mutual self-similarity of the prototiles \tileS{A++}{6} (left, small copies blue)
and \tileS{B++++}{3} (right, small copies red).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% alternatively:
%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0 -w=6 -a='(6,@A++)' -k=+2 -i=3
%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0 -w=8 -a='---(3,@B++++)' -k=+2 -i=3 --zoom=0.8


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-curve-r9-var1-koch-tiles.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
% VARIANT 1: R9-var-1
%%
%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0 -w=6 -a='(6,A++)'  -k=-12 -i=4 -J='A,6,4;B,3,4;'
%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0 -w=8 -a='---(3,B++++)' -k=-12 -i=4 --zoom=0.8 -J='A,6,4;B,3,4;'
%%
\begin{center}
{\includegraphics*[width=60mm, viewport={0 255 595 820}]{3464-curve-r9-var1-koch-tiles-A.pdf}}%
\hspace*{3mm}% layout
{\includegraphics*[width=60mm, viewport={0 255 595 820}]{3464-curve-r9-var1-koch-tiles-B.pdf}}%
\end{center}
\caption{\label{fig:3464-curve-r9-var1-koch-tiles}
%
Fourth iterates of the prototiles \tileS{A++}{6} (left) and \tileS{B++++}{3} (right).
Coloring by curves and their orientations.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-curve-r9-var1-motifs.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% VARIANT 1: R9-var-1
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0.1 -w=20 -a=A++A++A++A++A---B---A---B++++B---A  -k=-12 -i=0 --arrows=0.15 --letters=0.4
%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0.1 -w=20 -a=---B++++B---A---B++++B++++B---A---B  -k=-12 -i=0 --arrows=0.15 --letters=0.4 --zoom=0.9
%
%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0.1 -w=15 -a=A++A++A++A++A++A  -k=-12 -i=1 --arrows=0.2
%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0.1 -w=15 -a=---B++++B++++B -k=-12 -i=1 --arrows=0.2 --zoom=0.8
%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0.1 -w=15 -a=A---B---A---B -k=-12 -i=1 --arrows=0.2 --zoom=0.9
\begin{center}
{\includegraphics*[width=25mm, viewport={0 247 595 842}]{3464-curve-r9-var1-motif-A.pdf}}%
\hspace*{0mm}% layout
{\includegraphics*[width=25mm, viewport={0 247 595 842}]{3464-curve-r9-var1-motif-B.pdf}}%
%%
\hspace*{2mm}% layout
%\fbox{\includegraphics*[width=30mm, viewport={0 237 595 842}]{3464-curve-r9-var1-prototile-A6.pdf}}%
{\includegraphics*[width=27mm, viewport={0 237 595 842}]{3464-curve-r9-var1-prototile-A6.pdf}}%
\hspace*{0mm}% layout
%\fbox{\includegraphics*[width=25mm, viewport={0 210 595 842}]{3464-curve-r9-var1-prototile-B3.pdf}}%
{\includegraphics*[width=22mm, viewport={0 210 595 842}]{3464-curve-r9-var1-prototile-B3.pdf}}%
\hspace*{0mm}% layout
%\fbox{\includegraphics*[width=30mm, viewport={0 247 595 842}]{3464-curve-r9-var1-prototile-ABAB.pdf}}%
{\includegraphics*[width=27mm, viewport={30 247 565 842}]{3464-curve-r9-var1-prototile-ABAB.pdf}}%

\end{center}
\caption{\label{fig:3464-curve-r9-var1-motifs}
%
From left to right: motifs for the letter \texttt{A} and \texttt{B}, and
first iterates for prototiles \tileS{A++}{6}, \tileS{B++++}{3}, and \tileS{A---B---}{2}
of a curve on the $(3.4.6.4)$-grid.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-curve-r9-var1-tile-minus.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
% VARIANT 1: R9-var-1
%%
%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0 -w=8 -a='(6,A---B---)' -k=-12 -i=4 -J='A,6,4;B,3,4;'
%%
%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0 -w=8 -a='(3,@A---@B---)' -k=+3 -i=3 -J='A,6,4;B,3,4;'
%%
\begin{center}
{\includegraphics*[width=60mm, viewport={0 267 595 802}]{3464-curve-r9-var1-tile-minus.pdf}}%
\hspace*{3mm}% layout
{\includegraphics*[width=60mm, viewport={0 267 595 802}]{3464-curve-r9-var1-tile-minus-decomp.pdf}}%
\end{center}
\caption{\label{fig:3464-curve-r9-var1-tile-minus}
%
Fourth iterate of the prototile \tileS{A---B---}{2}
(left, coloring by orientation of curves contained)
and
its self-similarity
(right, coloring by orientation of small copies of itself).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-degenerate-curve-A-const-decomp.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -m='A A  B B---A++A++A++A++A---B---A---B++++B++++B---A---B++++B---A---B++++B ' -e=0 -w=3 -a='---@B' -k=12 --colors-pick='2,-12' -i=4 -r=+90 -J='A,6,4;B,3,4;'
%%
\begin{center}
%\fbox{\includegraphics*[width=70mm, viewport={0 300 595 752}]{3464-degenerate-curve-B-decomp.pdf}}%
{\includegraphics*[width=125mm, viewport={20 455 575 620}]{3464-degenerate-curve-A-const-decomp.pdf}}%
\end{center}
\caption{\label{fig:3464-degenerate-curve-A-const-decomp}
Self-similarity of curve \texttt{B},
coloring by orientation of the smaller curves.
The prototile \tileS{B++++}{3} is the apparent triangle in the center.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%% zrender -d=12 -m='A A  B B---A++A++A++A++A---B---A---B++++B++++B---A---B++++B---A---B++++B ' -e=0 -w=3 -a='---@B' -k=-12 -i=4 -r=+90 -J='A,6,4;B,3,4;'
%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-degenerate-curve-A-const-motif.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -m='A A  B B---A++A++A++A++A---B---A---B++++B++++B---A---B++++B---A---B++++B ' -e=0 -w=13 -a='~~~@B' -k=12 --colors-pick='2,-12' -i=0 -A=0.3 -L=0.4 -e=0.15
%% zrender -d=12 -m='A A  B B---A++A++A++A++A---B---A---B++++B++++B---A---B++++B---A---B++++B ' -e=0 -w=5 -a='~~~@B' -k=12 --colors-pick='2,-12' -i=1 -A=0.3 -e=0.15
%%
\begin{center}
%
{\includegraphics*[width=40mm, viewport={60 427 525 652}]{3464-degenerate-curve-A-const-motif.pdf}}%
\hspace*{3mm}% layout
{\includegraphics*[width=85mm, viewport={30 445 565 627}]{3464-degenerate-curve-A-const-motif-it2.pdf}}%
%
\end{center}
\caption{\label{fig:3464-degenerate-curve-A-const-motif}
%
First (left) and second (right) iterate of the curve \texttt{B}
of a curve-set with \texttt{A} constant.
Coloring by orientation of the edges of the first iterate.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-degenerate-curve-B-const-decomp.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -m='A A++A---B++++B---A++A++A---B---A---B++++B---A---B++++B++++B---A++A---B---A---B++++B++++B---A---B++++B++++B---A---B---A++A++A++A++A++A---B++++B---A  B B ' -e=0 -w=8 -a='(1,@A++)' -k=-12 -i=3 -r=26 -J='A,6,4;B,3,4;'
%%
%%
\begin{center}
%{\includegraphics*[width=70mm, viewport={20 287 575 760}]{3464-degenerate-curve-B-const-decomp.pdf}}%
{\includegraphics*[width=80mm, viewport={20 310 575 760}]{3464-degenerate-curve-B-const-decomp.pdf}}%
\end{center}
%\begin{center}
%%{\includegraphics*[width=70mm, viewport={20 287 575 760}]{3464-degenerate-curve-B-const-decomp.pdf}}%
%{\includegraphics*[width=70mm, viewport={20 287 575 760}]{3464-degenerate-curve-B-const-decomp.pdf}}%
%{\includegraphics*[width=60mm, viewport={20 247 575 820}]{3464-degenerate-curve-B-const-star.pdf}}%
%\end{center}
\caption{\label{fig:3464-degenerate-curve-B-const-decomp}
%
Decomposition of the curve \texttt{A} into 19 smaller copies of itself,
showing its self-similarity.
Coloring by orientation of the small copies.\IMAGENAME%
% (left)
%and the prototile \tileS{A++}{6} (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%% zrender -d=12 -m='A A++A---B++++B++++B---A---B++++B---A---B---A++A++A  B B ' -e=0 -w=3 -a='@A' -k=-12 -i=4



%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-degenerate-curve-B-const-motif.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -m='A A++A---B++++B---A++A++A---B---A---B++++B---A---B++++B++++B---A++A---B---A---B++++B++++B---A---B++++B++++B---A---B---A++A++A++A++A++A---B++++B---A  B B ' -e=0.15 -w=13 -a='(1,@A++)' -k=-12 -L=0.4 -A=0.3 -i=0
%%
%% zrender -d=12 -m='A A++A---B++++B---A++A++A---B---A---B++++B---A---B++++B++++B---A++A---B---A---B++++B++++B---A---B++++B++++B---A---B---A++A++A++A++A++A---B++++B---A  B B ' -e=0.2 -w=5 -a='(1,@A++)' -k=-12 -A=0.3 -i=1
%%
\begin{center}
%
{\includegraphics*[width=40mm, viewport={120 230 500 785}]{3464-degenerate-curve-B-const-motif.pdf}}%
\hspace*{5mm}% layout
{\includegraphics*[width=55mm, viewport={55 260 535 812}]{3464-degenerate-curve-B-const-motif-it2.pdf}}%
%
\end{center}
\caption{\label{fig:3464-degenerate-curve-B-const-motif}
%
First (left) and second (right) iterate of the curve \texttt{A}
of a curve-set with \texttt{B} constant.
Coloring by orientation of the edges of the first iterate.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-fhg-grid-graph.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-rotational-3464
%%
%% zrender -d=12 -m='F FGHFGgGgfF  f fhHhgfFf  G GHFGHhHhgG  g gfFfhgGg  H HFGHFfFfhH  h hgGgfhHh' -T='F++G,G++H,H++F,f++++h,h++++g,g++++f,F---f,f---F,G---g,g---G,H---h,h---H' -e=0 -A --arrow-offset=0.1 -L=0.4 -w=10 -a='(2,F++G++H++)' --colors-pick=1,6 -l -i=0 -@=2 --zoom=2.1
%%
%% zrender -d=12 -m='F FGHFGgGgfF  f fhHhgfFf  G GHFGHhHhgG  g gfFfhgGg  H HFGHFfFfhH  h hgGgfhHh' -T='F++G,G++H,H++F,f++++h,h++++g,g++++f,F---f,f---F,G---g,g---G,H---h,h---H' -e=0 -A --arrow-offset=0.1 -L=0.4 -w=10 -a='(2,F++G++H++)' -l=',Ff,Gg,Hh' -i=0 -@=2 --zoom=2.1
%%
%%
\begin{center}
%
\hspace*{0mm}% layout
\fbox{\includegraphics*[width=64mm, viewport={0 247 595 542}]{3464-fhg-grid-graph.pdf}}%
\hspace*{1mm}% layout
\fbox{\includegraphics*[width=64mm, viewport={0 247 595 542}]{3464-fhg-grid-graph-idea.pdf}}%
%
%\begin{subfigure}[b]{21mm}
%\fbox{\includegraphics*[width=20mm, viewport={0 247 595 842}]{3464-fhg-grid-graph.pdf}}
%\vspace*{12mm}% V
%\end{subfigure}
%%
%\begin{subfigure}[b]{20mm}
%\fbox{\includegraphics*[width=20mm, viewport={0 247 595 842}]{3464-fhg-grid-graph.pdf}}
%\fbox{\includegraphics*[width=20mm, viewport={0 247 595 842}]{3464-fhg-grid-graph.pdf}}
%\end{subfigure}
%
\end{center}
\caption{\label{fig:3464-fhg-grid-graph}
%
Coloring using six colors (left).
The three CW prototiles have 2-fold rotational symmetry,
each is drawn in one color on the right.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-fhg-r9-var0-tile-minus-decomp.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file: 00lsys-rotational-3464
%%
%% name = r9-FGH-var0
%% zrender -d=12 -m='F FGHFGgfFfFGgfF  f fhHhgfFf  G GHFGHhHhgG  g gfFfhgGg  H HFGHhH  h hgGgfhHh' -T='F++G,G++H,H++F,f++++h,h++++g,g++++f,F---f,f---F,G---g,g---G,H---h,h---H' -e=0.1 -w=2 -a='(2,F---f---)' -l=',Ff,Gg,Hh' -i=3 -@=1 -J -B=3,0.8 -r=i0
%% zrender -d=12 -m='F FGHFGgfFfFGgfF  f fhHhgfFf  G GHFGHhHhgG  g gfFfhgGg  H HFGHhH  h hgGgfhHh' -T='F++G,G++H,H++F,f++++h,h++++g,g++++f,F---f,f---F,G---g,g---G,H---h,h---H' -e=0.1 -w=2 -a='(2,G---g---)' -l=',Ff,Gg,Hh' -i=3 -@=1 -J -B=3,0.8 -r=i2
%% zrender -d=12 -m='F FGHFGgfFfFGgfF  f fhHhgfFf  G GHFGHhHhgG  g gfFfhgGg  H HFGHhH  h hgGgfhHh' -T='F++G,G++H,H++F,f++++h,h++++g,g++++f,F---f,f---F,G---g,g---G,H---h,h---H' -e=0.1 -w=2 -a='(2,H---h---)' -l=',Ff,Gg,Hh' -i=3 -@=1 -J -B=3,0.8 -r=i4
%%
%%
\begin{center}
%
{\includegraphics*[width=55mm, viewport={0 310 595 760}]{3464-fhg-r9-var0-tile-minus-decomp-FfFf.pdf}}%
%
\begin{subfigure}[b]{38.5mm}
{\includegraphics*[width=38mm, viewport={0 247 595 842}]{3464-fhg-r9-var0-tile-minus-decomp-GgGg.pdf}}%
\vspace*{2mm}% V
\end{subfigure}%
%
\begin{subfigure}[b]{31.5mm}
{\includegraphics*[width=31mm, viewport={0 247 595 842}]{3464-fhg-r9-var0-tile-minus-decomp-HhHh.pdf}}%
\vspace*{5mm}% V
\end{subfigure}
%
\end{center}
\caption{\label{fig:3464-fhg-r9-var0-tile-minus-decomp}
%
Mutual self-similarity of the CW prototiles
\tileS{F---f---}{2} (left, small copies blue),
\tileS{G---g---}{2} (middle, small copies red), and
\tileS{H---h---}{2} (right, small copies green).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-ju-r19-a-curves-decomp.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -m='A AAAABABBBAAAABABBABBABBBA B BAAABBBABAABB' -T='A++A,B++++B,A---B,B---A' -e=0 -w=1 -a='@A' -i=3 -k=-12 --comment='ju-R19-a' -J='A,6,4;B,3,4;'
%% zrender -d=12 -m='A AAAABABBBAAAABABBABBABBBA B BAAABBBABAABB' -T='A++A,B++++B,A---B,B---A' -e=0 -w=1 -a='---@B' -i=3 -k=-12 --comment='ju-R19-a' -J='A,6,4;B,3,4;'
%%
%%% matheart image:
%%% zrender -d=12 -m='A AAAABABBBAAAABABBABBABBBA B BAAABBBABAABB' -T='A++A,B++++B,A---B,B---A' -e=0 -w=1 -a='A---B---A---B' -i=0 -@=1 -k=+3 --comment='ju-R19' -J='A,6,4;B,3,4;'
%%
\begin{center}
%
{\includegraphics*[width=69.5mm, viewport={20 310 575 760}]{3464-ju19-curve-a-decomp.pdf}}%
\hspace*{5mm}% layout
\begin{subfigure}[b]{54mm}
{\includegraphics*[width=53.5mm, viewport={0 247 595 822}]{3464-ju19-curve-b-decomp.pdf}}%
\vspace*{3mm}% V
\end{subfigure}

%
\end{center}
\caption{\label{fig:3464-ju-r19-a-curves-decomp}
Fourth iterates of the curve-set, for \texttt{A} (left) and \texttt{B} (right).
Coloring by orientation of the curves.\IMAGENAME%
%The small copies of \texttt{B} are blue and green.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-ju-r19-a-curves-it1.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -m='A AAAABABBBAAAABABBABBABBBA B BAAABBBABAABB' -T='A++A,B++++B,A---B,B---A' -e=0 -w=1 -a='@A' -l -w=15 -e=0.1 -i=0 --colors-pick='1,2' --comment='ju-R19-a' --arrows=0.15 --letters=0.4
%%
%% zrender -d=12 -m='A AAAABABBBAAAABABBABBABBBA B BAAABBBABAABB' -T='A++A,B++++B,A---B,B---A' -e=0 -w=1 -a='@B' -l -w=15 -e=0.1 -i=0 --colors-pick='1,2' --comment='ju-R19-a' --arrows=0.15 --letters=0.4
%%
\begin{center}
%
{\includegraphics*[width=45mm, viewport={0 247 595 842}]{3464-ju19-curve-a-it1.pdf}}%
\hspace*{7mm}% layout
{\includegraphics*[width=45mm, viewport={0 300 595 842}]{3464-ju19-curve-b-it1.pdf}}%
%
\end{center}
\caption{\label{fig:3464-ju-r19-a-curves-it1}
First iterates (motifs) of a curve-set on the $(3.4.6.4)$-grid.
Motif for \texttt{A} (left) and for \texttt{B} (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-ju19-curve-prototile-minus.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -m='A AAAABABBBAAAABABBABBABBBA B BAAABBBABAABB' -T='A++A,B++++B,A---B,B---A' -e=0 -w=1 -a='(2,A---B---)' -w=10 -e=0.1 -@=0 -k=-12 -i=1 --comment='ju-R19-a' --arrows=0.15 -L=0.5
%% zrender -d=12 -m='A AAAABABBBAAAABABBABBABBBA B BAAABBBABAABB' -T='A++A,B++++B,A---B,B---A' -e=0 -w=1 -a='(6,A++)' -w=10 -e=0.1 -@=0 -k=-12 --comment='ju-R19-a' -a='(2,@A---B---)' -i=2 -a='(3,@A---@B---)' -k=+3 -J='A,6,4;B,3,4;'
%%
\begin{center}
%
{\includegraphics*[width=64.5mm, viewport={0 247 595 842}]{3464-ju19-curve-prototile-ABAB-it1.pdf}}%
\hspace*{0mm}% layout
%
{\includegraphics*[width=64.5mm, viewport={0 247 595 842}]{3464-ju19-curve-prototile-ABAB-decomp.pdf}}%
\hspace*{0mm}% layout
%
\end{center}
\caption{\label{fig:3464-ju19-curve-prototile-minus}
%
First iterate (left) and shape (right) of the CW prototile \tileS{A---B---}{2}.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-ju19-curve-prototiles-plus-decomp.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%%
%%
\begin{center}
%
{\includegraphics*[width=64.5mm, viewport={0 247 595 842}]{3464-ju19-curve-prototile-A-decomp.pdf}}%
\hspace*{0mm}% layout
%
{\includegraphics*[width=64.5mm, viewport={0 247 595 842}]{3464-ju19-curve-prototile-B-decomp.pdf}}%
\hspace*{0mm}% layout
%
\end{center}
\caption{\label{fig:3464-ju19-curve-prototiles-plus-decomp}
Shapes of the CCW prototiles \tileS{A++}{6} (left) and \tileS{B++++}{3} (right),
note the mutual self-similarity.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-ju19-curve-prototiles-plus-it1.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%%
%%
\begin{center}
%
{\includegraphics*[width=74.0mm, viewport={0 280 595 795}]{3464-ju19-curve-prototile-A6-it1.pdf}}%
\hspace*{0mm}% layout
%
{\includegraphics*[width=54.0mm, viewport={0 247 595 842}]{3464-ju19-curve-prototile-B3-it1.pdf}}%
\hspace*{0mm}% layout
%
%\fbox{\includegraphics*[width=44.0mm, viewport={0 247 595 842}]{3464-ju19-curve-prototile-ABAB-it1.pdf}}%
\hspace*{0mm}% layout
%
%\begin{subfigure}[b]{21mm}
%\fbox{\includegraphics*[width=20mm, viewport={0 247 595 842}]{XXX.pdf}}
%\vspace*{12mm}% V
%\end{subfigure}
%%
%\begin{subfigure}[b]{20mm}
%\fbox{\includegraphics*[width=20mm, viewport={0 247 595 842}]{XXX.pdf}}
%\fbox{\includegraphics*[width=20mm, viewport={0 247 595 842}]{XXX.pdf}}
%\end{subfigure}
%
\end{center}
\caption{\label{fig:3464-ju19-curve-prototiles-plus-it1}
First iterates of the prototiles \tileS{A++}{6} (left) and \tileS{B++++}{3} (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-ju19-curve-prototiles-plus-tiling.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%%
%%
\begin{center}
%
\fbox{\includegraphics*[width=90.0mm, viewport={0 547 595 842}]{3464-ju19-curve-prototiles-plus-tiling.pdf}}%
%
\end{center}
\caption{\label{fig:3464-ju19-curve-prototiles-plus-tiling}
%
Together, the two CCW prototiles tile the plane.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-r37-tile-plus-A6-decomp.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -m='A AAAABAAABBABAAABBAA  B BABBBABAAABBBABBBABBBABAABBBABBBABBBAABABBBAAABAAABAAAB ' -T='A++A,B++++B,A---B,B---A' -e=0 -w=2 -a='(6,A++)' -i=2 -@=1 -J -k=-12 -B
%% zrender -d=12 -m='A AAAABAAABBABAAABBAA  B BABBBABAAABBBABBBABBBABAABBBABBBABBBAABABBBAAABAAABAAAB ' -T='A++A,B++++B,A---B,B---A' -e=0 -w=2 -a='(6,A++)' -i=2 -@=1 -J -l=,A,B -B=1.5
%%
\begin{center}
%
{\includegraphics*[width=64.5mm, viewport={0 247 595 822}]{3464-r37-tile-plus-A6-decomp-1.pdf}}%
\hspace*{0mm}% layout
{\includegraphics*[width=64.5mm, viewport={0 247 595 822}]{3464-r37-tile-plus-A6-decomp-2.pdf}}%
%
\end{center}
\caption{\label{fig:3464-r37-tile-plus-A6-decomp}
%
Decomposition of the prototile \tileS{A++}{6} into smaller copies
of \tileS{A++}{6} and \tileS{B++++}{3}.
Coloring by orientation of curves (left)
and by tiles
(right, small copies of \tileS{A++}{6} blue,
 those of \tileS{B++++}{3} red).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-r37-tile-plus-B3-decomp.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -m='A AAAABAAABBABAAABBAA  B BABBBABAAABBBABBBABBBABAABBBABBBABBBAABABBBAAABAAABAAAB ' -T='A++A,B++++B,A---B,B---A' -e=0 -w=2 -a='(3,B++++)' -i=2 -@=1 -J -k=+12 -B
%% zrender -d=12 -m='A AAAABAAABBABAAABBAA  B BABBBABAAABBBABBBABBBABAABBBABBBABBBAABABBBAAABAAABAAAB ' -T='A++A,B++++B,A---B,B---A' -e=0 -w=2 -a='(3,B++++)' -i=2 -@=1 -J -l=,A,B -B
%%
\begin{center}
%
{\includegraphics*[width=64.5mm, viewport={0 247 595 822}]{3464-r37-tile-plus-B3-decomp-1.pdf}}%
\hspace*{0mm}% layout
{\includegraphics*[width=64.5mm, viewport={0 247 595 822}]{3464-r37-tile-plus-B3-decomp-2.pdf}}%
%
\end{center}
\caption{\label{fig:3464-r37-tile-plus-B3-decomp}
%
Decomposition of the prototile \tileS{B++++}{3} into smaller copies of \tileS{A++}{6} and \tileS{B++++}{3}.
Coloring by orientation of curves (left)
and by tiles (right, small copies of \tileS{A++}{6} blue,
 those of \tileS{B++++}{3} red).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-r37-tiles-plus.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%% zrender -d=12 -m='A AAAABAAABBABAAABBAA  B BABBBABAAABBBABBBABBBABAABBBABBBABBBAABABBBAAABAAABAAAB ' -T='A++A,B++++B,A---B,B---A' -e=0 -w=2 -a='(6,A++)' -k=-12 -i=3 -J
%% zrender -d=12 -m='A AAAABAAABBABAAABBAA  B BABBBABAAABBBABBBABBBABAABBBABBBABBBAABABBBAAABAAABAAAB ' -T='A++A,B++++B,A---B,B---A' -e=0 -w=2 -a='(3,B++++)' -k=+12 -i=3 -J
%%
%%
\begin{center}
%
{\includegraphics*[width=64.5mm, viewport={0 247 595 822}]{3464-r37-tiles-plus-A6.pdf}}%
\hspace*{0mm}% layout
{\includegraphics*[width=64.5mm, viewport={0 247 595 822}]{3464-r37-tiles-plus-B3.pdf}}%
%
\end{center}
\caption{\label{fig:3464-r37-tiles-plus}
%
Third iterates of the tiles \tileS{A++}{6} (left) and \tileS{B++++}{3} (right).
Coloring by orientation of curves contained.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-rotational-grid-graph.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a---b++++b++++b---A++a---b---A---B++++B---a++A++a  B B++++B---a++A---B  b b++++b---A++a---b ' -e=0 -w=7 -a='(3,@@A++@@a++)' -i=0 -l --arrows --arrow-offset=0.1 --letters=0.4 --zoom=2
%%
%% zrender -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a---b++++b++++b---A++a---b---A---B++++B---a++A++a  B B++++B---a++A---B  b b++++b---A++a---b ' -e=0 -w=25 -a='(3,A++a++)' -i=0 --arrows=0.15 --arrow-offset=0.05 --zoom=0.7 --no-text --letters=0.5 -l
%% zrender -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a---b++++b++++b---A++a---b---A---B++++B---a++A++a  B B++++B---a++A---B  b b++++b---A++a---b ' -e=0 -w=25 -a='---(3,B++++)' -i=0 --arrows=0.1 --arrow-offset=0.05 --zoom=0.6 --no-text --letters=0.3 -l
%% zrender -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a---b++++b++++b---A++a---b---A---B++++B---a++A++a  B B++++B---a++A---B  b b++++b---A++a---b ' -e=0 -w=25 -a='-(3,b++++)' -i=0 --arrows=0.1 --arrow-offset=0.05 --zoom=0.6 --no-text --letters=0.3 -l
%% zrender -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a---b++++b++++b---A++a---b---A---B++++B---a++A++a  B B++++B---a++A---B  b b++++b---A++a---b ' -e=0 -w=25 -a='(1,A---B---a---b)' -i=0 --arrows=0.1 --arrow-offset=0.05 --zoom=0.6 --no-text --letters=0.3 -l
%%
\begin{center}
%
\fbox{\includegraphics*[width=80mm, viewport={0 387 595 782}]{3464-rotational-grid-graph.pdf}}%
\hspace*{4mm}% layout
\begin{subfigure}[b]{20mm}
{\includegraphics*[width=18mm, viewport={0 247 595 802}]{3464-rotational-grid-graph-tile-AaAaAa.pdf}}
{\includegraphics*[width=18mm, viewport={0 247 595 802}]{3464-rotational-grid-graph-tile-B3.pdf}}
{\includegraphics*[width=18mm, viewport={0 247 595 802}]{3464-rotational-grid-graph-tile-b3.pdf}}
%\vspace*{7mm}% V
\end{subfigure}
\hspace*{0mm}% layout
\begin{subfigure}[b]{20mm}
{\includegraphics*[width=18mm, viewport={0 247 595 842}]{3464-rotational-grid-graph-tile-ABab.pdf}}
%\vspace*{1mm}% V
\end{subfigure}
\end{center}
%
\caption{\label{fig:3464-rotational-grid-graph}
%
%Directed edges
%\texttt{A},
%\texttt{a},
%\texttt{B}, and
%\texttt{b}
%on the $(3.4.6.4)$-grid with reduced rotational symmetry (left)
Coloring of the $(3.4.6.4)$-grid with four colors (left)
and the CCW (middle) and CW (right) prototiles.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% 3464-tile:
%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\begin{figure}[h!tbp]
%%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0 -w=5 -a='_(6,@@A++)' -i=0 --arrows=0.15 --arrow-offset=0.1 --zoom=2.0 --shift-y=-0.1 --letters=0.3 -l
%%%
%%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0 -w=20 -a='_(6,A++)' -i=0 --arrows=0.15 --arrow-offset=0.05 --zoom=0.7 --no-text --letters=0.5 -l
%%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0 -w=20 -a='_(3,B++++)' -i=0 --arrows=0.1 --arrow-offset=0.05 --zoom=0.6 --no-text --letters=0.3 -l
%%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0 -w=20 -a='_(2,A---B---)' -i=0 --arrows=0.1 --arrow-offset=0.05 --zoom=0.6 --no-text --letters=0.3 -l
%\begin{center}
%\fbox{\includegraphics*[width=70mm, viewport={0 387 595 782}]{3464-grid-graph.pdf}}%
%\hspace*{4mm}% layout
%{\includegraphics*[width=18mm, viewport={0 0 595 842}]{3464-tile-A6.pdf}}%
%{\includegraphics*[width=18mm, viewport={0 0 595 842}]{3464-tile-B3.pdf}}%
%{\includegraphics*[width=18mm, viewport={0 0 595 842}]{3464-tile-ABAB.pdf}}%
%\end{center}
%\caption{\label{fig:3464-tile}
%Directed edges on the $(3.4.6.4)$-grid and prototiles to be considered.\IMAGENAME%
%}
%\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-rotational-surgery.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a++A++a---b---A---B++++B---a---b++++b++++b---A++a  B B++++B---a++A---B  b b++++b---A++a---b' -e=0.1 -w=10 -l -@=0 -i=1 -A -L=0.4 -a='A---B---a---b' -r=A
%% zrender -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a++A++a---b---A---B++++B---a++A++a  B B++++B---a++A---B  b b++++b---A++a---b' -e=0.1 -w=10 -l -@=0 -i=1 -A -L=0.4 -a='A---B---a---b' -r=A
%% zrender -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a++A++a---b---A---B++++B---a++A++a  B B++++B---a---b++++b++++b---A---B  b b++++b---A++a---b' -e=0.1 -w=10 -l -@=0 -i=1 -A -L=0.4 -a='A---B---a---b' -r=A
%%
\begin{center}
%
{\includegraphics*[width=40mm, viewport={40 287 545 785}]{3464-rotational-surgery-start.pdf}}%
\hspace*{2mm}% layout
{\includegraphics*[width=40mm, viewport={40 287 545 785}]{3464-rotational-surgery-cut.pdf}}%
\hspace*{2mm}% layout
{\includegraphics*[width=40mm, viewport={40 287 545 785}]{3464-rotational-surgery-end.pdf}}%
%
\end{center}
\caption{\label{fig:3464-rotational-surgery}
%
CW tile \tileS{A---B---a---b---}{1} from the curve-set in the previous section (left).
The same with a triangle removed from curve \texttt{a} (middle).
The triangle attached to the curve \texttt{B} (right),
this is the CW tile for our current curve-set.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-rotational-x00-motifs.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a++A++a---b---A---B++++B---a---b++++b++++b---A++a  B B++++B---a++A---B  b b++++b---A++a---b' -e=0.1 -w=20 -l -@=1 -i=0 -A -L=0.4 -a=A
%%
%%
\begin{center}
%
{\includegraphics*[width=30mm, viewport={50 290 560 790}]{3464-rotational-x00-motifs-A.pdf}}%
{\includegraphics*[width=30mm, viewport={50 290 560 790}]{3464-rotational-x00-motifs-a.pdf}}%
{\includegraphics*[width=30mm, viewport={50 290 560 790}]{3464-rotational-x00-motifs-B.pdf}}%
{\includegraphics*[width=30mm, viewport={50 290 560 790}]{3464-rotational-x00-motifs-b.pdf}}%
%
\end{center}
\caption{\label{fig:3464-rotational-x00-motifs}
%
Motifs, from left to right,
for \texttt{A}, \texttt{a}, \texttt{B}, and \texttt{b}.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-rotational-x00-prototiles-plus-monochrome.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -a='(3,@A++@a++) ' -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a++A++a---b---A---B++++B---a---b++++b++++b---A++a  B B++++B---a++A---B  b b++++b---A++a---b ' -e=0 -w=8 -i=4 -J -l=,aA,B,b
%% zrender -a='+(3,@B++++) ' -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a++A++a---b---A---B++++B---a---b++++b++++b---A++a  B B++++B---a++A---B  b b++++b---A++a---b ' -e=0 -w=12 -i=4 -J -l=,aA,B,b
%% zrender -a='+++(3,@b++++) ' -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a++A++a---b---A---B++++B---a---b++++b++++b---A++a  B B++++B---a++A---B  b b++++b---A++a---b ' -e=0 -w=12 -i=4 -J -l=,aA,B,b
%%
%%
\begin{center}
{\includegraphics*[width=50mm, viewport={30 247 565 822}]{3464-rotational-x00-prototiles-plus-A6-monochrome.pdf}}%
\hspace*{18mm}% layout
\begin{subfigure}[b]{26mm}
{\includegraphics*[width=25mm, viewport={0 247 595 842}]{3464-rotational-x00-prototiles-plus-B3-monochrome.pdf}}
{\includegraphics*[width=25mm, viewport={0 247 595 842}]{3464-rotational-x00-prototiles-plus-b3-monochrome.pdf}}
\end{subfigure}
\end{center}
\caption{\label{fig:3464-rotational-x00-prototiles-plus-monochrome}
%
A version of the previous figure that may be easier to decipher:
coloring by tiles.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-rotational-x00-prototiles-plus.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -a='(3,@A++@a++) ' -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a++A++a---b---A---B++++B---a---b++++b++++b---A++a  B B++++B---a++A---B  b b++++b---A++a---b ' -e=0 -w=8 -k=-12 -i=4 -J='A,6,4;a,6,4;B,3,4;b,3,4;'
%% zrender -a='+(3,@B++++) ' -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a++A++a---b---A---B++++B---a---b++++b++++b---A++a  B B++++B---a++A---B  b b++++b---A++a---b ' -e=0 -w=12 -k=-12 -i=4 -J='A,6,4;a,6,4;B,3,4;b,3,4;'
%% zrender -a='+++(3,@b++++) ' -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a++A++a---b---A---B++++B---a---b++++b++++b---A++a  B B++++B---a++A---B  b b++++b---A++a---b ' -e=0 -w=12 -k=-12 -i=4 -J='A,6,4;a,6,4;B,3,4;b,3,4;'
%%
%%
\begin{center}
\hspace*{0mm}% layout
{\includegraphics*[width=50mm, viewport={30 247 565 822}]{3464-rotational-x00-prototiles-plus-A6.pdf}}%
\hspace*{20mm}% layout
\begin{subfigure}[b]{45mm}
{\includegraphics*[width=25mm, viewport={0 247 595 842}]{3464-rotational-x00-prototiles-plus-B3.pdf}}
{\includegraphics*[width=25mm, viewport={0 247 595 842}]{3464-rotational-x00-prototiles-plus-b3.pdf}}
\end{subfigure}
\end{center}
\caption{\label{fig:3464-rotational-x00-prototiles-plus}
%
Mutual self-similarity of the CCW prototiles
\tileS{A--a--}{3} (left),
\tileS{B----}{3} (upper right),
and
\tileS{b----}{3} (lower right).
Coloring by curves and their orientation.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-rotational-x02-motifs.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a++A++a---b---A---B++++B---a++A++a  B B++++B---a---b++++b++++b---A---B  b b++++b---A++a---b ' -e=0.1 -w=20 -l -@=1 -i=0 -A -L=0.4 -a=A
%%
%%
\begin{center}
%
{\includegraphics*[width=30mm, viewport={50 290 560 790}]{3464-rotational-x02-motifs-A.pdf}}%
{\includegraphics*[width=30mm, viewport={50 290 560 790}]{3464-rotational-x02-motifs-a.pdf}}%
{\includegraphics*[width=30mm, viewport={50 290 560 790}]{3464-rotational-x02-motifs-B.pdf}}%
{\includegraphics*[width=30mm, viewport={50 290 560 790}]{3464-rotational-x02-motifs-b.pdf}}%
%
\end{center}
\caption{\label{fig:3464-rotational-x02-motifs}
%
Motifs, from left to right,
for \texttt{A}, \texttt{a}, \texttt{B}, and \texttt{b}.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-rotational-x02-prototiles-minus.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%% rotated to save vertical space
%%
%% zrender -a='(1,@A---@B---@a---@b) ' -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a++A++a---b---A---B++++B---a++A++a  B B++++B---a---b++++b++++b---A---B  b b++++b---A++a---b ' -e=0 -w=6 -k=+3 -i=4 -r=i+2.0 -J
%%
\begin{center}
\hspace*{0mm}% layout
%{\includegraphics*[width=85mm, viewport={0 270 595 800}]{3464-rotational-x02-prototiles-minus-ABab.pdf}}
%{\includegraphics*[width=120mm, viewport={0 400 595 670}]{3464-rotational-x02-prototiles-minus-ABab.pdf}}
%
{\includegraphics*[width=120mm, viewport={0 400 595 670}]{3464-rotational-x02-prototiles-minus-ABab-decomp.pdf}}
\end{center}
\caption{\label{fig:3464-rotational-x02-prototiles-minus}
%
%The prototile \texttt{ABab} (top).
%It is self-similar and the smaller copies appear in three rotations (bottom).
Self-similarity of the CW prototile \tileS{A---B---a---b---}{1},
the small copies appear in three orientations.
Coloring by orientation.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%% zrender -a='(1,@A---@B---@a---@b) ' -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a++A++a---b---A---B++++B---a++A++a  B B++++B---a---b++++b++++b---A---B  b b++++b---A++a---b ' -e=0 -w=6 -k=-12 -i=4 -r=i+2.0 -J='A,6,4;a,6,4;B,3,4;b,3,4;'
%%

%% zrender -a='(1,@A---@B---@a---@b) ' -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a++A++a---b---A---B++++B---a++A++a  B B++++B---a---b++++b++++b---A---B  b b++++b---A++a---b ' -e=0 -w=8 -k=-12 -i=3 -J='A,6,4;a,6,4;B,3,4;b,3,4;'



%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-rotational-x02-prototiles-plus-monochrome.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -a='(3,@A++@a++) ' -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a++A++a---b---A---B++++B---a++A++a  B B++++B---a---b++++b++++b---A---B  b b++++b---A++a---b ' -e=0 -w=8 -i=4 -J -l=,aA,B,b
%% zrender -a='+(3,@B++++) ' -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a++A++a---b---A---B++++B---a++A++a  B B++++B---a---b++++b++++b---A---B  b b++++b---A++a---b ' -e=0 -w=12 -i=4 -J -l=,aA,B,b
%% zrender -a='+++(3,@b++++) ' -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a++A++a---b---A---B++++B---a++A++a  B B++++B---a---b++++b++++b---A---B  b b++++b---A++a---b ' -e=0 -w=12 -i=4 -J -l=,aA,B,b
%%
%%
\begin{center}
{\includegraphics*[width=50mm, viewport={30 247 565 822}]{3464-rotational-x02-prototiles-plus-A6-monochrome.pdf}}%
\hspace*{18mm}% layout
\begin{subfigure}[b]{26mm}
{\includegraphics*[width=25mm, viewport={0 247 595 842}]{3464-rotational-x02-prototiles-plus-B3-monochrome.pdf}}
{\includegraphics*[width=25mm, viewport={0 247 595 842}]{3464-rotational-x02-prototiles-plus-b3-monochrome.pdf}}
\end{subfigure}
\end{center}
\caption{\label{fig:3464-rotational-x02-prototiles-plus-monochrome}
%
A version of the previous figure that may be easier to decipher.
Coloring by tiles.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-rotational-x02-prototiles-plus.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -a='(3,@A++@a++) ' -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a++A++a---b---A---B++++B---a++A++a  B B++++B---a---b++++b++++b---A---B  b b++++b---A++a---b ' -e=0 -w=8 -k=-12 -i=4 -J='A,6,4;a,6,4;B,3,4;b,3,4;'
%% zrender -a='+(3,@B++++) ' -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a++A++a---b---A---B++++B---a++A++a  B B++++B---a---b++++b++++b---A---B  b b++++b---A++a---b ' -e=0 -w=12 -k=-12 -i=4 -J='A,6,4;a,6,4;B,3,4;b,3,4;'
%% zrender -a='+++(3,@b++++) ' -d=12 -m='A A---B++++B++++B---a++A---B---a---b++++b---A++a++A  a a++A++a---b---A---B++++B---a++A++a  B B++++B---a---b++++b++++b---A---B  b b++++b---A++a---b ' -e=0 -w=12 -k=-12 -i=4 -J='A,6,4;a,6,4;B,3,4;b,3,4;'
%%
%%
\begin{center}
\hspace*{0mm}% layout
{\includegraphics*[width=85mm, viewport={30 247 565 822}]{3464-rotational-x02-prototiles-plus-A6.pdf}}%
\hspace*{0mm}% layout
\begin{subfigure}[b]{45mm}
{\includegraphics*[width=45mm, viewport={0 247 595 842}]{3464-rotational-x02-prototiles-plus-B3.pdf}}
{\includegraphics*[width=45mm, viewport={0 247 595 842}]{3464-rotational-x02-prototiles-plus-b3.pdf}}
\end{subfigure}
\end{center}
\caption{\label{fig:3464-rotational-x02-prototiles-plus}
%
Mutual self-similarity of the CCW prototiles
\tileS{A++a++}{3} (left),
\tileS{B++++}{3} (upper right),
and
\tileS{b++++}{3} (lower right).
Coloring by curves and their orientation.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-tile-repeat.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-3464.txt
%%
%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0 -w=10 -a='_(6,@@A++)' -i=0 --arrows=0.15 --arrow-offset=0.1 --zoom=2.0 --shift-y=-0.1 -L=0.4 -l
%%
%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0 -w=20 -a='_(6,A++)' -i=0 --arrows=0.15 --arrow-offset=0.05 --zoom=0.7 --letters=0.5 -l
%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0 -w=20 -a='_(3,B++++)' -i=0 --arrows=0.1 --arrow-offset=0.05 --zoom=0.6 --letters=0.3 -l
%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0 -w=20 -a='_(2,A---B---)' -i=0 --arrows=0.1 --arrow-offset=0.05 --zoom=0.6 --letters=0.3 -l
%%
\begin{center}
%
\hspace*{4mm}% layout
\fbox{\includegraphics*[width=70mm, viewport={0 387 595 782}]{3464-grid-graph.pdf}}%
\hspace*{2mm}% layout
%
\begin{subfigure}[b]{20mm}
{\includegraphics*[width=18mm, viewport={0 247 595 842}]{3464-tile-A6.pdf}}
{\includegraphics*[width=18mm, viewport={0 247 595 842}]{3464-tile-B3.pdf}}%
\vspace*{5mm}% V
\end{subfigure}%
%
\begin{subfigure}[b]{20mm}
{\includegraphics*[width=18mm, viewport={0 247 595 842}]{3464-tile-ABAB.pdf}}%
\vspace*{5mm}% V
\end{subfigure}
%
\end{center}
%\caption{\label{fig:3464-tile}% prior version
\caption{\label{fig:3464-tile-repeat}
The minimal coloring of the $(3.4.6.4)$-grid (left).
Its CCW prototiles \tileS{A++}{6} and \tileS{B++++}{3} (middle),
and the CW prototile \tileS{A---B---}{2} (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3464-tile.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-3464.txt
%%
%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0 -w=10 -a='_(6,@@A++)' -i=0 --arrows=0.15 --arrow-offset=0.1 --zoom=2.0 --shift-y=-0.1 -L=0.4 -l
%%
%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0 -w=20 -a='_(6,A++)' -i=0 --arrows=0.15 --arrow-offset=0.05 --zoom=0.7 --letters=0.5 -l
%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0 -w=20 -a='_(3,B++++)' -i=0 --arrows=0.1 --arrow-offset=0.05 --zoom=0.6 --letters=0.3 -l
%% zrender -d=12 -m='A A++A++A++A++A---B---A---B++++B---A  B B++++B---A---B++++B++++B---A---B' -e=0 -w=20 -a='_(2,A---B---)' -i=0 --arrows=0.1 --arrow-offset=0.05 --zoom=0.6 --letters=0.3 -l
%%
\begin{center}
%
\hspace*{4mm}% layout
\fbox{\includegraphics*[width=70mm, viewport={0 387 595 782}]{3464-grid-graph.pdf}}%
\hspace*{2mm}% layout
%
\begin{subfigure}[b]{20mm}
{\includegraphics*[width=18mm, viewport={0 247 595 842}]{3464-tile-A6.pdf}}
{\includegraphics*[width=18mm, viewport={0 247 595 842}]{3464-tile-B3.pdf}}%
\vspace*{5mm}% V
\end{subfigure}%
%
\begin{subfigure}[b]{20mm}
{\includegraphics*[width=18mm, viewport={0 247 595 842}]{3464-tile-ABAB.pdf}}%
\vspace*{5mm}% V
\end{subfigure}
%
\end{center}
\caption{\label{fig:3464-tile}
The minimal coloring of the $(3.4.6.4)$-grid (left).
Its CCW prototiles \tileS{A++}{6} and \tileS{B++++}{3} (middle),
and the CW prototile \tileS{A---B---}{2} (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3636-AB-grid-graph.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%% zrender -d=6 -a='_(3,@@A--) ' -m='A A+B+A--A+B+A--A--A+B+A--A+B--B+A+B+A--A+B+A+B+A+B--B+A--A  B B+A--A+B+A+B+A+B--B--B+A+B--B--B+A+B--B+A--A+B+A+B+A+B--B ' -e=0 -w=5 -i=0 --letters=0.4 --arrows --arrow-offset=0.1 --zoom=4 -l
%%
%% zrender -d=6 -a='_(3,A+B+) ' -m='A A  B B ' -e=0 -w=25 -i=0 --arrows=0.15 --arrow-offset=0.05 --zoom=1.0 --no-text --letters=0.6 -l
%% zrender -d=6 -a='_(3,A--) ' -m='A A  B B ' -e=0 -w=20 -i=0 --arrows=0.1 --arrow-offset=0.05 --zoom=0.6 --no-text --letters=0.3 -l
%% zrender -d=6 -a='_+(3,B--) ' -m='A A  B B ' -e=0 -w=20 -i=0 --arrows=0.1 --arrow-offset=0.05 --zoom=0.6 --no-text --letters=0.3 -l
%%
%%% zrender -d=6 -a='(2,A--)(3,A+B+)-(2,--B) ' -m='A A+B+A--A+B+A--A--A+B+A--A+B--B+A+B+A--A+B+A+B+A+B--B+A--A  B B+A--A+B+A+B+A+B--B--B+A+B--B--B+A+B--B+A--A+B+A+B+A+B--B ' -e=0.1 -w=20 -i=0 --arrows=0.1 --arrow-offset=0.05 --zoom=0.6 --no-text --letters=0.3 -k=+6
%%
\begin{center}
\hspace*{0mm}% layout
\fbox{\includegraphics*[width=75mm, viewport={0 457 400 720}]{3636-AB-grid-graph.pdf}}%
\hspace*{0mm}% layout
\begin{subfigure}[b]{21mm}
{\includegraphics*[width=20mm, viewport={0 247 595 842}]{3636-AB-grid-graph-tile-ABABAB.pdf}}
\vspace*{8mm}% V
\end{subfigure}
\begin{subfigure}[b]{20mm}
{\includegraphics*[width=20mm, viewport={0 247 595 842}]{3636-AB-grid-graph-tile-A3.pdf}}
{\includegraphics*[width=20mm, viewport={0 247 595 842}]{3636-AB-grid-graph-tile-B3.pdf}}
\end{subfigure}
%\begin{subfigure}[b]{25mm}
%\fbox{\includegraphics*[width=25mm, viewport={0 247 595 842}]{3636-AB-grid-graph-outline-it0.pdf}}
%\vspace*{10mm}% V
%\end{subfigure}
\end{center}
\caption{\label{fig:3636-AB-grid-graph}
%
Coloring of the $(3.6.3.6)$-grid using two colors (left).
The CCW prototile (middle) and
the two CW prototiles (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3636-AB-r16-B-const-it4.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -a='A' -m='A A+B+A--A--A+B+A--A+B+A+B+A+B--B+A--A+B--B--B+A+B+A+B--B--B+A+B+A+B+A--A  B B ' -e=0.15 -k=-1 -w=7 -@=1 -i=3 -k=-1 -J
%% == shape of R16-t-7: F0F+F+F-F-F0F-F0F+F0F+F+F-F-F0F
%% zrender -d=3 -a=F -m='F F+F-F-F+F-F+F+F0F-F-F+F-F+F+F-F' -@=1 -i=2 -J -k=-1
%%
\begin{center}
%
{\includegraphics*[width=70mm, viewport={0 370 595 700}]{3636-AB-r16-B-const-it4.pdf}}%
%
\end{center}
\caption{\label{fig:3636-AB-r16-B-const-it4}
%
Fourth iterate of the curve \texttt{A},
decomposed into 16 smaller copies of itself.
Coloring by orientation of the small copies.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3636-AB-r16-B-const.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%% zrender -d=6 -a='A' -m='A A+B+A--A--A+B+A--A+B+A+B+A+B--B+A--A+B--B--B+A+B+A+B--B--B+A+B+A+B+A--A  B B ' -e=0.12 -k=-1 -w=12 -@=1 -i=0 -l=,A,B -L=0.5 -A
%% zrender -d=6 -a='A' -m='A A+B+A--A--A+B+A--A+B+A+B+A+B--B+A--A+B--B--B+A+B+A+B--B--B+A+B+A+B+A--A  B B ' -e=0.25 -k=-1 -w=10 -@=1 -i=1 -l=,A,B
%% zrender -d=6 -a='A' -m='A A+B+A--A--A+B+A--A+B+A+B+A+B--B+A--A+B--B--B+A+B+A+B--B--B+A+B+A+B+A--A  B B ' -e=0.15 -k=-1 -w=7 -@=1 -i=2 -l=,A,B -J
%%
%%
\begin{center}
%
{\includegraphics*[width=40mm, viewport={0 370 595 720}]{3636-AB-r16-B-const-A-it1.pdf}}%
{\includegraphics*[width=40mm, viewport={0 370 595 720}]{3636-AB-r16-B-const-A-it2.pdf}}%
{\includegraphics*[width=40mm, viewport={0 370 595 720}]{3636-AB-r16-B-const-A-it3.pdf}}%
\hspace*{0mm}% layout
%
\end{center}
\caption{\label{fig:3636-AB-r16-B-const}
%
First (left), second (middle), and third (right) iterate of a curve-set with one letter constant.
Coloring by letters, blue for \texttt{A} and red for the constant \texttt{B}.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3636-AB-r25-curve-motifs.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%% zrender -d=6 -a='A' -m='A A+B+A--A+B+A--A--A+B+A--A+B--B+A+B+A--A+B+A+B+A+B--B+A--A  B B+A--A+B+A+B+A+B--B--B+A+B--B--B+A+B--B+A--A+B+A+B+A+B--B ' -e=0.12 -k=-6 --colors-pick=1,6 -w=17 -@=1 -i=0 -A -L=0.6 -l
%% zrender -d=6 -a='(3,A--)' -m='A A+B+A--A+B+A--A--A+B+A--A+B--B+A+B+A--A+B+A+B+A+B--B+A--A  B B+A--A+B+A+B+A+B--B--B+A+B--B--B+A+B--B+A--A+B+A+B+A+B--B ' -e=0.12 -k=-6 --colors-pick=1,6 -w=12 -@=1 -i=0 -A -l
%%
%% zrender -d=6 -a='B' -m='A A+B+A--A+B+A--A--A+B+A--A+B--B+A+B+A--A+B+A+B+A+B--B+A--A  B B+A--A+B+A+B+A+B--B--B+A+B--B--B+A+B--B+A--A+B+A+B+A+B--B ' -e=0.12 -k=-6 --colors-pick=1,6 -w=17 -@=1 -i=0 -A -L=0.6 -l
%% zrender -d=6 -a='(3,B--)' -m='A A+B+A--A+B+A--A--A+B+A--A+B--B+A+B+A--A+B+A+B+A+B--B+A--A  B B+A--A+B+A+B+A+B--B--B+A+B--B--B+A+B--B+A--A+B+A+B+A+B--B ' -e=0.12 -k=-6 --colors-pick=1,6 -w=12 -@=1 -i=0 -A -l
%%
%%
\begin{center}
%
{\includegraphics*[width=32mm, viewport={0 267 595 822}]{3636-AB-r25-curve-motifs-A.pdf}}%
{\includegraphics*[width=32mm, viewport={0 267 595 822}]{3636-AB-r25-curve-motifs-AAA.pdf}}%
{\includegraphics*[width=32mm, viewport={0 267 595 822}]{3636-AB-r25-curve-motifs-B.pdf}}%
{\includegraphics*[width=32mm, viewport={0 267 595 822}]{3636-AB-r25-curve-motifs-BBB.pdf}}%
%\hspace*{0mm}% layout
%
\end{center}
\caption{\label{fig:3636-AB-r25-curve-motifs}
%
From left to right:
motif for curve \texttt{A},
motif for tile \tileS{A--}{3},
motif for curve \texttt{B}, and
motif for tile \tileS{B--}{3}.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3636-AB-r25-curve-tile-minus-decomp.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -a='(3,A--) ' -m='A A+B+A--A+B+A--A--A+B+A--A+B--B+A+B+A--A+B+A+B+A+B--B+A--A  B B+A--A+B+A+B+A+B--B--B+A+B--B--B+A+B--B+A--A+B+A+B+A+B--B ' -e=0.1 -k=-6 --colors-pick=1,6 -w=3 -i=2 -@=1 -J
%%
%% zrender -d=6 -a='+(3,B--) ' -m='A A+B+A--A+B+A--A--A+B+A--A+B--B+A+B+A--A+B+A+B+A+B--B+A--A  B B+A--A+B+A+B+A+B--B--B+A+B--B--B+A+B--B+A--A+B+A+B+A+B--B ' -e=0.1 -k=-6 --colors-pick=1,6 -w=3 -i=2 -@=1 -J
%%
\begin{center}
%
{\includegraphics*[width=64.5mm, viewport={0 300 595 780}]{3636-AB-r25-curve-tile-minus-decomp-A3.pdf}}%
\hspace*{0mm}% layout
{\includegraphics*[width=64.5mm, viewport={0 300 595 780}]{3636-AB-r25-curve-tile-minus-decomp-B3.pdf}}%
%
\end{center}
\caption{\label{fig:3636-AB-r25-curve-tile-minus-decomp}
%
Decompositions of the CW tiles \tileS{A--}{3} (left) and \tileS{B--}{3} (right)
into smaller copies of themselves.
Coloring by orientations of the curves in the small copies.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3636-AB-r25-curve-tile-minus.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -a='(3,A--) ' -m='A A+B+A--A+B+A--A--A+B+A--A+B--B+A+B+A--A+B+A+B+A+B--B+A--A  B B+A--A+B+A+B+A+B--B--B+A+B--B--B+A+B--B+A--A+B+A+B+A+B--B ' -e=0.1 -k=-6 --colors-pick=1,6 -w=3 -i=3 -J
%%
%% zrender -d=6 -a='+(3,B--) ' -m='A A+B+A--A+B+A--A--A+B+A--A+B--B+A+B+A--A+B+A+B+A+B--B+A--A  B B+A--A+B+A+B+A+B--B--B+A+B--B--B+A+B--B+A--A+B+A+B+A+B--B ' -e=0.1 -k=-6 --colors-pick=1,6 -w=3 -i=3 -J
%%
\begin{center}
%
{\includegraphics*[width=50mm, viewport={0 300 595 780}]{3636-AB-r25-curve-tile-minus-A3.pdf}}%
\hspace*{0mm}% layout
{\includegraphics*[width=50mm, viewport={0 300 595 780}]{3636-AB-r25-curve-tile-minus-B3.pdf}}%
%
\end{center}
\caption{\label{fig:3636-AB-r25-curve-tile-minus}
%
Third iterates of the CW tiles \tileS{A--}{3} (left) and \tileS{B--}{3} (right).
Coloring by orientation of curves.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3636-AB-r25-curve-tile-plus.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%% zrender -d=6 -a='(3,A+B+) ' -m='A A+B+A--A+B+A--A--A+B+A--A+B--B+A+B+A--A+B+A+B+A+B--B+A--A  B B+A--A+B+A+B+A+B--B--B+A+B--B--B+A+B--B+A--A+B+A+B+A+B--B ' -e=0.1 -k=-6 --colors-pick=1,6 -w=3 -i=3 -J
%%
%% zrender -d=6 -a='(3,A+B+) ' -m='A A+B+A--A+B+A--A--A+B+A--A+B--B+A+B+A--A+B+A+B+A+B--B+A--A  B B+A--A+B+A+B+A+B--B--B+A+B--B--B+A+B--B+A--A+B+A+B+A+B--B ' -e=0.1 -k=-6 --colors-pick=1,6 -w=3 -i=2 -@=1 -J
%%
%%
\begin{center}
%
{\includegraphics*[width=50mm, viewport={0 252 595 822}]{3636-AB-r25-curve-tile-plus.pdf}}%
\hspace*{3mm}% layout
{\includegraphics*[width=70mm, viewport={0 262 595 812}]{3636-AB-r25-curve-tile-plus-decomp.pdf}}%
%
\end{center}
\caption{\label{fig:3636-AB-r25-curve-tile-plus}
%
Third iterate of the CCW tile \tileS{A+B+}{3},
colored by orientations of the curves contained (left).
The same, decomposed into 25 smaller copies of itself (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3636-FGH-grid-graph.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-rotational-x6.txt
%%
%% zrender -d=6 -a='(2,F--G--H--) ' -m='F F+G+H--F+G+H--F--G+H+F--G+H--F+G+H+F--G+H+F+G+H+F--G+H--F  G G+H+F--G+H+F--G--H+F+G--H+F--G+H+F+G--H+F+G+H+F+G--H+F--G H H+F+G--H+F+G--H--F+G+H--F+G--H+F+G+H--F+G+H+F+G+H--F+G--H ' -e=0 -w=7 -i=0 -@=2 -l=',F,G,H' -L=0.4 -A --arrow-offset=0.1 --zoom=4
%% zrender -d=6 -a='(2,F+G+H+) ' --const-maps -e=0 -w=30 -i=0 -@=2 -l=',F,G,H' -L=0.5 -A=0.15,0.1
%% zrender -d=6 -a='(2,F--G--H--) ' --const-maps -e=0 -w=30 -i=0 -@=2 -l=',F,G,H' -L=0.3 -A=0.15,0.1
%%
%%
%%
\begin{center}
%
\fbox{\includegraphics*[width=89mm, viewport={0 447 595 742}]{3636-FGH-grid-graph.pdf}}%
%
\begin{subfigure}[b]{40mm}
{\includegraphics*[width=20mm, viewport={50 247 545 842}]{3636-FGH-grid-graph-tile-plus.pdf}}%
{\includegraphics*[width=18mm, viewport={90 247 525 842}]{3636-FGH-grid-graph-tile-minus.pdf}}
\vspace*{6mm}% V
\end{subfigure}
%
\end{center}
\caption{\label{fig:3636-FGH-grid-graph}
%
A coloring of the trihex grid with three colors (left)
and
its prototiles \tileS{F+G+H+}{2} (middle)
and \tileS{F--G--H--}{1} (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3636-FGH-motifs.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -m='F F+G+H--F+G+H--F--G+H--F+G+H+F+G--H--F+G+H+F--G+H+F+G+H+F--G+H--F  G G+H+F+G--H--F+G+H+F--G--H+F+G--H+F--G+H+F+G--H+F+G+H+F+G--H+F--G H H+F+G--H+F+G--H--F+G+H--F+G--H+F+G+H+F+G--H ' -e=0.15 -w=15 -A -L=0.5 -l=',F,G,H' -i=0 -@=1 -a=F
%%
%%
\begin{center}
%
{\includegraphics*[width=40mm, viewport={0 277 595 805}]{3636-FGH-motifs-F.pdf}}%
{\includegraphics*[width=40mm, viewport={0 277 595 805}]{3636-FGH-motifs-G.pdf}}%
{\includegraphics*[width=40mm, viewport={0 277 595 805}]{3636-FGH-motifs-H.pdf}}%
%\hspace*{0mm}% layout
%
\end{center}
\caption{\label{fig:3636-FGH-motifs}
%
Motifs for the curves
\texttt{F} (left),
\texttt{G} (middle), and
\texttt{H} (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3636-FGH-tile-minus.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-rotational-x6.txt , curve-set r25-fgh-var2
%%
%% zrender -d=6 -a='(2,F--G--H--) ' -m='F F+G+H--F+G+H--F--G+H--F+G+H+F+G--H--F+G+H+F--G+H+F+G+H+F--G+H--F  G G+H+F+G--H--F+G+H+F--G--H+F+G--H+F--G+H+F+G--H+F+G+H+F+G--H+F--G H H+F+G--H+F+G--H--F+G+H--F+G--H+F+G+H+F+G--H ' -e=0.1 -w=7 -A -L=0.45 -l=',F,G,H' -i=1 -@=0
%%
%% zrender -d=6 -a='(1,F--G--H--) ' -m='F F+G+H--F+G+H--F--G+H--F+G+H+F+G--H--F+G+H+F--G+H+F+G+H+F--G+H--F  G G+H+F+G--H--F+G+H+F--G--H+F+G--H+F--G+H+F+G--H+F+G+H+F+G--H+F--G H H+F+G--H+F+G--H--F+G+H--F+G--H+F+G+H+F+G--H ' -e=0 -k=+2  -i=2 -@=1 -J='F,6,3;G,6,3;H,6,3;'
%%
\begin{center}
%
{\includegraphics*[width=64.5mm, viewport={0 305 595 790}]{3636-FGH-tile-minus-it1.pdf}}%
\hspace*{0mm}% layout
{\includegraphics*[width=64.5mm, viewport={0 297 595 782}]{3636-FGH-tile-minus-self-sim.pdf}}%
%
\end{center}
\caption{\label{fig:3636-FGH-tile-minus}
%
First iterate (left, coloring by curves) and
self-similarity (right, coloring of the small tiles by orientation)
of the CW tile \tileS{F--G--H--}{1}.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3636-FGH-tile-plus.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-rotational-x6.txt , curve-set r25-fgh-var2
%%
%%% zrender -d=6 -a='(2,F+G+H+) ' -m='F F+G+H--F+G+H--F--G+H--F+G+H+F+G--H--F+G+H+F--G+H+F+G+H+F--G+H--F  G G+H+F+G--H--F+G+H+F--G--H+F+G--H+F--G+H+F+G--H+F+G+H+F+G--H+F--G H H+F+G--H+F+G--H--F+G+H--F+G--H+F+G+H+F+G--H ' -e=0.15 -w=10 -A -L=0.6 -l=',F,G,H'  -i=1 -@=0
%%
%% zrender -d=6 -a='(2,F+G+H+) ' -m='F F+G+H--F+G+H--F--G+H--F+G+H+F+G--H--F+G+H+F--G+H+F+G+H+F--G+H--F  G G+H+F+G--H--F+G+H+F--G--H+F+G--H+F--G+H+F+G--H+F+G+H+F+G--H+F--G H H+F+G--H+F+G--H--F+G+H--F+G--H+F+G+H+F+G--H ' --colors-pick=1,6 -t='+,-' -i=3 -@=0 -J
%%
%% zrender -d=6 -a='(2,F+G+H+) ' -m='F F+G+H--F+G+H--F--G+H--F+G+H+F+G--H--F+G+H+F--G+H+F+G+H+F--G+H--F  G G+H+F+G--H--F+G+H+F--G--H+F+G--H+F--G+H+F+G--H+F+G+H+F+G--H+F--G H H+F+G--H+F+G--H--F+G+H--F+G--H+F+G+H+F+G--H ' --colors-pick=1,6 -t='+,-' -i=2 -@=1 -J
%%
\begin{center}
%
%{\includegraphics*[width=60mm, viewport={0 257 595 822}]{3636-FGH-tile-plus-it1.pdf}}%
{\includegraphics*[width=50mm, viewport={0 265 595 805}]{3636-FGH-tile-plus-it3.pdf}}%
\hspace*{3mm}% layout
{\includegraphics*[width=70mm, viewport={0 265 595 805}]{3636-FGH-tile-plus-it3-decomp.pdf}}%
%
\end{center}
\caption{\label{fig:3636-FGH-tile-plus}
%
%First (left) and third (right) iterate of the CCW tile \tileS{F+G+H+}{2}.\IMAGENAME%
Third iterate of the CCW tile \tileS{F+G+H+}{2}, colored by curves contained (left).
The same, decomposed into 25 smaller copies of itself (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3636-grid-graph.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -a='F' --const-maps -w=5 --letters=0.4 -A=0.2,0.1 -T='F+F,F--F' --grid=15,15 -l --zoom=1.3 --shift-y=-0.03
%%
%% zrender -d=6 -a='(6,F+)'  -m='F F' -e=0 -w=25 -i=0 -A=0.15,0.05 --zoom=1.0 --no-text --letters=0.6 -l
%% zrender -d=6 -a='(3,F--)' -m='F F' -e=0 -w=20 -i=0 -A=0.1,0.05 --zoom=0.6 --no-text --letters=0.3 -l
%%
%%
\begin{center}
\hspace*{0mm}% layout
\fbox{\includegraphics*[width=65mm, viewport={0 477 400 720}]{3636-grid-graph.pdf}}%
\hspace*{3mm}% layout
%
\begin{subfigure}[b]{21mm}
{\includegraphics*[width=20mm, viewport={0 247 595 842}]{3636-grid-graph-tile-plus.pdf}}
\vspace*{8mm}% V
%
\end{subfigure}
\begin{subfigure}[b]{21mm}
{\includegraphics*[width=20mm, viewport={160 367 495 782}]{3636-grid-graph-tile-minus.pdf}}
\vspace*{8mm}% V
\end{subfigure}
%
\end{center}
\caption{\label{fig:3636-grid-graph}
%
Minimal coloring of the $(3.6.3.6)$-grid (left),
the CCW prototile \tileS{F+}{6} (middle), and
the CW prototile \tileS{F--}{3} (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3636-set-curve-r16-CW-tiles.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -T='A+B,B+C,C+D,D+E,E+F,F+A,A--E,E--C,C--A,B--F,F--D,D--B' -a='A--E--C--' --colors-pick=1,6 -l -e=0.12 -m='A AEFABCDBCABCAEFDEFABCAEFA  B BCDBFAB  C CABCDEFDECDBFABCDECABC  D DBCDEFAEFDBCD  E ECDEFABFAEFDBCDEFAECDE  F FABFDEF' -i=1 -w=10 -A -L=0.45
%%
%% zrender -d=6 -T='A+B,B+C,C+D,D+E,E+F,F+A,A--E,E--C,C--A,B--F,F--D,D--B' -a='A--E--C--' --colors-pick=1,6 -l -e=0.12 -m='A AEFABCDBCABCAEFDEFABCAEFA  B BCDBFAB  C CABCDEFDECDBFABCDECABC  D DBCDEFAEFDBCD  E ECDEFABFAEFDBCDEFAECDE  F FABFDEF' -i=3 -J
%%
%%
%%  zrender -d=6 -T='A+B,B+C,C+D,D+E,E+F,F+A,A--E,E--C,C--A,B--F,F--D,D--B' -a='+B--F--D--' --colors-pick=1,6 -l -e=0.12 -m='A AEFABCDBCABCAEFDEFABCAEFA  B BCDBFAB  C CABCDEFDECDBFABCDECABC  D DBCDEFAEFDBCD  E ECDEFABFAEFDBCDEFAECDE  F FABFDEF' -i=1 -w=10 -A -L=0.45
%%
%% zrender -d=6 -T='A+B,B+C,C+D,D+E,E+F,F+A,A--E,E--C,C--A,B--F,F--D,D--B' -a='+B--F--D--' --colors-pick=1,6 -l -e=0.12 -m='A AEFABCDBCABCAEFDEFABCAEFA  B BCDBFAB  C CABCDEFDECDBFABCDECABC  D DBCDEFAEFDBCD  E ECDEFABFAEFDBCDEFAECDE  F FABFDEF' -i=3 -J
%%
\begin{center}
%
{\includegraphics*[width=25mm, viewport={70 247 530 812}]{3636-set-curve-r16-CW-tiles-AEC-it1.pdf}}%
{\includegraphics*[width=40mm, viewport={0 247 595 822}]{3636-set-curve-r16-CW-tiles-AEC-it.pdf}}%
{\includegraphics*[width=25mm, viewport={70 247 530 812}]{3636-set-curve-r16-CW-tiles-BFD-it1.pdf}}%
{\includegraphics*[width=40mm, viewport={20 265 575 802}]{3636-set-curve-r16-CW-tiles-BFD-it.pdf}}%
\hspace*{0mm}% layout
%
%
%\begin{subfigure}[b]{20mm}
%\fbox{\includegraphics*[width=20mm, viewport={0 247 595 842}]{3636-set-curve-r16-CW-tiles.pdf}}
%\fbox{\includegraphics*[width=20mm, viewport={0 247 595 842}]{3636-set-curve-r16-CW-tiles.pdf}}
%\end{subfigure}
%
\end{center}
\caption{\label{fig:3636-set-curve-r16-CW-tiles}
From left to right:
first and third iterates of the CW tile \tileS{A--E--C--}{1},
first and third iterates of the CW tile \tileS{B--F--D--}{1}.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3636-set-curve-r16-lattice-tile1.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -T='A+B,B+C,C+D,D+E,E+F,F+A,A--E,E--C,C--A,B--F,F--D,D--B' -a='+B+C--A--E+F--D' --colors-pick=1,6 -l -e=0.12 -m='A AEFABCDBCABCAEFDEFABCAEFA  B BCDBFAB  C CABCDEFDECDBFABCDECABC  D DBCDEFAEFDBCD  E ECDEFABFAEFDBCDEFAECDE  F FABFDEF' -i=0 -w=20 -A -L=0.4
%%
%%  zrender -d=6 -T='A+B,B+C,C+D,D+E,E+F,F+A,A--E,E--C,C--A,B--F,F--D,D--B' -a='+B+C--A--E+F--D' --colors-pick=1,6 -l -e=0.12 -m='A AEFABCDBCABCAEFDEFABCAEFA  B BCDBFAB  C CABCDEFDECDBFABCDECABC  D DBCDEFAEFDBCD  E ECDEFABFAEFDBCDEFAECDE  F FABFDEF' -i=3 -J
%%
%% zrender -d=6 -T='A+B,B+C,C+D,D+E,E+F,F+A,A--E,E--C,C--A,B--F,F--D,D--B' -a='+B+C--A--E+F--D' --colors-pick=1,6 -l -e=0.12 -m='A AEFABCDBCABCAEFDEFABCAEFA  B BCDBFAB  C CABCDEFDECDBFABCDECABC  D DBCDEFAEFDBCD  E ECDEFABFAEFDBCDEFAECDE  F FABFDEF' -i=2 -@=1 -J
%%
\begin{center}
%
{\includegraphics*[width=28mm, viewport={0 247 595 812}]{3636-set-curve-r16-lattice-tile1-it0.pdf}}%
{\includegraphics*[width=47mm, viewport={0 250 595 815}]{3636-set-curve-r16-lattice-tile1-it.pdf}}%
{\includegraphics*[width=47mm, viewport={0 250 595 815}]{3636-set-curve-r16-lattice-tile1-decomp.pdf}}%
\hspace*{0mm}% layout
%
\end{center}
\caption{\label{fig:3636-set-curve-r16-lattice-tile1}
Arrangement (axiom) for a lattice tile (left),
its third iterate (middle), and
its decomposition into 16 smaller copies of itself (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3636-set-curve-r16-lattice-tile2.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -T='A+B,B+C,C+D,D+E,E+F,F+A,A--E,E--C,C--A,B--F,F--D,D--B' -a='A+B--F--D+E--C' --colors-pick=1,6 -l -e=0.12 -m='A AEFABCDBCABCAEFDEFABCAEFA  B BCDBFAB  C CABCDEFDECDBFABCDECABC  D DBCDEFAEFDBCD  E ECDEFABFAEFDBCDEFAECDE  F FABFDEF' -i=0 -w=20 -A -L=0.4
%%
%%  zrender -d=6 -T='A+B,B+C,C+D,D+E,E+F,F+A,A--E,E--C,C--A,B--F,F--D,D--B' -a='A+B--F--D+E--C' --colors-pick=1,6 -l -e=0.12 -m='A AEFABCDBCABCAEFDEFABCAEFA  B BCDBFAB  C CABCDEFDECDBFABCDECABC  D DBCDEFAEFDBCD  E ECDEFABFAEFDBCDEFAECDE  F FABFDEF' -i=3 -J
%%
%% zrender -d=6 -T='A+B,B+C,C+D,D+E,E+F,F+A,A--E,E--C,C--A,B--F,F--D,D--B' -a='A+B--F--D+E--C' --colors-pick=1,6 -l -e=0.12 -m='A AEFABCDBCABCAEFDEFABCAEFA  B BCDBFAB  C CABCDEFDECDBFABCDECABC  D DBCDEFAEFDBCD  E ECDEFABFAEFDBCDEFAECDE  F FABFDEF' -i=2 -@=1 -J
%%
\begin{center}
%
{\includegraphics*[width=23mm, viewport={90 247 490 700}]{3636-set-curve-r16-lattice-tile2-it0.pdf}}%
{\includegraphics*[width=53mm, viewport={0 300 585 780}]{3636-set-curve-r16-lattice-tile2-it.pdf}}%
{\includegraphics*[width=53mm, viewport={0 300 585 780}]{3636-set-curve-r16-lattice-tile2-decomp.pdf}}%
\hspace*{0mm}% layout
%
%
\end{center}
\caption{\label{fig:3636-set-curve-r16-lattice-tile2}
Arrangement (axiom) for a lattice tile (left),
its third iterate (middle), and
a failed attempt to decompose it into smaller copies of itself (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3636-set-curve-r16-var0.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -T='A+B,B+C,C+D,D+E,E+F,F+A,A--E,E--C,C--A,B--F,F--D,D--B' -a='A+B+C+D+E+F+' --colors-pick=1,6 -l -e=0.12 -m='A AEFABCDBCABCAEFDEFABCAEFA  B BCDBFAB  C CABCDEFDECDBFABCDECABC  D DBCDEFAEFDBCD  E ECDEFABFAEFDBCDEFAECDE  F FABFDEF' -i=1 -L=0.5 -A=0.25,0.1 --letters-mv=0.45 -w=10
%%
%%  zrender -d=6 -T='A+B,B+C,C+D,D+E,E+F,F+A,A--E,E--C,C--A,B--F,F--D,D--B' -a='A+B+C+D+E+F+' --colors-pick=1,6 -l -e=0.12 -m='A AEFABCDBCABCAEFDEFABCAEFA  B BCDBFAB  C CABCDEFDECDBFABCDECABC  D DBCDEFAEFDBCD  E ECDEFABFAEFDBCDEFAECDE  F FABFDEF' -i=4 -J
%%
%% zrender -d=6 -T='A+B,B+C,C+D,D+E,E+F,F+A,A--E,E--C,C--A,B--F,F--D,D--B' -a='A+B+C+D+E+F+' --colors-pick=1,6 -l -e=0.12 -m='A AEFABCDBCABCAEFDEFABCAEFA  B BCDBFAB  C CABCDEFDECDBFABCDECABC  D DBCDEFAEFDBCD  E ECDEFABFAEFDBCDEFAECDE  F FABFDEF' -i=3 -@=1 -J
%%
\begin{center}
%
{\includegraphics*[width=40mm, viewport={65 247 530 810}]{3636-set-curve-r16-var0-CCW-it1.pdf}}%
\hspace*{2mm}%
{\includegraphics*[width=43mm, viewport={50 247 525 815}]{3636-set-curve-r16-var0-CCW-it.pdf}}%
{\includegraphics*[width=43mm, viewport={50 247 525 815}]{3636-set-curve-r16-var0-CCW-decomp.pdf}}%
\hspace*{0mm}% layout
%
\end{center}
\caption{\label{fig:3636-set-curve-r16-var0}
First (left) and fourth (middle) iterate of the CCW tile \tileS{A+B+C+D+E+F+}{1},
colored by curves contained.
The self-similarity of the tile is shown on the right:
it can be decomposed into 16 small copies of itself.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3636-set-grid.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -T='A+B,B+C,C+D,D+E,E+F,F+A,A--E,E--C,C--A,B--F,F--D,D--B' -a=A -L=0.35 -w=10 -A=0.25,0.1 --colors-pick=1,6 -l --const-maps --grid=12 --zoom=1.35
%%
%%
%%  zrender -d=6 -T='A+B,B+C,C+D,D+E,E+F,F+A,A--E,E--C,C--A,B--F,F--D,D--B' -a='A+B+C+D+E+F' -L=0.4 -w=35 -A=0.2,0.1 --colors-pick=1,6 -l --const-maps --letters-mv=0.4
%% zrender -d=6 -T='A+B,B+C,C+D,D+E,E+F,F+A,A--E,E--C,C--A,B--F,F--D,D--B' -a='A--E--C--' -L=0.4 -w=25 -A=0.15,0.1 --colors-pick=1,6 -l --const-maps --letters-mv=0.4
%% zrender -d=6 -T='A+B,B+C,C+D,D+E,E+F,F+A,A--E,E--C,C--A,B--F,F--D,D--B' -a='+B--F--D--' -L=0.4 -w=25 -A=0.15,0.1 --colors-pick=1,6 -l --const-maps --letters-mv=0.4
%%
%%
%%
\begin{center}
%
\fbox{\includegraphics*[width=70mm, viewport={0 500 595 842}]{3636-set-grid.pdf}}%
\hspace*{3mm}% layout
%
%
\begin{subfigure}[b]{18mm}
{\includegraphics*[width=18mm, viewport={0 247 545 842}]{3636-set-grid-CCW.pdf}}%
%\vspace*{5mm}
\end{subfigure}
%
\begin{subfigure}[b]{19mm}
{\includegraphics*[width=18mm, viewport={50 330 595 842}]{3636-set-grid-CW-AEC.pdf}}
{\includegraphics*[width=18mm, viewport={50 247 595 842}]{3636-set-grid-CW-BFD.pdf}}%
%\vspace*{5mm}
\end{subfigure}
%
\end{center}
\caption{\label{fig:3636-set-grid}
Coloring of the $(3.6.3.6)$-grid with six colors (left),
its CCW prototile \tileS{A+B+C+D+E+F+}{1} (middle),
and its CW prototiles
\tileS{A--E--C--}{1} and \tileS{B--F--D--}{1}.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3636-unique-r67-1-tiles.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -m='F F--F+F--F+F--F+F--F+F+F--F+F--F+F+F--F+F--F+F+F+F--F+F+F--F--F+F+F--F+F--F+F+F+F--F+F+F--F+F+F+F--F+F+F--F+F--F+F+F+F+F+F--F+F--F+F+F+F--F+F+F+F--F+F+F+F+F' -a='(6,F+)' -@=0 -k=+1 -d=6 --comment=' # R67-1' -w=2 -c=glasbey2 -e=0.2 -w=4 -i=2
%%
%% zrender -m='F F--F+F--F+F--F+F--F+F+F--F+F--F+F+F--F+F--F+F+F+F--F+F+F--F--F+F+F--F+F--F+F+F+F--F+F+F--F+F+F+F--F+F+F--F+F--F+F+F+F+F+F--F+F--F+F+F+F--F+F+F+F--F+F+F+F+F' -a='(3,F--)' -@=0 -k=+1 -d=6 --comment=' # R67-1' -w=2 -c=glasbey2 -e=0.2 -w=4 -i=2
%%
\begin{center}
%
{\includegraphics*[width=60mm, viewport={20 247 575 815}]{3636-unique-r67-1-tiles-plus.pdf}}%
\hspace*{0mm}% layout
{\includegraphics*[width=60mm, viewport={20 247 575 802}]{3636-unique-r67-1-tiles-minus.pdf}}%
%
%
\end{center}
\caption{\label{fig:3636-unique-r67-1-tiles}
%
Second iterates of the CCW (left) and CW (right) tile of the curve.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/3636-unique-r67-1.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%% zrender -i=1 -m='F F--F+F--F+F--F+F--F+F+F--F+F--F+F+F--F+F--F+F+F+F--F+F+F--F--F+F+F--F+F--F+F+F+F--F+F+F--F+F+F+F--F+F+F--F+F--F+F+F+F+F+F--F+F--F+F+F+F--F+F+F+F--F+F+F+F+F' -a='F' -@=0 -k=+1 -d=6 --comment=' # unique R67-1' -w=1 -e=0.1 -i=1 -w=10 -A=0.3
%% zrender -i=1 -m='F F--F+F--F+F--F+F--F+F+F--F+F--F+F+F--F+F--F+F+F+F--F+F+F--F--F+F+F--F+F--F+F+F+F--F+F+F--F+F+F+F--F+F+F--F+F--F+F+F+F+F+F--F+F--F+F+F+F--F+F+F+F--F+F+F+F+F' -a='(6,F+)' -@=0 -k=+1 -d=6 --comment=' # unique R67-1' -w=1 -e=0.15 -i=1 -w=12
%% zrender -i=1 -m='F F--F+F--F+F--F+F--F+F+F--F+F--F+F+F--F+F--F+F+F+F--F+F+F--F--F+F+F--F+F--F+F+F+F--F+F+F--F+F+F+F--F+F+F--F+F--F+F+F+F+F+F--F+F--F+F+F+F--F+F+F+F--F+F+F+F+F' -a='(3,F--)' -@=0 -k=+1 -d=6 --comment=' # unique R67-1' -w=1 -e=0.15 -i=1 -w=12
%%
%%
\begin{center}
%
{\includegraphics*[width=40mm, viewport={0 247 595 842}]{3636-unique-r67-1.pdf}}%
{\includegraphics*[width=45mm, viewport={0 247 595 842}]{3636-unique-r67-1-tile-plus.pdf}}%
{\includegraphics*[width=35mm, viewport={0 247 595 842}]{3636-unique-r67-1-tile-minus.pdf}}%
%\hspace*{0mm}% layout
%
\end{center}
\caption{\label{fig:3636-unique-r67-1}
%
Motif of a curve of order 67 (left),
the CCW tile \tileS{F+}{6} (middle),
and the CW tile \tileS{F--}{3}.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/4444-counter-example-curve-r13-x01-decomp.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-rotational-x4.txt
%%
%% zrender -d=4 -a='@L'  -m='L L-R-L+R-L+R+L+R-L+R-L-R+L  R R+L-R-L-R+L+R+L-R-L-R+L+R ' -k=-4 -i=3 -J='L,4,4;R,4,4;'
%% zrender -d=4 -a='+@R' -m='L L-R-L+R-L+R+L+R-L+R-L-R+L  R R+L-R-L-R+L+R+L-R-L-R+L+R ' -k=-4 -i=3 -J='L,4,4;R,4,4;'
%%
\begin{center}
{\includegraphics*[width=50mm, viewport={0 250 595 830}]{4444-counter-example-curve-r13-x01-decomp-L.pdf}}%
\hspace*{2mm}% layout
{\includegraphics*[width=50mm, viewport={0 250 595 830}]{4444-counter-example-curve-r13-x01-decomp-R.pdf}}%
\end{center}
\caption{\label{fig:4444-counter-example-curve-r13-x01-decomp}
Mutual self-similarity of the two curves:
each can be decomposed into smaller copies of both curves.
Coloring by orientation of the small copies.\IMAGENAME%
%The curve on the left has the shape of the black and red regions,
%the curve on the right has the shape of the blue and green regions.
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% was (not really order 13, rather 14):
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%\begin{figure}[h!tbp]
%%%
%%% zrender -d=4 -a='@L' -m='L L-R+L+R-L-R+L+R+L-R-L  R R+L+R-L0+R-L-R-L+0R-L+R+L+R-L-R-L+R' -e=0 -w=2 -k=-4 -i=3
%%% zrender -d=4 -a='+@R' -m='L L-R+L+R-L-R+L+R+L-R-L  R R+L+R-L0+R-L-R-L+0R-L+R+L+R-L-R-L+R' -e=0 -w=2 -k=-4 -i=3
%\begin{center}
%{\includegraphics*[width=60mm, viewport={0 367 595 700}]{4444-counter-example-curve-r13-x01-decomp-L.pdf}}%
%\hspace*{2mm}% layout
%{\includegraphics*[width=60mm, viewport={0 367 595 700}]{4444-counter-example-curve-r13-x01-decomp-R.pdf}}%
%\end{center}
%\caption{\label{fig:4444-counter-example-curve-r13-x01}
%TODO: XXX.\IMAGENAME%
%}
%\end{figure}
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/4444-counter-example-curve-r13-x01-it1.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-rotational-x4.txt
%%
%  zrender -d=4 -a='L' -m='L L-R-L+R-L+R+L+R-L+R-L-R+L  R R+L-R-L-R+L+R+L-R-L-R+L+R ' -e=0.1 -w=15 -k=-4 -i=0 -@=1 -A -L
%  zrender -d=4 -a='_R' -m='L L-R-L+R-L+R+L+R-L+R-L-R+L  R R+L-R-L-R+L+R+L-R-L-R+L+R ' -e=0.1 -w=15 -k=-4 -i=0 -@=1 -A -L --colors-pick=0,4
%%
\begin{center}
{\includegraphics*[width=40mm, viewport={0 310 595 770}]{4444-counter-example-curve-r13-x01-it1-L.pdf}}%
\hspace*{8mm}% layout
{\includegraphics*[width=38mm, viewport={0 300 595 790}]{4444-counter-example-curve-r13-x01-it1-R.pdf}}
%%
\end{center}
\caption{\label{fig:4444-counter-example-curve-r13-x01-it1}
%
First iterates for a curve-set of order 13:
left for the letter \texttt{L}, right for \texttt{R}.
Coloring by orientation of the edges.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% was (not really order 13, rather 14):
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%\begin{figure}[h!tbp]
%%%
%%% zrender -d=4 -a='(2,L+R+)' -m='L L-R+L+R-L-R+L+R+L-R-L  R R+L+R-L0+R-L-R-L+0R-L+R+L+R-L-R-L+R' -e=0.1 -w=15 -k=-4 -i=1 --arrows --letters=0.4
%%% zrender -d=4 -a='(2,L-R-)' -m='L L-R+L+R-L-R+L+R+L-R-L  R R+L+R-L0+R-L-R-L+0R-L+R+L+R-L-R-L+R' -e=0.1 -w=15 -k=-4 -i=1 --arrows --letters=0.4
%%%
%%% zrender -d=4 -a='(2,L+R+)' -m='L L-R+L+R-L-R+L+R+L-R-L  R R+L+R-L0+R-L-R-L+0R-L+R+L+R-L-R-L+R' -e=0 -w=3 -k=-4 -i=3
%%% zrender -d=4 -a='(2,L-R-)' -m='L L-R+L+R-L-R+L+R+L-R-L  R R+L+R-L0+R-L-R-L+0R-L+R+L+R-L-R-L+R' -e=0 -w=3 -k=-4 -i=3 --zoom=0.7
%\begin{center}
%{\includegraphics*[width=30mm, viewport={0 247 595 842}]{4444-counter-example-tile-r13-x01-plus-it1.pdf}}%
%\hspace*{15mm}% layout
%{\includegraphics*[width=40mm, viewport={0 310 595 770}]{4444-counter-example-tile-r13-x01-minus-it1.pdf}}
%%%
%{\includegraphics*[width=50mm, viewport={0 347 595 742}]{4444-counter-example-tile-r13-x01-plus.pdf}}%
%\hspace*{0mm}% layout
%{\includegraphics*[width=50mm, viewport={0 347 595 742}]{4444-counter-example-tile-r13-x01-minus.pdf}}%
%\end{center}
%\caption{\label{fig:4444-counter-example-tile-r13-x01}
%TODO: XXX.\IMAGENAME%
%}
%\end{figure}
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/4444-r29-84-dragon.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%% zrender -d=4 -m='F F+F+F-F-F-F+F+F-F-F-F+F+F-F-F+F+F-F-F+F+F+F-F-F+F+F+F-F-F' -a='(1,F+)' -e=0.1 --id='R29-84' -@=1 -i=0 -k=-1 -w=13 -A=0.3 -L=0.4 -r=-120
%% zrender -d=4 -m='F F+F+F-F-F-F+F+F-F-F-F+F+F-F-F+F+F-F-F+F+F+F-F-F+F+F+F-F-F' -a='(1,F+)' -e=0 --id='R29-84' -@=1 -i=2 -k=-1 -J -r=-70
%%
%%
\begin{center}
%
\begin{subfigure}[b]{61mm}
{\includegraphics*[width=60mm, viewport={20 387 575 702}]{4444-r29-84-dragon-it1.pdf}}
%\vspace*{12mm}% V
\end{subfigure}
%
{\includegraphics*[width=64mm, viewport={0 387 595 702}]{4444-r29-84-dragon-it3.pdf}}%
\hspace*{0mm}% layout
%
%
\end{center}
\caption{\label{fig:4444-r29-84-dragon}
%
First iterate of a curve of order 29 on the square grid (left)
and third iterate as area drawing (right).
Coloring by edges in the first iterate.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/4444-r49-double-manta-it1.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -m='F F+G-F+G+F-G-F-G+F-G-F+G-F+G+F-G-F+G+F+G-F+G+F-G-F+G-F-G-F+G+F+G-F+G-F-G-F+G+F+G-F  G G+F-G+F+G-F-G+F-G-F-G+F+G+F-G-F-G+F-G+F-G+F+G-F-G+F+G-F+G+F+G-F-G-F+G+F+G-F+G-F-G+F-G-F-G+F+G+F-G+F-G-F-G+F+G+F-G' -a='F' -d=4 --comment='' -k=-1 --colors-pick=0,4 -@=1 -i=0 -e=0.15 -w=15 -A=0.3 -L=0.5 -r=90
%%
%% zrender -m='F F+G-F+G+F-G-F-G+F-G-F+G-F+G+F-G-F+G+F+G-F+G+F-G-F+G-F-G-F+G+F+G-F+G-F-G-F+G+F+G-F  G G+F-G+F+G-F-G+F-G-F-G+F+G+F-G-F-G+F-G+F-G+F+G-F-G+F+G-F+G+F+G-F-G-F+G+F+G-F+G-F-G+F-G-F-G+F+G+F-G+F-G-F-G+F+G+F-G' -a='G' -d=4 --comment='' -k=+1 --colors-pick=0,4 -@=1 -i=0 -e=0.15 -w=15 -A=0.3 -L=0.5
%%
%%
\begin{center}
%
{\includegraphics*[width=45mm, viewport={20 270 575 800}]{4444-r49-double-manta-it1-F.pdf}}%
\hspace*{12mm}% layout
%
{\includegraphics*[width=40mm, viewport={55 278 530 805}]{4444-r49-double-manta-it1-G.pdf}}
%
\end{center}
\caption{\label{fig:4444-r49-double-manta-it1}
%
First iterate of the two curves of a curve-set of order 49.
Curves \texttt{F} (left) and \texttt{G} (right).
Coloring by orientation of the edges.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/4444-r49-double-manta.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -m='F F+G-F+G+F-G-F-G+F-G-F+G-F+G+F-G-F+G+F+G-F+G+F-G-F+G-F-G-F+G+F+G-F+G-F-G-F+G+F+G-F  G G+F-G+F+G-F-G+F-G-F-G+F+G+F-G-F-G+F-G+F-G+F+G-F-G+F+G-F+G+F+G-F-G-F+G+F+G-F+G-F-G+F-G-F-G+F+G+F-G+F-G-F-G+F+G+F-G' -a='F' -d=4 --comment='' -k=-1 --colors-pick=0,4 -@=1 -i=2 -J -r=90
%%
%% zrender -m='F F+G-F+G+F-G-F-G+F-G-F+G-F+G+F-G-F+G+F+G-F+G+F-G-F+G-F-G-F+G+F+G-F+G-F-G-F+G+F+G-F  G G+F-G+F+G-F-G+F-G-F-G+F+G+F-G-F-G+F-G+F-G+F+G-F-G+F+G-F+G+F+G-F-G-F+G+F+G-F+G-F-G+F-G-F-G+F+G+F-G+F-G-F-G+F+G+F-G' -a='G' -d=4 --comment='' -k=+1 --colors-pick=0,4 -@=1 -i=2 -J
%%
\begin{center}
%
%
{\includegraphics*[width=45mm, viewport={20 257 575 812}]{4444-r49-double-manta-F.pdf}}%
\hspace*{12mm}% layout
%
{\includegraphics*[width=40mm, viewport={85 257 510 815}]{4444-r49-double-manta-G.pdf}}
%
\end{center}
\caption{\label{fig:4444-r49-double-manta}
%
Fourth iterate of the two curves of a curve-set of order 49.
Curves \texttt{F} (left) and \texttt{G} (right).
Coloring by orientation of the small curves.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/4444-rotational-lr-grid-graph.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=4 -T='L+R,L-R,R+L,R-L' -a='R' --const-maps -e=0 -w=10 -l=,L,R -i=0 -L -A=0.2,0.05 --grid=8 --zoom=1.1
%%
%% zrender -d=4 -a='L+R+L+R-L-R-L' -m="L L  R R" -e=0.1 -w=25 -l=',L,R' -i=0 -L -A='0.2,0.1' --zoom=0.9
%%
%% zrender -d=4 --const-maps -e=0 -w=20 -a='(2,L-R-)' -i=0 --zoom=0.5 --arrows=0.15 --arrow-offset=0.1 --letters -l=',L,R' -r=90
%%
\begin{center}
%
%\fbox{\includegraphics*[width=64.5mm, viewport={15 480 590 830}]{4444-rotational-lr-grid-graph.pdf}}%
\fbox{\includegraphics*[width=64.5mm, viewport={15 490 590 820}]{4444-rotational-lr-grid-graph.pdf}}%
%
%
\hspace*{2mm}% H
%\begin{subfigure}[b]{41mm}
{\includegraphics*[width=20mm, viewport={150 347 435 742}]{4444-rotational-lr-grid-graph-tile-plus.pdf}}
{\includegraphics*[width=20mm, viewport={150 347 435 742}]{4444-rotational-lr-grid-graph-tile-minus.pdf}}
%\vspace*{5mm}% V
%\end{subfigure}%
%
%
\end{center}
\caption{\label{fig:4444-rotational-lr-grid-graph}
%
Coloring of the square grid with two colors (left)
and its two prototiles
\tileS{L+R+}{2} (middle) and
\tileS{L-R-}{2} (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/4444-set-dan-gosper-island-oid.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=4 -a='A+B+C+D' -m='A A-D+A  B B-A+B  C C-B-A+B+C-B+C+D+A-D-C-B+C  D D+A-D+A-D-C-B+C+D' -e=0.1 -w=5 -l -i=6 -J -r=90
%%
%% zrender -d=3 -a='(3,F+)' -m='F F+F-F-F+F+F-F' -i=5 -k=+1 -J --flip -r=10
%%
\begin{center}
%
{\includegraphics*[width=80mm, viewport={0 365 595 702}]{4444-set-dan-gosper-island-oid.pdf}}%
{\includegraphics*[width=48mm, viewport={0 257 595 815}]{4444-set-dan-gosper-island-gosper.pdf}}%
%
\end{center}
\caption{\label{fig:4444-set-dan-gosper-island-oid}
%
Iterate 6 of the CCW prototile of a curve-set of order 7
(left, coloring by curves).
Iterate 6 of the CCW tile of a curve of order 7 on the triangle grid
(right, coloring by orientation of the curves).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/4444-set-dan-terdragon-oid.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=4 -a='_A+B+C+D' -m='A A+B-A  B B+C-B  C C+D+A-D-C  D D' -e=0.1 -w=5 -l -i=10 -P='*4' -J -r=A
%%
%% zrender -d=3 -a='(3,F+)' -m='F F+F-F' -i=9 -k=+1 -J -r=35
%%
\begin{center}
%
{\includegraphics*[width=60mm, viewport={0 255 595 815}]{4444-set-dan-terdragon-oid.pdf}}%
{\includegraphics*[width=60mm, viewport={0 255 595 815}]{4444-set-dan-terdragon-oid-terdragon.pdf}}%
\hspace*{0mm}% layout
%
\end{center}
\caption{\label{fig:4444-set-dan-terdragon-oid}
%
Iterate 10 of the CCW prototile for a curve of order 3 (left).
Iterate 10 of the CCW prototile for terdragon (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/4444-set-dan-twin-ter-oid.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%% zrender -d=4 -T='A+B,A-D,B-A,B+C,C-B,C+D,D+A,D-C' -m='A A-D-C+D-C-B+C+D+A-D+A  B B-A+B-A-D+A+B  C C-B+C-B+C  D D  ' -a='A+B+C+D' --comment=' id = 1453   #simple' -l --fancy-print-maps --colors-pick='1,12' -i=6 -J -r=A
%% zrender -d=4 -T='A+B,A-D,B-A,B+C,C-B,C+D,D+A,D-C' -m='A A-D-C+D-C-B+C+D+A-D+A  B B-A+B-A-D+A+B  C C-B+C-B+C  D D  ' -a='D-C-B-A' --comment=' id = 1453   #simple' -l --fancy-print-maps --colors-pick='1,12' -i=6 -J -r=A
%%
%%
\begin{center}
%
{\includegraphics*[width=60mm, viewport={0 247 595 822}]{4444-set-dan-twin-ter-oid-tile-plus.pdf}}%
{\includegraphics*[width=60mm, viewport={0 247 595 822}]{4444-set-dan-twin-ter-oid-tile-minus.pdf}}%
\hspace*{0mm}% layout
%
\end{center}
\caption{\label{fig:4444-set-dan-twin-ter-oid}
%
Iterate 6 of the CCW (left) and CW  prototile (right)
of a curve-set of order 6.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/4444-set-dan-twindragon-square.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=4 --const-maps -a='A+B+C+D-C-B-A' -l --colors-pick='1,12' -w=20 -e=0 -i=0 -A=0.2,0.1 -L=0.4
%% zrender -d=4 -T='A+B,A-D,B-A,B+C,C-B,C+D,D+A,D-C' -m='A D+A-D-C-B+C+D  B A-D+A+B-A  C B+C-B  D C  ' -a='A+B+C+D-C-B-A' --comment='# id = 42' -l --fancy-print-maps --colors-pick='1,12' -w=3 -e=0.15 -i=7 -@=0 -J
%%
%%
\begin{center}
%
\begin{subfigure}[b]{31mm}
{\includegraphics*[width=30mm, viewport={0 247 595 842}]{4444-set-dan-twindragon-square-axiom.pdf}}
\vspace*{9mm}% V
\end{subfigure}
%
{\includegraphics*[width=80mm, viewport={0 327 575 742}]{4444-set-dan-twindragon-square.pdf}}%
\hspace*{0mm}% layout
%
\end{center}
\caption{\label{fig:4444-set-dan-twindragon-square}
%
A curve-set drawn with the axiom \texttt{A+B+C+D-C-B-A} connecting both prototiles (left).
The seventh iterate of this is shown on the right.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/4444-set-grid.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=4 -a='A+B+C+D' --const-maps -i=0 -w=30 -l -L=0.5 -A=0.15,0.05 --zoom=0.7
%%
%% zrender -d=4 -a='A-D-C-B' --const-maps -i=0 -w=30 -l -L=0.5 -A=0.15,0.05 --zoom=0.7
%%
\begin{center}
%
% boorowd from {fig:grid-colorings-3}
\fbox{\includegraphics*[width=65mm, viewport={70 467 525 772}, page=7]{zout-2x2-uniq.pdf}}%
\hspace*{0mm}% layout
%
\begin{subfigure}[b]{34mm}
\hspace*{6mm}%
{\includegraphics*[width=12mm, viewport={150 247 455 840}]{4444-set-grid-tile-plus.pdf}}%
\hspace*{3mm}%
{\includegraphics*[width=12mm, viewport={150 247 455 840}]{4444-set-grid-tile-minus.pdf}}%
\end{subfigure}
%
\end{center}
\caption{\label{fig:4444-set-grid}
%
A coloring of the square grid using four colors (left)
and
its prototiles \tileS{A+B+C+D+}{1} (middle) and \tileS{A-D-C-B-}{1} (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/4444-star-grid-graph.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-star-x4.txt
%%
%% zrender -d=4 -a='A' -m='A A+B-C-D-A+B+C+D-A+B+C-D-A-B+C-D-A+B-C+D+A+B-C+D-A  B B+C-D-A-B+C+D+A-B+C+D-A-B-C+D-A-B+C-D+A+B+C-D+A-B  C C+D-A-B-C+D+A+B-C+D+A-B-C-D+A-B-C+D-A+B+C+D-A+B-C  D D+A-B-C-D+A+B+C-D+A+B-C-D-A+B-C-D+A-B+C+D+A-B+C-D ' -e=0 -i=0 -@=2 -w=10 -l -L=0.33 -A=0.15 --arrow-offset=0.1 --zoom=3.5
%%
%% zrender -d=4 -a='A+B+C+D' --const-maps -i=0 -w=30 -l -L=0.33 -A=0.15,0.05 --zoom=0.7
%% zrender -d=4 -a='A-B-C-D' --const-maps -i=0 -w=30 -l -L=0.33 -A=0.15,0.05 --zoom=0.7
%%
\begin{center}
%
\fbox{\includegraphics*[width=70mm, viewport={0 527 595 842}]{4444-star-grid-graph.pdf}}%
\hspace*{5mm}% layout
%
\begin{subfigure}[b]{31mm}
{\includegraphics*[width=15mm, viewport={0 247 595 840}]{4444-star-grid-graph-tile-plus.pdf}}%
\vspace*{10mm}%
{\includegraphics*[width=15mm, viewport={0 247 595 840}]{4444-star-grid-graph-tile-minus.pdf}}%
\end{subfigure}
%
\end{center}
\caption{\label{fig:4444-star-grid-graph}
%
A coloring of the square grid with four colors (left).
The prototiles are
 \tileS{A+B+C+D+}{4} and \tileS{A-B-C-D-}{4} (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/4444-star-r05-lattice-tile-plus.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=4 -a='(1,_A-_B+C+D+A-~B-__C-~D+A-___B+C+D+A-~~~B+C-_D+A+B-~~C+D-~)(1,_A-~~~~~~~B+C+D+A-_______B-____C-_D+A-~~~B+C+D+A-___B+C-~D+A+B-~~~~C+D-~)' -m='A A-B+C  B D+A-B-C-D+A-B+C+D+A-B  C C-D+A  D B-C+D' -e=0.15 -w=15 -P='*4' -i=0 -L=0.5 -A=0.25 -r=+45
%%
%% zrender -d=4 -a='(1,_A-_B+C+D+A-~B-__C-~D+A-___B+C+D+A-~~~B+C-_D+A+B-~~C+D-~)(1,_A-~~~~~~~B+C+D+A-_______B-____C-_D+A-~~~B+C+D+A-___B+C-~D+A+B-~~~~C+D-~)' -m='A A-B+C  B D+A-B-C-D+A-B+C+D+A-B  C C-D+A  D B-C+D' -e=0.15 -w=15 -P='*4' -i=4 -J -r=155
%%
\begin{center}
%
{\includegraphics*[width=35mm, viewport={60 300 535 750}]{4444-star-r05-lattice-tile-plus-it1.pdf}}%
{\includegraphics*[width=35mm, viewport={20 280 575 790}]{4444-star-r05-lattice-tile-plus-it.pdf}}%
\fbox{\includegraphics*[width=50mm, viewport={230 480 500 700}]{4444-star-r05-lattice-tile-plus-tiling.pdf}}%
%
\end{center}
\caption{\label{fig:4444-star-r05-lattice-tile-plus}
%
Attempt to decompose the first iterate of the lattice tile
\texttt{A+B+C+D-A+B+C+D-} into smaller copies of itself (left)
and
fourth iterate with this coloring (middle).
Several such tiles, loosely assembled to tile the plane (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/4444-star-r05-lattice-tile.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=4 -a='A-B-C-D+A-B-C-D' -m='A A-B+C  B D+A-B-C-D+A-B+C+D+A-B  C C-D+A  D B-C+D' -e=0.15 -w=15 -l -P='*4' -i=1 -L=0.5 -A=0.25 -r=-90
%%
%% zrender -d=4 -a='(2,A-B+_C-D+A-B-C-D+A-B~+C+___D+A-B-C-D+A-B-C+~~~D+)' -m='A A-B+C  B D+A-B-C-D+A-B+C+D+A-B  C C-D+A  D B-C+D' -e=0.15 -w=5 -P='*4' -@=0 -i=5 --colors-pick=3,12 -J -r=50
%%
%% numsys: radix-m2pi-dragon.png
%%
\begin{center}
%
{\includegraphics*[width=35mm, viewport={50 247 555 802}]{4444-star-r05-lattice-tile-it1.pdf}}%
{\includegraphics*[width=35mm, viewport={80 247 515 820}]{4444-star-r05-lattice-tile-it6.pdf}}%
\hspace*{2mm}% layout
\fbox{\includegraphics*[width=45mm, viewport={35 0 990 1007}]{4444-star-r05-lattice-tile-numsys.png}}%
%
%
\end{center}
\caption{\label{fig:4444-star-r05-lattice-tile}
%
First iterate of the lattice tile with axiom \texttt{A-B-C-D+A-B-C-D},
coloring by curves (left).
Sixth iterate of the lattice tile,
decomposed into smaller copies of itself (middle)
and the corresponding numeration system (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/4444-star-r49-manta-curve-decomp.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-star-x4.txt, curve-set r49-manta
%%
%% zrender -d=4 -a='A' -m='A A+B-C+D+A-B-C-D+A+B-C+D-A-B-C+D-A+B-C+D-A+B+C-D-A+B+C+D-A-B+C-D+A+B+C-D+A-B+C-D-A+B-C-D-A+B+C+D-A+B-C-D-A+B+C+D-A  B B+C-D+A+B-C-D-A+B-C-D+A-B+C+D-A-B+C+D+A-B+C+D-A-B+C-D-A-B+C+D+A-B+C+D-A-B-C+D-A-B+C-D+A+B+C-D+A-B  C C+D-A+B-C+D-A-B-C+D-A+B-C+D+A-B+C-D+A+B+C-D+A-B-C+D-A-B-C+D+A+B-C+D-A-B-C+D+A+B-C  D D+A-B+C+D-A-B-C+D+A-B-C-D+A-B+C-D+A+B-C-D+A+B+C-D-A+B+C+D-A+B-C-D+A-B-C-D+A+B+C-D+A-B-C-D+A+B+C-D ' -e=0.15 -i=1 -l -i=0 -@=1 -w=20 -L=0.5 -A -r=0
%% zrender -d=4 -a='B' -m='A A+B-C+D+A-B-C-D+A+B-C+D-A-B-C+D-A+B-C+D-A+B+C-D-A+B+C+D-A-B+C-D+A+B+C-D+A-B+C-D-A+B-C-D-A+B+C+D-A+B-C-D-A+B+C+D-A  B B+C-D+A+B-C-D-A+B-C-D+A-B+C+D-A-B+C+D+A-B+C+D-A-B+C-D-A-B+C+D+A-B+C+D-A-B-C+D-A-B+C-D+A+B+C-D+A-B  C C+D-A+B-C+D-A-B-C+D-A+B-C+D+A-B+C-D+A+B+C-D+A-B-C+D-A-B-C+D+A+B-C+D-A-B-C+D+A+B-C  D D+A-B+C+D-A-B-C+D+A-B-C-D+A-B+C-D+A+B-C-D+A+B+C-D-A+B+C+D-A+B-C-D+A-B-C-D+A+B+C-D+A-B-C-D+A+B+C-D ' -e=0.15 -i=1 -l -i=0 -@=1 -w=20 -L=0.5 -A -r=90
%% zrender -d=4 -a='C' -m='A A+B-C+D+A-B-C-D+A+B-C+D-A-B-C+D-A+B-C+D-A+B+C-D-A+B+C+D-A-B+C-D+A+B+C-D+A-B+C-D-A+B-C-D-A+B+C+D-A+B-C-D-A+B+C+D-A  B B+C-D+A+B-C-D-A+B-C-D+A-B+C+D-A-B+C+D+A-B+C+D-A-B+C-D-A-B+C+D+A-B+C+D-A-B-C+D-A-B+C-D+A+B+C-D+A-B  C C+D-A+B-C+D-A-B-C+D-A+B-C+D+A-B+C-D+A+B+C-D+A-B-C+D-A-B-C+D+A+B-C+D-A-B-C+D+A+B-C  D D+A-B+C+D-A-B-C+D+A-B-C-D+A-B+C-D+A+B-C-D+A+B+C-D-A+B+C+D-A+B-C-D+A-B-C-D+A+B+C-D+A-B-C-D+A+B+C-D ' -e=0.15 -i=1 -l -i=0 -@=1 -w=20 -L=0.5 -A -r=180
%% zrender -d=4 -a='D' -m='A A+B-C+D+A-B-C-D+A+B-C+D-A-B-C+D-A+B-C+D-A+B+C-D-A+B+C+D-A-B+C-D+A+B+C-D+A-B+C-D-A+B-C-D-A+B+C+D-A+B-C-D-A+B+C+D-A  B B+C-D+A+B-C-D-A+B-C-D+A-B+C+D-A-B+C+D+A-B+C+D-A-B+C-D-A-B+C+D+A-B+C+D-A-B-C+D-A-B+C-D+A+B+C-D+A-B  C C+D-A+B-C+D-A-B-C+D-A+B-C+D+A-B+C-D+A+B+C-D+A-B-C+D-A-B-C+D+A+B-C+D-A-B-C+D+A+B-C  D D+A-B+C+D-A-B-C+D+A-B-C-D+A-B+C-D+A+B-C-D+A+B+C-D-A+B+C+D-A+B-C-D+A-B-C-D+A+B+C-D+A-B-C-D+A+B+C-D ' -e=0.15 -i=1 -l -i=0 -@=1 -w=20 -L=0.5 -A -r=270
%%
%% zrender -d=4 -a='A' -m='A A+B-C+D+A-B-C-D+A+B-C+D-A-B-C+D-A+B-C+D-A+B+C-D-A+B+C+D-A-B+C-D+A+B+C-D+A-B+C-D-A+B-C-D-A+B+C+D-A+B-C-D-A+B+C+D-A  B B+C-D+A+B-C-D-A+B-C-D+A-B+C+D-A-B+C+D+A-B+C+D-A-B+C-D-A-B+C+D+A-B+C+D-A-B-C+D-A-B+C-D+A+B+C-D+A-B  C C+D-A+B-C+D-A-B-C+D-A+B-C+D+A-B+C-D+A+B+C-D+A-B-C+D-A-B-C+D+A+B-C+D-A-B-C+D+A+B-C  D D+A-B+C+D-A-B-C+D+A-B-C-D+A-B+C-D+A+B-C-D+A+B+C-D-A+B+C+D-A+B-C-D+A-B-C-D+A+B+C-D+A-B-C-D+A+B+C-D ' -e=0.2 -i=1 -l -i=2 -@=1 -J='*4' -r=0
%% zrender -d=4 -a='B' -m='A A+B-C+D+A-B-C-D+A+B-C+D-A-B-C+D-A+B-C+D-A+B+C-D-A+B+C+D-A-B+C-D+A+B+C-D+A-B+C-D-A+B-C-D-A+B+C+D-A+B-C-D-A+B+C+D-A  B B+C-D+A+B-C-D-A+B-C-D+A-B+C+D-A-B+C+D+A-B+C+D-A-B+C-D-A-B+C+D+A-B+C+D-A-B-C+D-A-B+C-D+A+B+C-D+A-B  C C+D-A+B-C+D-A-B-C+D-A+B-C+D+A-B+C-D+A+B+C-D+A-B-C+D-A-B-C+D+A+B-C+D-A-B-C+D+A+B-C  D D+A-B+C+D-A-B-C+D+A-B-C-D+A-B+C-D+A+B-C-D+A+B+C-D-A+B+C+D-A+B-C-D+A-B-C-D+A+B+C-D+A-B-C-D+A+B+C-D ' -e=0.2 -i=1 -l -i=2 -@=1 -J='*4' -r=90
%% zrender -d=4 -a='C' -m='A A+B-C+D+A-B-C-D+A+B-C+D-A-B-C+D-A+B-C+D-A+B+C-D-A+B+C+D-A-B+C-D+A+B+C-D+A-B+C-D-A+B-C-D-A+B+C+D-A+B-C-D-A+B+C+D-A  B B+C-D+A+B-C-D-A+B-C-D+A-B+C+D-A-B+C+D+A-B+C+D-A-B+C-D-A-B+C+D+A-B+C+D-A-B-C+D-A-B+C-D+A+B+C-D+A-B  C C+D-A+B-C+D-A-B-C+D-A+B-C+D+A-B+C-D+A+B+C-D+A-B-C+D-A-B-C+D+A+B-C+D-A-B-C+D+A+B-C  D D+A-B+C+D-A-B-C+D+A-B-C-D+A-B+C-D+A+B-C-D+A+B+C-D-A+B+C+D-A+B-C-D+A-B-C-D+A+B+C-D+A-B-C-D+A+B+C-D ' -e=0.2 -i=1 -l -i=2 -@=1 -J='*4' -r=180
%% zrender -d=4 -a='D' -m='A A+B-C+D+A-B-C-D+A+B-C+D-A-B-C+D-A+B-C+D-A+B+C-D-A+B+C+D-A-B+C-D+A+B+C-D+A-B+C-D-A+B-C-D-A+B+C+D-A+B-C-D-A+B+C+D-A  B B+C-D+A+B-C-D-A+B-C-D+A-B+C+D-A-B+C+D+A-B+C+D-A-B+C-D-A-B+C+D+A-B+C+D-A-B-C+D-A-B+C-D+A+B+C-D+A-B  C C+D-A+B-C+D-A-B-C+D-A+B-C+D+A-B+C-D+A+B+C-D+A-B-C+D-A-B-C+D+A+B-C+D-A-B-C+D+A+B-C  D D+A-B+C+D-A-B-C+D+A-B-C-D+A-B+C-D+A+B-C-D+A+B+C-D-A+B+C+D-A+B-C-D+A-B-C-D+A+B+C-D+A-B-C-D+A+B+C-D ' -e=0.2 -i=1 -l -i=2 -@=1 -J='*4' -r=270
%%
\begin{center}
%
{\includegraphics*[width=32mm, viewport={0 247 595 842}]{4444-star-r49-manta-curve-decomp-A-it1.pdf}}%
{\includegraphics*[width=32mm, viewport={0 247 595 842}]{4444-star-r49-manta-curve-decomp-B-it1.pdf}}%
{\includegraphics*[width=32mm, viewport={0 247 595 842}]{4444-star-r49-manta-curve-decomp-C-it1.pdf}}%
{\includegraphics*[width=32mm, viewport={0 247 595 842}]{4444-star-r49-manta-curve-decomp-D-it1.pdf}}
%\hspace*{0mm}% layout
%
{\includegraphics*[width=32mm, viewport={0 247 595 842}]{4444-star-r49-manta-curve-decomp-A-it3.pdf}}%
{\includegraphics*[width=32mm, viewport={0 247 595 842}]{4444-star-r49-manta-curve-decomp-B-it3.pdf}}%
{\includegraphics*[width=32mm, viewport={0 247 595 842}]{4444-star-r49-manta-curve-decomp-C-it3.pdf}}%
{\includegraphics*[width=32mm, viewport={0 247 595 842}]{4444-star-r49-manta-curve-decomp-D-it3.pdf}}%
%
\end{center}
\caption{\label{fig:4444-star-r49-manta-curve-decomp}
Mutual self-similarity of the curves (from left to right)
\texttt{A} (small copies black),
\texttt{B} (small copies blue),
\texttt{C} (small copies red), and
\texttt{D} (small copies green).
First iterates in top row, third iterates in bottom row.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/4444-translational-decomp.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%%% translational-r25-2:
%%% not rotated:
%% zrender -d=4 -m='F F+F+F-G-F+F-G-F-G+G+G-F+F-G-F-G+G+G+G-F+F+F-G+G-F  G G-F+F-G+G+G-F+F+F-G-F+F+F-G-F-G+G+G-F-G-F+F-G+G+G ' -a='@F' -e=0.5 -k=-1 -w=8 -i=2 -J='F,4,4;G,4,4;'
%% zrender -d=4 -m='F F+F+F-G-F+F-G-F-G+G+G-F+F-G-F-G+G+G+G-F+F+F-G+G-F  G G-F+F-G+G+G-F+F+F-G-F+F+F-G-F-G+G+G-F-G-F+F-G+G+G ' -a='_@G' -e=0.5 -k=-1 -w=8 -i=2 -J='F,4,4;G,4,4;'
%%
\begin{center}
%
{\includegraphics*[width=58mm, viewport={0 247 595 842}]{4444-translational-decomp-F.pdf}}%
\hspace*{0mm}% layout
%
{\includegraphics*[width=68mm, viewport={0 275 595 790}]{4444-translational-decomp-G.pdf}}
\end{center}
\caption{\label{fig:4444-translational-decomp}
Mutual self-similarity of the curves
\texttt{F} (left) and \texttt{G} (right).
Coloring cycling through 12 colors in the small copies.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% rotated:
%% zrender -d=4 -m='F F+F+F-G-F+F-G-F-G+G+G-F+F-G-F-G+G+G+G-F+F+F-G+G-F  G G-F+F-G+G+G-F+F+F-G-F+F+F-G-F-G+G+G-F-G-F+F-G+G+G ' -a='@F' -e=0.5 -k=-1 -w=8 -i=2 -r=+45
%% zrender -d=4 -m='F F+F+F-G-F+F-G-F-G+G+G-F+F-G-F-G+G+G+G-F+F+F-G+G-F  G G-F+F-G+G+G-F+F+F-G-F+F+F-G-F-G+G+G-F-G-F+F-G+G+G ' -a='_@G' -e=0.5 -k=-1 -w=8 -i=2 -r=-45

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/4444-translational-grid-graph.tex <==



%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=4 -m='F F  G G  t t ' -a='_(4,(6,G+G-F-G+)t+t+(6,G-F+F+F-)t-t-)' -e=0 -w=10 -l -i=0 -L=0.4 --arrows --arrow-offset=0.05 --zoom=2
%%
%% zrender -d=4 -m='F F  G G ' -e=0 -w=40 -a='_(4,F+)' -i=0 --zoom=0.5 --arrows=0.15 --arrow-offset=0.1 --letters -l
%% zrender -d=4 -m='F F  G G ' -e=0 -w=40 -a='_(4,G+)' -i=0 --zoom=0.5 --arrows=0.15 --arrow-offset=0.1 --letters -l
%% zrender -d=4 -m='F F  G G ' -e=0 -w=40 -a='_(2,F-G-)' -i=0 --zoom=0.5 --arrows=0.15 --arrow-offset=0.1 --letters -l
%%
\begin{center}
%
%{\includegraphics*[width=60mm, viewport={0 377 595 802}]{4444-translational-grid-graph.pdf}}
%\fbox{\includegraphics*[width=60mm, viewport={0 377 595 802}]{4444-translational-grid-graph.pdf}}
\fbox{\includegraphics*[width=60mm, viewport={0 437 595 802}]{4444-translational-grid-graph.pdf}}
%
\hspace*{2mm}% H
\begin{subfigure}[b]{60mm}
{\includegraphics*[width=20mm, viewport={0 247 595 842}]{4444-translational-prototile-F4-it0.pdf}}%
{\includegraphics*[width=20mm, viewport={0 247 595 842}]{4444-translational-prototile-G4-it0.pdf}}%
{\includegraphics*[width=20mm, viewport={0 247 595 842}]{4444-translational-prototile-FGFG-it0.pdf}}
\vspace*{5mm}% V
\end{subfigure}%
%
%{\includegraphics*[width=20mm, viewport={0 0 595 842}]{4444-translational-outline.pdf}}
%
\end{center}
\caption{\label{fig:4444-translational-grid-graph}
%
Coloring of the square grid with two colors (left)
and its three prototiles (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/4444-translational-motif.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=4 -m='F F+F+F-G-F+F-G-F-G+G+G-F+F-G-F-G+G+G+G-F+F+F-G+G-F G G-F+F-G+G+G-F+F+F-G-F+F+F-G-F-G+G+G-F-G-F+F-G+G+G ' -a='_@F' -e=0.1 -l -w=15 -i=0 -L=0.5 -A
%% zrender -d=4 -m='F F+F+F-G-F+F-G-F-G+G+G-F+F-G-F-G+G+G+G-F+F+F-G+G-F G G-F+F-G+G+G-F+F+F-G-F+F+F-G-F-G+G+G-F-G-F+F-G+G+G ' -a='_@G' -e=0.1 -l -w=15 -i=0 -L=0.5 -A
%%
\begin{center}
%
{\includegraphics*[width=35mm, viewport={0 295 595 812}]{4444-translational-motif-F.pdf}}%
\hspace*{15mm}% layout
{\includegraphics*[width=40mm, viewport={0 320 595 770}]{4444-translational-motif-G.pdf}}
%
\end{center}
\caption{\label{fig:4444-translational-motif}
%
Motifs for the two curves for
\texttt{F} (left) and \texttt{G} (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/4444-translational-r25-3s-tiles-plus.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=4 -m='F G-F+F-G-F-G+G+G-F+F-G-F+F+F+F-G+G  G F-G-F+F-G+G+G-F0-G+G+G+G-0F+F-G-F+F+F-G-F-G+G+G-F-G-F+F-G+G+G-F+F+F ' -a='(4,F+)' -e=0.1 -l --colors-pick=1,2 -w=3 -@=1 -i=2 -J='*4' --fancy-print-maps
%%
%% zrender -d=4 -m='F G-F+F-G-F-G+G+G-F+F-G-F+F+F+F-G+G  G F-G-F+F-G+G+G-F0-G+G+G+G-0F+F-G-F+F+F-G-F-G+G+G-F-G-F+F-G+G+G-F+F+F ' -a='(4,G+)' -e=0.1 -l --colors-pick=1,2 -w=3 -@=1 -i=2 -J='*4' --fancy-print-maps
%%
\begin{center}
%
{\includegraphics*[width=64.5mm, viewport={0 257 595 812}]{4444-translational-r25-3s-tiles-plus-F.pdf}}%
\hspace*{0mm}% layout
{\includegraphics*[width=64.5mm, viewport={0 257 595 812}]{4444-translational-r25-3s-tiles-plus-G.pdf}}%
%
%\begin{subfigure}[b]{21mm}
%\fbox{\includegraphics*[width=20mm, viewport={0 247 595 842}]{4444-translational-r25-3s-tiles-plus.pdf}}
%\vspace*{12mm}% V
%\end{subfigure}
%
%
\end{center}
\caption{\label{fig:4444-translational-r25-3s-tiles-plus}
%
Mutual self-similarity of the CCW prototiles of a curve-set.
Small copies of the left and right prototile respectively in blue and red.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/4444-translational-tile-FGFG-self-sim.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%%% file 00lsys-translational-x4.txt , translational-r25-2:
%%
%% zrender -d=4 -m='F F+F+F-G-F+F-G-F-G+G+G-F+F-G-F-G+G+G+G-F+F+F-G+G-F  G G-F+F-G+G+G-F+F+F-G-F+F+F-G-F-G+G+G-F-G-F+F-G+G+G ' -a='(2,F-G-)' -@=1  -e=0 -w=3 -i=2 -t='+,' --colors-pick=1,2 -J='*4' -r=+45
%%
\begin{center}
%
%{\includegraphics*[width=90mm, viewport={0 257 595 812}]{4444-translational-tile-FGFG-self-sim.pdf}}%
{\includegraphics*[width=90mm, viewport={0 357 595 712}]{4444-translational-tile-FGFG-self-sim.pdf}}%
%
\end{center}
\caption{\label{fig:4444-translational-tile-FGFG-self-sim}
The CW prototile \tileS{F-G-}{2} is self-similar and tiles the plane.\IMAGENAME%
%Splitting by both the horizontal and vertical lines through the center
%gives the decomposition into four curves.
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% rot:
%% zrender -d=4 -m='F F+F+F-G-F+F-G-F-G+G+G-F+F-G-F-G+G+G+G-F+F+F-G+G-F  G G-F+F-G+G+G-F+F+F-G-F+F+F-G-F-G+G+G-F-G-F+F-G+G+G ' -a='(2,@F-@G-)' -e=0.5 -w=4 -i=2 -k=-1 -r=+45 -J='F,4,4;G,4,4;'
%% zrender -d=4 -m='F F+F+F-G-F+F-G-F-G+G+G-F+F-G-F-G+G+G+G-F+F+F-G+G-F  G G-F+F-G+G+G-F+F+F-G-F+F+F-G-F-G+G+G-F-G-F+F-G+G+G ' -a='(2,@F-@G-)' -e=0.5 -w=4 -i=2 -k=-1
%%% decomp:
%% zrender -d=4 -m='F F+F+F-G-F+F-G-F-G+G+G-F+F-G-F-G+G+G+G-F+F+F-G+G-F  G G-F+F-G+G+G-F+F+F-G-F+F+F-G-F-G+G+G-F-G-F+F-G+G+G ' -a='(2,@F-@G-)' -e=0.5 -w=4 -i=2 -t='+,' -r=+45 --colors-pick=1,2 -J='F,4,4;G,4,4;'

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d31212-grid.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -a='B' --const-maps -T='A!A,B!b,b!B,A+B,A-b,B+A,B----B,b++++b,b-A' -w=7 -e=0.1 -i=4 -@=1 -l=',A,bB' -L=0.4 --letters-mv=0.45,0.15 -A=0.3,0.1 -H=L --grid --zoom=1.5
%%
%%  zrender -d=12 -a='B' --const-maps -T='A!A,B!b,b!B,A+B,A-b,B+A,B----B,b++++b,b-A' -w=7 -e=0.1 -i=4 -@=0 -l=',A,B,b' -L=0.4 --letters-mv=0.45,0.15 --grid --zoom=1.5 -B=3,0.7 -P='A,12,0;B,12,0;b,3,0;' -J
%%
\begin{center}
%
\fbox{\includegraphics*[width=63mm, viewport={0 500 500 842}]{d31212-grid.pdf}}%
\hspace*{3mm}% layout
\fbox{\includegraphics*[width=63mm, viewport={0 500 500 842}]{d31212-grid-area.pdf}}%
%
%
\end{center}
\caption{\label{fig:d31212-grid}
%
The $(3.12.12)$ grid with double edges.
Line drawing with letters \texttt{A} blue,
\texttt{b} and \texttt{B} red (left).
Area drawing with letters \texttt{A} blue,
\texttt{B} red, and \texttt{b} green (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d31212-r27-var0-curves-it.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -a=':A:' -T='A!A,B!b,b!B,A+B,A-b,B+A,B----B,b++++b,b-A' --colors-pick=1,12 --letters-mv=0.45,0.15 -m='A ABbbbABbbbAABAABABABAABbbbABABA  B BABABBbbbABABBbbbABBbbbAABABABBbbbABABAB  b bbBAbbbBAb' -P='A,12,0;B,12,0;b,3,0;' -@=0 -l -w=12 -A=0.35,0.15 -H=L --margin=0.01 -J -r=70 -i=3
%%
%%  zrender -d=12 -a=':B:' -T='A!A,B!b,b!B,A+B,A-b,B+A,B----B,b++++b,b-A' --colors-pick=1,12 --letters-mv=0.45,0.15 -m='A ABbbbABbbbAABAABABABAABbbbABABA  B BABABBbbbABABBbbbABBbbbAABABABBbbbABABAB  b bbBAbbbBAb' -P='A,12,0;B,12,0;b,3,0;' -@=0 -i=3 -l -w=12 -A=0.35,0.15 -H=L --margin=0.01 -J -r=60
%%
%%  zrender -d=12 -a=':b:' -T='A!A,B!b,b!B,A+B,A-b,B+A,B----B,b++++b,b-A' --colors-pick=1,12 --letters-mv=0.45,0.15 -m='A ABbbbABbbbAABAABABABAABbbbABABA  B BABABBbbbABABBbbbABBbbbAABABABBbbbABABAB  b bbBAbbbBAb' -P='A,12,0;B,12,0;b,3,0;' -@=0 -l -w=12 -A=0.35,0.15 -H=L --margin=0.01 -J -r=+53 -i=3
%%
\begin{center}
%
%
\begin{subfigure}[b]{130mm}
{\includegraphics*[width=40mm, viewport={0 247 595 840}]{d31212-r27-var0-curves-it-A.pdf}}%
{\includegraphics*[width=40mm, viewport={0 247 595 840}]{d31212-r27-var0-curves-it-B.pdf}}%
{\includegraphics*[width=40mm, viewport={0 247 595 840}]{d31212-r27-var0-curves-it-b.pdf}}
\end{subfigure}
%
\end{center}
\caption{\label{fig:d31212-r27-var0-curves-it}
Area drawing of the third iterates of
\texttt{A} (left),
\texttt{B} (middle), and
\texttt{b} (right).\IMAGENAME%
%Coloring by axiom.
%Start and end of curves marked.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d31212-r27-var0-curves.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%  zrender -d=12 -a=':B:' -T='A!A,B!b,b!B,A+B,A-b,B+A,B----B,b++++b,b-A' --colors-pick=1,12 --letters-mv=0.45,0.15 -m='A ABbbbABbbbAABAABABABAABbbbABABA  B BABABBbbbABABBbbbABBbbbAABABABBbbbABABAB  b bbBAbbbBAb' -P='A,12,0;B,12,0;b,3,0;' -@=0 -i=1 -l -w=12 -A=0.35,0.15 -H=L -L=0.4 --margin=0.01
%%
%%
\begin{center}
%
%
\begin{subfigure}[b]{130mm}
{\includegraphics*[width=43mm, viewport={0 247 595 822}]{d31212-r27-var0-curves-A-it1.pdf}}%
{\includegraphics*[width=43mm, viewport={0 247 595 822}]{d31212-r27-var0-curves-B-it1.pdf}}%
{\includegraphics*[width=43mm, viewport={0 247 595 822}]{d31212-r27-var0-curves-b-it1.pdf}}
\end{subfigure}
%
\end{center}
\caption{\label{fig:d31212-r27-var0-curves}
First iterates of curve
\texttt{A} (left),
\texttt{B} (middle), and
\texttt{b} (right).
Coloring by axiom.
Start and end of curves marked.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d31212-r27-var0-digons.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -a='(2,A!_~)' -T='A!A,B!b,b!B,A+B,A-b,B+A,B----B,b++++b,b-A' --colors-pick=1,12 --letters-mv=0.45,0.15 -m='A ABbbbABbbbAABAABABABAABbbbABABA  B BABABBbbbABABBbbbABBbbbAABABABBbbbABABAB  b bbBAbbbBAb' -P='A,12,0;B,12,0;b,3,0;' -@=0 -l -w=12 -A=0.35,0.15 -H=L --margin=0.01 -J -r=0 -i=3 -B=5,0.9
%%
%% zrender -d=12 -a='(1,B!b!)' -T='A!A,B!b,b!B,A+B,A-b,B+A,B----B,b++++b,b-A' --colors-pick=1,12 --letters-mv=0.45,0.15 -m='A ABbbbABbbbAABAABABABAABbbbABABA  B BABABBbbbABABBbbbABBbbbAABABABBbbbABABAB  b bbBAbbbBAb' -P='A,12,0;B,12,0;b,3,0;' -@=0 -l -w=12 -A=0.35,0.15 -H=L --margin=0.01 -J -r=25 -i=3 -B=5,0.9
%%
\begin{center}
%
{\includegraphics*[width=45mm, viewport={0 340 595 742}]{d31212-r27-var0-digons-AA.pdf}}%
\hspace*{10mm}% layout
{\includegraphics*[width=45mm, viewport={0 340 595 742}]{d31212-r27-var0-digons-Bb.pdf}}%
%
%
\end{center}
\caption{\label{fig:d31212-r27-var0-digons}
The CW (digon) tiles \tileS{A!}{2} (left) and \tileS{B!b!}{1} (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d31212-r27-var0-tiles-plus-big-AB6.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%% 3. it (axiom expanded by hand):
%%  zrender -d=12 -a='(6,,A+B!b++++b++++b-A+B!b++++b++++b-A_!~A+B+A_!~A+B+A+B+A+B+A_!~A+B!b++++b++++b-A+B+A+B+A+,B+A+B+A+B----B!b++++b++++b-A+B+A+B----B!b++++b++++b-A+B----B!b++++b++++b-A_!~A+B+A+B+A+B----B!b++++b++++b-A+B+A+B+A+B+)' -T='A!A,B!b,b!B,A+B,A-b,B+A,B----B,b++++b,b-A' -w=3 --colors-pick=1,12 --letters-mv=0.45,0.15 -m='A ABbbbABbbbAABAABABABAABbbbABABA  B BABABBbbbABABBbbbABBbbbAABABABBbbbABABAB  b bbBAbbbBAb' -P='A,12,0;B,12,0;b,3,0;' -J -@=0 -i=2 -l -B=2,0.7 --margin=0.01
%%
%%
\begin{center}
%
{\includegraphics*[width=129mm, viewport={0 255 595 828}]{d31212-r27-var0-tiles-plus-AB6.pdf}}
%
%
\end{center}
\caption{\label{fig:d31212-r27-var0-tiles-plus-big-AB6}
The CCW tile \tileS{A+B+}{6},
decomposed into copies if itself (blue and red)
and copies of \tileS{b++++}{3} (green).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d31212-r27-var0-tiles-plus-big-b3.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%% 4. it:
%%  zrender -d=12 -a='(3,b++++)' -T='A!A,B!b,b!B,A+B,A-b,B+A,B----B,b++++b,b-A' -w=3 --colors-pick=1,12 --letters-mv=0.45,0.15 -m='A ABbbbABbbbAABAABABABAABbbbABABA  B BABABBbbbABABBbbbABBbbbAABABABBbbbABABAB  b bbBAbbbBAb' -P='A,12,0;B,12,0;b,3,0;' -J -@=1 -i=3 -l -B=2,0.7 --margin=0.01
%%
%%
\begin{center}
%
{\includegraphics*[width=70mm, viewport={0 270 595 810}]{d31212-r27-var0-tiles-plus-b3.pdf}}
%
%
\end{center}
\caption{\label{fig:d31212-r27-var0-tiles-plus-big-b3}
The CCW tile \tileS{b++++}{3},
decomposed into
one copy of the CCW tile \tileS{A+B+}{6} (blue and red)
and six copies of itself (green).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d31212-r27-var0-tiles-plus-small.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=12 -a='(3,b++++)' -T='A!A,B!b,b!B,A+B,A-b,B+A,B----B,b++++b,b-A' -w=3 --colors-pick=1,12 --letters-mv=0.45,0.15 -m='A ABbbbABbbbAABAABABABAABbbbABABA  B BABABBbbbABABBbbbABBbbbAABABABBbbbABABAB  b bbBAbbbBAb' -P='A,12,0;B,12,0;b,3,0;' -J -@=0 -i=3 -l -B=5,0.7 --margin=0.01
%%
%% zrender -d=12 -a='(6,A+B+)' -T='A!A,B!b,b!B,A+B,A-b,B+A,B----B,b++++b,b-A' -w=3 --colors-pick=1,12 --letters-mv=0.45,0.15 -m='A ABbbbABbbbAABAABABABAABbbbABABA  B BABABBbbbABABBbbbABBbbbAABABABBbbbABABAB  b bbBAbbbBAb' -P='A,12,0;B,12,0;b,3,0;' -J -@=0 -i=3 -l -B=5,0.7 --margin=0.01
%%
\begin{center}
%
{\includegraphics*[width=40mm, viewport={0 247 595 842}]{d31212-r27-var0-tiles-plus-small-b3.pdf}}%
\hspace*{10mm}% layout
{\includegraphics*[width=40mm, viewport={0 247 595 842}]{d31212-r27-var0-tiles-plus-small-AB6.pdf}}%
%
%
\end{center}
\caption{\label{fig:d31212-r27-var0-tiles-plus-small}
The CCW tiles \tileS{b++++}{3} (left) and \tileS{A+B+}{6} (right).
Coloring by letters in the axioms.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d333333-AB-grid.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -T='A++A, A0A, A!B, B++B, B0B, B!A' --const-maps -w=3 -a='A' -A=0.25,0.15 -H=L -w=10 --letters-mv='0.45,0.15' -L=0.3 --zoom=1.8 --shift-y=-0.1 --grid=8,8
%%
%% zrender -d=6 -T='A++A, A0A, A!B, B++B, B0B, B!A' --const-maps -w=3 -a='A' --colors-pick=1,6 --zoom=1.8 --shift-y=-0.1 -l --grid=8,8 -J='*,3,0;'
%%
\begin{center}
%
\fbox{\includegraphics*[width=60mm, viewport={0 455 595 842}]{d333333-AB-grid.pdf}}%
\hspace*{3mm}% layout
\fbox{\includegraphics*[width=60mm, viewport={0 455 595 842}]{d333333-AB-grid-area.pdf}}%
%

\end{center}
\caption{\label{fig:d333333-AB-grid}
%
Coloring the triangle grid with double edges using two colors.
Line drawing (left) and area drawing (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d333333-AB-r13-var00-build.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -a='(3,A++)--!(3,B++)' -m='A A0A-B+A  B B-A+B0B' -A=0.25,0 -L --letters-mv='0.45,0.15' -H=L -l=',A,B' -e=0 -w=13
%%
%% zrender -d=6 -a='(3,A++)--!(3,B++)' -m='A A++A!B++B!A++A++A!B0B+A  B B++B!A++A!B++B!A++A+B++B++B!A+B!A0A+B' -w=13 -A=0.25,0 -L --letters-mv='0.45,0.15' -H=L -l=',A,B' -e=0.12
%%
\begin{center}
%
{\includegraphics*[width=50mm, viewport={0 317 595 760}]{d333333-AB-r13-var00-build-border.pdf}}%
\hspace*{3mm}% layout
{\includegraphics*[width=50mm, viewport={0 317 595 760}]{d333333-AB-r13-var00-build-filled.pdf}}%
%
\end{center}
\caption{\label{fig:d333333-AB-r13-var00-build}
%
Borders of the CCW tiles
\tileS{A++}{3} (blue) and \tileS{B++}{3} (red),
drawn side by side (left).
Filling the tiles gives the curves (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d333333-AB-r13-var00-tile-minus-decomp.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -a='A!B' -m='A A++A!B++B!A++A++A!B0B+A  B B++B!A++A!B++B!A++A+B++B++B!A+B!A0A+B' -w=5 -k=+6 -e=0.1 -@=1 -i=0 -J='*,3,0;' -r=-60
%%
%% zrender -d=6 -a='A!B' -m='A A++A!B++B!A++A++A!B0B+A  B B++B!A++A!B++B!A++A+B++B++B!A+B!A0A+B' -w=5 -k=+6 -e=0.1 -@=1 -i=3 -J='*,3,0;'
%%
%% zrender -d=6 -a='A!B' -m='A A++A!B++B!A++A++A!B0B+A  B B++B!A++A!B++B!A++A+B++B++B!A+B!A0A+B' -w=5 -k=+6 -e=0.1 -@=0 -i=3 -J='*,3,0;'
%% zrender -d=6 -a='++A!B' -m='A A++A!B++B!A++A++A!B0B+A  B B++B!A++A!B++B!A++A+B++B++B!A+B!A0A+B' -w=5 -k=+6 -e=0.1 -@=0 -i=3 -J='*,3,0;'
%% zrender -d=6 -a='--A!B' -m='A A++A!B++B!A++A++A!B0B+A  B B++B!A++A!B++B!A++A+B++B++B!A+B!A0A+B' -w=5 -k=+6 -e=0.1 -@=0 -i=3 -J='*,3,0;'
%%
%%
\begin{center}
%
{\includegraphics*[width=45mm, viewport={140 255 460 820}]{d333333-AB-r13-var00-tile-minus-decomp-it1.pdf}}%
\hspace*{3mm}% layout
%
{\includegraphics*[width=45mm, viewport={140 255 460 820}]{d333333-AB-r13-var00-tile-minus-decomp-it4.pdf}}%
\hspace*{3mm}% layout
%
\begin{subfigure}[b]{31mm}
{\includegraphics*[width=26mm, viewport={0 257 595 822}]{d333333-AB-r13-var00-tile-minus-decomp-it3-1.pdf}}%
\vspace*{3mm}
{\includegraphics*[width=26mm, viewport={0 247 595 822}]{d333333-AB-r13-var00-tile-minus-decomp-it3-2.pdf}}%
\vspace*{3mm}
{\includegraphics*[width=26mm, viewport={0 347 595 742}]{d333333-AB-r13-var00-tile-minus-decomp-it3-3.pdf}}%
\vspace*{3mm}
\end{subfigure}
%
\end{center}
\caption{\label{fig:d333333-AB-r13-var00-tile-minus-decomp}
%
Area drawing of the first iterate of the CW (digon) tile \tileS{A!B}{2} (left).
The third iterate (middle),
decomposed into 13 copies of the second iterate,
each colored by orientation (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d333333-AB-r13-var00-tile-plus-decomp.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -a='(3,A++)' -m='A A++A!B++B!A++A++A!B0B+A  B B++B!A++A!B++B!A++A+B++B++B!A+B!A0A+B' -w=5 -k=+2 -e=0.1 -@=1 -i=3 -J='*,3,0;'
%%
%% zrender -d=6 -a='+(3,B++)' -m='A A++A!B++B!A++A++A!B0B+A  B B++B!A++A!B++B!A++A+B++B++B!A+B!A0A+B' -w=5 -k=+2 -e=0.1 -@=1 -i=3 -J='*,3,0;'
%%
\begin{center}
%
{\includegraphics*[width=50mm, viewport={0 267 595 842}]{d333333-AB-r13-var00-tile-plus-decomp-AAA.pdf}}%
\hspace*{8mm}% layout
{\includegraphics*[width=60mm, viewport={0 267 595 805}]{d333333-AB-r13-var00-tile-plus-decomp-BBB.pdf}}%
%
%
\end{center}
\caption{\label{fig:d333333-AB-r13-var00-tile-plus-decomp}
%
Mutual self-similarity of the CCW tiles:
\tileS{A++}{3} (left, small copies in blue)
and
\tileS{B++}{3} (right, small copies in red).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d333333-curve-r13-1-digon.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%% zrender -i=0 -m='A A0A++A0A0A--A++A--A--A0A++A++A--A  B B++B--B--B0B++B++B--B++B0B0B--B0B' -a='A!B' -@=1 -d=6 -e=0.1 -l=',A,B' -w=15 --id='R13-1' -A=0.15 -J='*3,0'
%%
%% zrender -i=0 -m='A A0A++A0A0A--A++A--A--A0A++A++A--A  B B++B--B--B0B++B++B--B++B0B0B--B0B' -a='A!B' -@=1 -d=6 -e=0.1 -l=',A,B' -w=15 --id='R13-1' -J='*3,0' -i=1 -r=-46.6
%%
% % zrender -i=0 -m='A A0A++A0A0A--A++A--A--A0A++A++A--A  B B++B--B--B0B++B++B--B++B0B0B--B0B' -a='A!B' -@=1 -d=6 -e=0.1 -w=15 --id='R13-1' -J='*3,0' -@=1 -i=1 -k=-6 -r=-46.6 --colors-pick=1,6
%%
\begin{center}
%
{\includegraphics*[width=35mm, viewport={100 270 495 800}]{d333333-curve-r13-1-digon-it1.pdf}}%
\hspace*{7mm}% layout
{\includegraphics*[width=35mm, viewport={100 270 495 800}]{d333333-curve-r13-1-digon-it2.pdf}}%
\hspace*{7mm}% layout
{\includegraphics*[width=35mm, viewport={100 270 495 800}]{d333333-curve-r13-1-digon-it2-decomp.pdf}}%
%
\end{center}
\caption{\label{fig:d333333-curve-r13-1-digon}
First (left) and second (middle) iterate of a digon tile,
colored by letters.
Second iterate decomposed into first iterates,
colored by orientations (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d333333-curve-r13-1-solid.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -i=0 -m='A A0A+A0A0A-A+A-A-A0A+A+A-A' -a='A' -@=1 -d=3  -e=0.1 -k=-1 -w=15 --id='R13-1' -A=0.25,0.1 -H=L
%%
%% zrender -i=0 -m='A A0A+A0A0A-A+A-A-A0A+A+A-A' -a='A' -@=1 -d=3  -e=0.1 -k=-1 -w=15 --id='R13-1' -A=0.15 -J='*3,0'
%%
%%
\begin{center}
%
{\includegraphics*[width=40mm, viewport={50 310 545 805}]{d333333-curve-r13-1-solid-line-it1.pdf}}
\hspace*{1mm}% H
%
{\includegraphics*[width=40mm, viewport={50 310 545 805}]{d333333-curve-r13-1-solid-it1.pdf}}
%
\end{center}
\caption{\label{fig:d333333-curve-r13-1-solid}
First iterate of a curve on the triangle grid with double edges:
line drawing (left) and area drawing (right).
Areas are on the left of the edges.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d333333-grid-graph.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -m='A A++A!A++A++A!A++A++A!A++A-A-A-A ' -e=0 -a='(6,A(1,++A!A+)+)' -i=2 -A --zoom=5 --shift-y=-0.1 -w=10 -A=0.2,0.2 -H=L
%%
%% zrender -d=6 -m='A A++A!A++A++A!A++A++A!A++A-A-A-A ' -e=0.1 -w=3 -a='(6,A(1,++A!A+)+)' -t='+,-!!!' --colors-pick=1,6 -@=2 -i=0 -A -J='A,3,0;' --zoom=5 --shift-y=-0.1
%%
%%
\begin{center}
%
\fbox{\includegraphics*[width=64.5mm, viewport={0 475 595 842}]{d333333-grid-graph.pdf}}%
\hspace*{0.5mm}% layout
\fbox{\includegraphics*[width=64.5mm, viewport={0 475 595 842}]{d333333-grid-graph-solid.pdf}}%
%
%
\end{center}
\caption{\label{fig:d333333-grid-graph}
Grid-graph of the triangle grid with double edges,
line drawing (left) and
area drawing with colors indicating orientation (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d333333-r61-var2-motif.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%  zrender -d=6 -m='A  A++A!A++A!A++A++A!A++A!A++A++A!A++A!A++A++A!A++A++A!A++A!A++A++A!A+A++A++A!A++A!A++A++A!A++A++A--A-AAA!A++A!A++A++A!A++A!A++A++A!A++A!A++A++A!AAAAA' -e=0.1 -w=7 -a=':A:' -i=1 --margin=0.01 -A=0.25,0.1 -H=L
%%
%% zrender -d=6 -m='A  A++A!A++A!A++A++A!A++A!A++A++A!A++A!A++A++A!A++A++A!A++A!A++A++A!A+A++A++A!A++A!A++A++A!A++A++A--A-AAA!A++A!A++A++A!A++A!A++A++A!A++A!A++A++A!AAAAA' -e=0.1 -w=7 -a='A' -i=1 --margin=0.01 -A=0.25,0.1 -H=L -J='A,3,0'
%%
\begin{center}
%
{\includegraphics*[width=60mm, viewport={0 375 595 710}]{d333333-r61-var2-motif-line.pdf}}%
\hspace*{0mm}% layout
{\includegraphics*[width=60mm, viewport={0 375 595 710}]{d333333-r61-var2-motif-area.pdf}}%
%
\end{center}
\caption{\label{fig:d333333-r61-var2-motif}
%
Motif of a curve of order 61 (left),
the curve starts at the lower left and ends at the upper right.
Area drawing of the same (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d333333-r61-var2-tile-A3.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -m='A  A++A!A++A!A++A++A!A++A!A++A++A!A++A!A++A++A!A++A++A!A++A!A++A++A!A+A++A++A!A++A!A++A++A!A++A++A--A-AAA!A++A!A++A++A!A++A!A++A++A!A++A!A++A++A!AAAAA' -e=0.1 -w=3 -a='(3,A++)' -k=-6 --colors-pick=1,6 -i=2 -@=1 -J='A,3,0;' --margin=0.01
%%
%% zrender -d=6 -m='A  A++A!A++A!A++A++A!A++A!A++A++A!A++A!A++A++A!A++A++A!A++A!A++A++A!A+A++A++A!A++A!A++A++A!A++A++A--A-AAA!A++A!A++A++A!A++A!A++A++A!A++A!A++A++A!AAAAA' -e=0.1 -w=3 -a='(3,A++)' -k=-6 --colors-pick=1,6 -i=2 -@=0 -J='A,3,0;' --margin=0.01
%%
%% zrender -d=6 -m='A  A++A!A++A!A++A++A!A++A!A++A++A!A++A!A++A++A!A++A++A!A++A!A++A++A!A+A++A++A!A++A!A++A++A!A++A++A--A-AAA!A++A!A++A++A!A++A!A++A++A!A++A!A++A++A!AAAAA' -e=0.1 -w=3 -a='+(3,A++)' -k=-6 --colors-pick=1,6 -i=2 -@=0 -J='A,3,0;' --margin=0.01
%%
\begin{center}
%
\begin{subfigure}[b]{19mm}
{\includegraphics*[width=19mm, viewport={0 247 595 842}]{d333333-r61-var2-tile-A3-r0.pdf}}%
\vspace*{25mm}
{\includegraphics*[width=19mm, viewport={0 247 595 842}]{d333333-r61-var2-tile-A3-r1.pdf}}%
\vspace*{15mm}
\end{subfigure}%
%
{\includegraphics*[width=90mm, viewport={0 247 595 832}]{d333333-r61-var2-tile-A3-decomp.pdf}}%
%
\end{center}
\caption{\label{fig:d333333-r61-var2-tile-A3}
The third iterate of the CCW prototile \tileS{A++}{3} (right),
decomposed into 61 copies of its second iterate (left),
appearing in 2 orientations.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% line drawing:
%% zrender -d=6 -m='A A++A!A++A!A++A++A!A++A!A++A++A!A++A!A++A++A!A++A++A!A++A!A++A++A!A+A++A++A!A++A!A++A++A!A++A++A--A-AAA!A++A!A++A++A!A++A!A++A++A!A++A!A++A++A!AAAAA ' -e=0 -w=30 -a='(6,A(1,++A!A+)+)' -@=0 -i=0 -A=0.17,0.1 --margin=0.01

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d333333-r61-var2-tile-digon.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -m='A  A++A!A++A!A++A++A!A++A!A++A++A!A++A!A++A++A!A++A++A!A++A!A++A++A!A+A++A++A!A++A!A++A++A!A++A++A--A-AAA!A++A!A++A++A!A++A!A++A++A!A++A!A++A++A!AAAAA' -e=0.1 -w=3 -a='++(2,A!)' -k=-6 --colors-pick=1,6 -i=2 -@=1 -J='A,3,0;' --margin=0.01
%%
%% zrender -d=6 -m='A  A++A!A++A!A++A++A!A++A!A++A++A!A++A!A++A++A!A++A++A!A++A!A++A++A!A+A++A++A!A++A!A++A++A!A++A++A--A-AAA!A++A!A++A++A!A++A!A++A++A!A++A!A++A++A!AAAAA' -e=0.1 -w=3 -a='++(2,A!)' -k=-6 --colors-pick=1,6 -i=2 -@=0 -J='A,3,0;' --margin=0.01
%%
%% zrender -d=6 -m='A  A++A!A++A!A++A++A!A++A!A++A++A!A++A!A++A++A!A++A++A!A++A!A++A++A!A+A++A++A!A++A!A++A++A!A++A++A--A-AAA!A++A!A++A++A!A++A!A++A++A!A++A!A++A++A!AAAAA' -e=0.1 -w=3 -a='(2,A!)' -k=-6 --colors-pick=1,6 -i=2 -@=0 -J='A,3,0;' --margin=0.01
%%
%% zrender -d=6 -m='A  A++A!A++A!A++A++A!A++A!A++A++A!A++A!A++A++A!A++A++A!A++A!A++A++A!A+A++A++A!A++A!A++A++A!A++A++A--A-AAA!A++A!A++A++A!A++A!A++A++A!A++A!A++A++A!AAAAA' -e=0.1 -w=3 -a='--(2,A!)' -k=-6 --colors-pick=1,6 -i=2 -@=0 -J='A,3,0;' --margin=0.01
%%
\begin{center}
%
{\includegraphics*[width=100mm, viewport={0 372 595 712}]{d333333-r61-var2-tile-digon-decomp.pdf}}%
\hspace*{3mm}% layout
%
\begin{subfigure}[b]{21mm}
{\includegraphics*[width=15mm, viewport={0 247 595 842}]{d333333-r61-var2-tile-digon-2.pdf}}
{\includegraphics*[width=15mm, viewport={0 247 595 842}]{d333333-r61-var2-tile-digon-1.pdf}}
{\includegraphics*[width=15mm, viewport={0 247 595 842}]{d333333-r61-var2-tile-digon-3.pdf}}
\vspace*{5mm}% V
\end{subfigure}
%%
%
\end{center}
\caption{\label{fig:d333333-r61-var2-tile-digon}
The third iterate of the prototile \tileS{A!}{2} (left),
decomposed into smaller copies of itself
appearing in three orientations (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d333333-szilard-quinton-decor.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -a='A' -m='A AF+F+AF-F-F-AF-F+F+F-F+F+F-A F F' -@=1 -k=+6 -i=3 -w=10 --sed='s/A//g;'
%%
%% zrender -d=6 -a='(3,_AF+F+)' -m='A AF+F+AF-F-F-AF-F+F+F-F+F+F-A F F' -i=3 -w=10 --sed='s/A//g;'
%%
\begin{center}
%
{\includegraphics*[width=75mm, viewport={20 410 575 672}]{d333333-szilard-quinton-decor-curve.pdf}}%
\hspace*{3mm}% layout
{\includegraphics*[width=45mm, viewport={0 295 595 785}]{d333333-szilard-quinton-decor-tile.pdf}}%
%
%
\end{center}
\caption{\label{fig:d333333-szilard-quinton-decor}
%
The curve, rendered as suggested by Szilard and Quinton:
self-similarity (left) and the CCW tile (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d333333-szilard-quinton.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -a='A' -m='A A++A!A+A ' -e=0.1 -i=1 -w=20 -A=0.25,0.1 -H=L
%% zrender -d=6 -a='(3,A++)' -m='A A++A!A+A ' -e=0.15 -i=1 -w=20 -A=0.25,0.1 -H=L -k=+1
%% zrender -d=6 -a='(3,A++)' -m='A A++A!A+A ' -e=0.15 -i=6 -w=20 -A=0.25,0.1 -H=L -k=+1 -J='*3,0'
%% zrender -d=6 -a='_____(2,A!~~~)' -m='A A++A!A+A ' -e=0.15 -i=6 -w=20 -A=0.25,0.1 -H=L -J='*3,0' -r=-60
%%
\begin{center}
%
\begin{subfigure}[b]{31mm}
{\includegraphics*[width=30mm, viewport={90 290 505 622}]{d333333-szilard-quinton-A-it1.pdf}}
{\includegraphics*[width=30mm, viewport={90 350 505 682}]{d333333-szilard-quinton-AAA-it1.pdf}}
\end{subfigure}
%\hspace*{1mm}% layout
%
{\includegraphics*[width=50mm, viewport={20 297 595 770}]{d333333-szilard-quinton-AAA-it.pdf}}%
{\includegraphics*[width=38mm, viewport={30 252 565 810}]{d333333-szilard-quinton-AA-it.pdf}}%
%%
%\begin{subfigure}[b]{21mm}
%\fbox{\includegraphics*[width=20mm, viewport={0 247 595 842}]{d333333-szilard-quinton.pdf}}
%\vspace*{12mm}% V
%\end{subfigure}
%
%
\end{center}
\caption{\label{fig:d333333-szilard-quinton}
%
First iterate of a curve of order 4 (top left).
First (bottom left) and sixth (middle) iterate of its CCW tile \tileS{A++}{6}.
Sixth iterate of the CW (digon) tile \tileS{A!}{2} (right).
Coloring by orientation of the curves.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d333333-terdragon-1.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -a='A' -m='A A++A--A ' -e=0.1 -i=1 -w=20 -A=0.22,0.1 -H=L
%% zrender -d=6 -a='(3,A++)' -m='A A++A--A ' -e=0.1 -i=1 -w=20 -A=0.25,0.1 -H=L -k=+1
%%
%% zrender -d=6 -a='(3,A++)' -m='A A++A--A ' -e=0.12 -i=3 -w=15 -A=0.25,0.1 -H=L -k=+1
%% zrender -d=6 -a='(3,A++)' -m='A A++A--A ' -e=0.12 -i=3 -w=15 -A=0.25,0.1 -H=L -k=+1 -J='*3,0'
%%
\begin{center}
%
\begin{subfigure}[b]{21mm}
{\includegraphics*[width=20mm, viewport={120 297 475 702}]{d333333-terdragon-1-A.pdf}}
{\includegraphics*[width=20mm, viewport={120 347 475 702}]{d333333-terdragon-1-AAA.pdf}}
\end{subfigure}
%
{\includegraphics*[width=50mm, viewport={50 310 555 755}]{d333333-terdragon-1-AAA-it1-line.pdf}}%
{\includegraphics*[width=50mm, viewport={50 310 555 755}]{d333333-terdragon-1-AAA-it1-area.pdf}}%
%\hspace*{0mm}% layout
%%
%\begin{subfigure}[b]{21mm}
%\fbox{\includegraphics*[width=20mm, viewport={0 247 595 842}]{d333333-terdragon-1.pdf}}
%\vspace*{12mm}% V
%\end{subfigure}
%
%
\end{center}
\caption{\label{fig:d333333-terdragon-1}
%
First iterate of a curve of order 3 (top left)
and its CCW tile \tileS{A++}{3} (bottom left).
The third iterate of the tile drawn using lines (middle)
and as area drawing (right).
Coloring by orientation of the curves.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d333333-terdragon-2.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -a='(2,:A!)' -m='A A++A--A ' -e=0.12 -i=3 -w=15 -A=0.25,0.1 -H=L
%% zrender -d=6 -a='(2,A!)' -m='A A++A--A ' -e=0.12 -i=3 -w=15 -A=0.25,0.1 -H=L -k=+1 -J='*3,0'
%% zrender -d=6 -a='A++A++A!A--A--A' -m='A A++A--A ' -e=0.12 -i=3 -w=15 -A=0.25,0.1 -H=L -k=+1 -J='*3,0'
%%
\begin{center}
%
{\includegraphics*[width=25mm, viewport={150 247 445 812}]{d333333-terdragon-2-AA-line.pdf}}%
\hspace*{5mm}% layout
{\includegraphics*[width=25mm, viewport={150 247 445 802}]{d333333-terdragon-2-AA-area.pdf}}%
%
{\includegraphics*[width=60mm, viewport={0 293 595 755}]{d333333-terdragon-2-A6.pdf}}
%
%
\end{center}
\caption{\label{fig:d333333-terdragon-2}
%
Third iterate of the CW tile \tileS{A!}{2} with U-turns marked by the two disks (left)
and area drawing of the same (middle).
The area drawing for the axiom \texttt{A++A++A!A--A--A} (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d3636-grid.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -a=F --const-maps --grid=12 -T='F+F,F0G,F--F,F!G, G++G,G0F,G-G,G!F' -L=0.3 --letters-mv=0.45,0.15 -A=0.2,0.15 -H=L -w=8 --zoom=1.3
%%
%% zrender -d=6  -a=F --const-maps -l=,F,G --grid=12 -T='F+F,F0G,F--F,F!G, G++G,G0F,G-G,G!F' -L=0.3 --letters-mv=0.45,0.15 --fancy-print-maps --zoom=1.3 -J='F,6,0;G,3,0' -B=3,0.8
%%
\begin{center}
%
\fbox{\includegraphics*[width=60mm, viewport={100 247 595 600}]{d3636-grid-line.pdf}}%
\hspace*{3mm}% layout
\fbox{\includegraphics*[width=60mm, viewport={100 247 595 600}]{d3636-grid-area.pdf}}%
%
%
\end{center}
\caption{\label{fig:d3636-grid}
%
The trihex grid with double edges,
line drawing (left) and area drawing (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d3636-r13-1-motif.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -a=F -m='F F+F+F+F+F--F+F+F--F--F+F+F--F' -e=0.1 -A -w=10
%% zrender -d=6 -a=F -m='F F+F+F+F+F--F+F+F--F--F+F+F--F' -e=0.1 -A -w=10 -J
%%
%% zrender -d=6 -a='F!G' -m='F F+F+F+F+F--F+F+F--F--F+F+F--F  G G++G-G-G++G++G-G-G++G-G-G-G-G' -e=0.1 -L=0.4 --letters-mv=0.45,0.15 -A=0.2,0.1 -H=L -w=10
%% zrender -d=6 -a='F!G' -m='F F+F+F+F+F--F+F+F--F--F+F+F--F  G G++G-G-G++G++G-G-G++G-G-G-G-G' -e=0.1 -L=0.4 --letters-mv=0.45,0.15 -H=L -l=',F,G' -P='F,6,0;G,3,0;' -J
%%
\begin{center}
%
{\includegraphics*[width=30mm, viewport={50 330 545 780}]{d3636-r13-1-motif-F.pdf}}%
{\includegraphics*[width=32mm, viewport={0 330 545 800}]{d3636-r13-1-motif-F-area.pdf}}%
{\includegraphics*[width=30mm, viewport={50 330 545 780}]{d3636-r13-1-motif-FG.pdf}}%
{\includegraphics*[width=32mm, viewport={0 330 545 800}]{d3636-r13-1-motif-FG-area.pdf}}%
\hspace*{0mm}% layout
%
%
%\begin{subfigure}[b]{20mm}
%\fbox{\includegraphics*[width=20mm, viewport={0 247 595 842}]{d3636-r13-1-motif.pdf}}
%\fbox{\includegraphics*[width=20mm, viewport={0 247 595 842}]{d3636-r13-1-motif.pdf}}
%\end{subfigure}
%
\end{center}
\caption{\label{fig:d3636-r13-1-motif}
%
From left  to right:
curve of order 13 on the trihex grid,
its area drawing,
the digon tile \tileS{F!G}{1} on the grid with double edges,
and its area drawing.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d3636-r13-digon-tiling.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -a=F -m='F F+F+F+F+F--F+F+F--F--F+F+F--F' -e=0.1 -A -w=10 --grid=8 -i=0 -k=6 --colors-pick=1,6 -i=2 -J -r=A --zoom=1.5 --shift-y=-0.055 --shift-x=+0.02
%%
\begin{center}
%
\fbox{\includegraphics*[width=80mm, viewport={0 447 595 842}]{d3636-r13-digon-tiling.pdf}}%
%
%
\end{center}
\caption{\label{fig:d3636-r13-digon-tiling}
%
Tiling the plane by digon tiles \tileS{F!G}{1}.
Coloring by orientation of tiles,
not distinguishing the two curves in any tile.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d3636-r9-koch.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -a='(6,+F)!(3,G++)' -m='F F+F+F!G++G++G!F--F+F+F  G G++G!F+F!G++G++G-G ' -A=0.25,0.1 -H=L -e=0.1 -@=0 -i=1 -k=-1 -w=5 -L=0.4 --letters-mv=0.45,0.15 -r=90
%%
%% zrender -d=6 -a='(6,+F)!(3,G++)' -m='F F+F+F!G++G++G!F--F+F+F  G G++G!F+F!G++G++G-G ' -A -@=0 -i=4 -k=-1 -J='F,6,0;G,3,0' -r=90
%%
\begin{center}
%
{\includegraphics*[width=55mm, viewport={0 247 595 742}]{d3636-r9-koch-it1.pdf}}%
\hspace*{3mm}% layout
{\includegraphics*[width=70mm, viewport={20 325 575 745}]{d3636-r9-koch-it.pdf}}%
%
%
\end{center}
\caption{\label{fig:d3636-r9-koch}
%
First (left) and fourth (right) iterate
of the CCW tile \tileS{F+}{6} and \tileS{G++}{3}
drawn next to each other.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d3636-rx-6fold-it.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -a='_(6,+F)_!(3,G++)' -m='F F+F+F+F--F--F+F+F+F--F  G G++G-G-G-G++G++G-G-G-G ' --filled-paths -i=2
%%
%% zrender -d=6 -a='_(6,+F)_!(3,G++)' -m='F F+F+F+F--F--F+F+F+F--F  G G++G-G-G-G++G++G-G-G-G ' --filled-paths -i=3 -r=-45
%%
\begin{center}
%
%\fbox{\includegraphics*[width=50mm, viewport={30 247 565 742}]{d3636-rx-6fold-it2.pdf}}%
{\includegraphics*[width=100mm, viewport={0 340 595 731}]{d3636-rx-6fold-it3.pdf}}%
\hspace*{0mm}% layout
%
%
\end{center}
\caption{\label{fig:d3636-rx-6fold-it}
Third iterates of the CCW prototiles:
tile \tileS{F+}{6} colored blue,
tile \tileS{G++}{3} colored red.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d3636-rx-6fold-it1.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -a='(6,+F)!(3,G++)' -m='F F+F+F+F--F--F+F+F+F--F  G G++G-G-G-G++G++G-G-G-G ' -A=0.25,0.1 -H=L -e=0.1 -@=0 -i=1 -w=7 -L=0.4 --letters-mv=0.45,0.15
%%
%% zrender -d=6 -a='_(6,+F)_!(3,G++)' -m='F F+F+F+F--F--F+F+F+F--F  G G++G-G-G-G++G++G-G-G-G ' --filled-paths
%%
\begin{center}
%
{\includegraphics*[width=40mm, viewport={0 310 595 762}]{d3636-rx-6fold-it1.pdf}}%
\hspace*{10mm}% layout
{\includegraphics*[width=40mm, viewport={0 310 595 762}]{d3636-rx-6fold-it1-area.pdf}}%
%
\end{center}
\caption{\label{fig:d3636-rx-6fold-it1}
Borders of the CCW tiles, drawn next to each other.
Tile \tileS{F+}{6} is the bigger one, tile \tileS{G++}{3} the smaller one.
Line drawing (left) and area drawing (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d4444-grid-graph.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=4 -m='A A+A0A!A+A' -a='(4,A+)' -i=3 -w=10 -e=0 --zoom=2.4 -A=0.2,0.15 -H=L
%% zrender -d=4 -m='A A+A0A!A+A' -a='(4,A+)' -i=0 -@=3 -w=10 -e=0 -k=-4 --zoom=2.4 -J='A,4,0'
%%
\begin{center}
%
\fbox{\includegraphics*[width=60mm, viewport={0 495 595 822}]{d4444-grid-graph.pdf}}%
\hspace*{3mm}% layout
\fbox{\includegraphics*[width=60mm, viewport={0 495 595 822}]{d4444-grid-graph-solid.pdf}}%
%
%
\end{center}
\caption{\label{fig:d4444-grid-graph}
Grid-graph of the square grid with double edges,
line drawing (left) and area drawing (right).
Coloring by the orientations of the edges.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%% zrender -d=6 -m='A A++A!A++A++A!A++A++A!A++A-A-A-A ' -e=0.1 -w=3 -a='(6,A(1,++A!A+)+)' -t='+,-!!!' --colors-pick=1,6 -@=2 -i=0 -A -J='A,3,0;' --zoom=5 --shift-y=-0.1
%%
%% zrender -d=6 -m='A A++A!A++A++A!A++A++A!A++A-A-A-A ' -e=0 -a='(6,A(1,++A!A+)+)' -i=2 -A --zoom=5 --shift-y=-0.1 -w=10 -A=0.1 --arrow-offset=0.15

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d4444-r17-tile-it1.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-double-edge.txt , d4444-r17
%%
%% zrender -d=4 -a='(4,A+)' -m='A A0A+A-A0A' -w=15 -e=0.1 -i=1 -@=0 -k=-1 -A=0.25,0.1 -H=L
%%
%% zrender -d=4 -a='(4,A+)' -m='A A+A!A+A+A0A0A!A0A+A+A+A!A+A!A0A+A' -w=15 -e=0.1 -i=1 -@=0 -k=-1 -A=0.2,0.1 -H=L
%%
%% zrender -d=4 -a='(4,A+)' -m='A A+A!A+A+A0A0A!A0A+A+A+A!A+A!A0A+A' -w=15 -e=0.1 -i=1 -@=0 -k=-1 -A -J='A,4,0;'
%%
\begin{center}
%
{\includegraphics*[width=33mm, viewport={0 260 595 812}]{d4444-r17-tile-it1-outline.pdf}}%
\hspace*{8mm}% layout
{\includegraphics*[width=33mm, viewport={0 260 595 812}]{d4444-r17-tile-it1.pdf}}%
\hspace*{8mm}% layout
{\includegraphics*[width=33mm, viewport={0 260 595 812}]{d4444-r17-tile-it1-solid.pdf}}%
%
\end{center}
\caption{\label{fig:d4444-r17-tile-it1}
Border of the CCW tile \tileS{A+}{4} (left),
tile filled with an order 17 curve,
line drawing (middle) and
area drawing (right).
First iterates.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d4444-r17-tiles.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-double-edge.txt , d4444-r17
%%
%% zrender -d=4 -a='(4,A+)' -m='A A+A!A+A+A0A0A!A0A+A+A+A!A+A!A0A+A' -w=15 -e=0.1 -i=4 -@=0 -k=-1 -A -J='A,4,0;'
%%
%% zrender -d=4 -a='(2,A!)' -m='A A+A!A+A+A0A0A!A0A+A+A+A!A+A!A0A+A' -w=15 -e=0.1 -i=4 -@=0 --colors-pick=1,2 -k=-1 -A -J='A,4,0;'
%%
%% zrender -d=4 -a='(2,A!)' -m='A A+A!A+A+A0A0A!A0A+A+A+A!A+A!A0A+A' -w=15 -e=0.1 -i=3 -@=1 --colors-pick=1,2 -t='!!+,-' -J='A,4,0;'
%%
\begin{center}
%
{\includegraphics*[width=50.5mm, viewport={10 247 585 812}]{d4444-r17-tiles-plus.pdf}}%
\hspace*{1mm}% layout
{\includegraphics*[width=38mm, viewport={75 247 520 822}]{d4444-r17-tiles-digon.pdf}}%
\hspace*{1mm}% layout
{\includegraphics*[width=38mm, viewport={75 247 520 822}]{d4444-r17-tiles-digon-self-sim.pdf}}%
%
\end{center}
\caption{\label{fig:d4444-r17-tiles}
Fourth iterates of the tiles \tileS{A+}{4} (left) and \tileS{A!}{2} (middle).
Self-similarity of the digon tile \tileS{A!}{2} (right),
small copies appear in two orientations.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d4444-r4-pc-curve.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=8 -m='A A+A!A+A' -a='(1,A+)' -i=3 -w=10 --sed='s/+/+F+/g; s/A/+F-F-F+/g; s/!/--F--/g;'
%%
\begin{center}
%
{\includegraphics*[width=75mm, viewport={30 400 565 665}]{d4444-r4-pc-curve.pdf}}%
\hspace*{0mm}% layout
%
%
\end{center}
\caption{\label{fig:d4444-r4-pc-curve}
%
The curve rendered to traverse
the points of the $(4.8.8)$-grid.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d4444-r4-tile-it1.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-double-edge.txt , d4444-r5
%%
%% zrender -d=4 -m='A A0A' -a='(4,A+)' -k=-1 -i=1  -w=15 -e=0.1 -A=0.2,0.1 -H=L
%% zrender -d=4 -m='A A+A!A+A' -a='(4,A+)' -k=-1 -i=1  -w=15 -e=0.1 -A=0.2,0.1 -H=L
%% zrender -d=4 -m='A A+A!A+A' -a='(4,A+)' -k=-1 -i=2  -w=15 -e=0.1 -A=0.2,0.1 -H=L
%%% zrender -d=4 -m='A A+A!A+A' -a='(4,A+)' -k=-1 -i=2  -w=15 -e=0.1 -A=0.2,0.1 -H=L -J='*,4,0'
%%
\begin{center}
%
{\includegraphics*[width=40mm, viewport={0 320 595 752}]{d4444-r4-tile-it1-outline.pdf}}%
%{\includegraphics*[width=32mm, viewport={0 247 595 842}]{d4444-r4-tile-it1-outline-solid.pdf}}%
\hspace*{0mm}% layout
{\includegraphics*[width=40mm, viewport={0 320 595 752}]{d4444-r4-tile-it1.pdf}}%
{\includegraphics*[width=40mm, viewport={0 310 595 757}]{d4444-r4-tile-it2.pdf}}%
%{\includegraphics*[width=32mm, viewport={0 247 595 842}]{d4444-r4-tile-it1-solid.pdf}}%
%
\end{center}
\caption{\label{fig:d4444-r4-tile-it1}
Border of the CCW tile \tileS{A+}{4} (left)
and the tile filled with a curve of order 4 (middle).
Second iterate of the tile (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d4444-r5-tile-it1.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-double-edge.txt , d4444-r5
%%
%% zrender -d=4 -m='A A+A-A' -a='(4,A+)' -k=-1 -i=1  -w=15 -e=0.1 -A=0.2,0.1 -H=L
%%% zrender -d=4 -m='A A+A-A' -a='(4,A+)' -k=-1 -i=1  -w=15 -e=0.1 -A -J='A,4,0'
%%
%% zrender -d=4 -m='A A+A0A!A+A' -a='(4,A+)' -k=-1 -i=1  -w=15 -e=0.1 -A=0.2,0.1 -H=L
%%% zrender -d=4 -m='A A+A0A!A+A' -a='(4,A+)' -k=-1 -i=1  -w=7 -e=0.1 -J='A,4,0'
%%
\begin{center}
%
{\includegraphics*[width=40mm, viewport={0 320 595 752}]{d4444-r5-tile-it1-outline.pdf}}%
%{\includegraphics*[width=32mm, viewport={0 247 595 842}]{d4444-r5-tile-it1-outline-solid.pdf}}%
\hspace*{8mm}% layout
{\includegraphics*[width=40mm, viewport={0 320 595 752}]{d4444-r5-tile-it1.pdf}}%
%{\includegraphics*[width=32mm, viewport={0 247 595 842}]{d4444-r5-tile-it1-solid.pdf}}%
%
\end{center}
\caption{\label{fig:d4444-r5-tile-it1}
Border of the CCW tile \tileS{A+}{4} (left)
and the tile filled with a curve of order 5 (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d4444-r5-tiles.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%% file 00lsys-double-edge.txt , d4444-r5
%%
%% zrender -d=4 -m='A A+A0A!A+A' -a='(4,A+)' -k=-1 -i=6 -w=7 -e=0.1 -J='A,4,0'
%%
%% zrender -d=4 -m='A A+A0A!A+A' -a='(2,A!)' --colors-pick=1,2 -k=-1 -i=6 -w=7 -e=0.1 -J='A,4,0'
%%
\begin{center}
%
{\includegraphics*[width=54.5mm, viewport={0 265 595 812}]{d4444-r5-tiles-plus.pdf}}%
\hspace*{10mm}% layout
{\includegraphics*[width=54.5mm, viewport={0 265 595 812}]{d4444-r5-tiles-digon.pdf}}%
%
\end{center}
\caption{\label{fig:d4444-r5-tiles}
Sixth iterates of the tiles \tileS{A+}{4} (left)
and \tileS{A!}{2} (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d4444-r85-var1-motif.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=4 -w=12 -e=0 -m='A AAAAAA+A!A0A+A!A+A+A!A+A+A!A+A+A!A+A+A!A+A!A+0A+A!A+A+A!A+A+A!A+A+A!A+A!A+0A+A!A+A+A!A+A+A!A+A!A+0A+A!A+A+A!A+A!A+0A+A!A+A!A+0A+A+AA+AAA+AAAA+AAAAA+AAAAAA' -a=':A:' -i=1 --margin=0.01 -A=0.25,0.1 -H=L -e=0.1
%%
%% zrender -d=4 -w=12 -e=0 -m='A AAAAAA+A!A0A+A!A+A+A!A+A+A!A+A+A!A+A+A!A+A!A+0A+A!A+A+A!A+A+A!A+A+A!A+A!A+0A+A!A+A+A!A+A+A!A+A!A+0A+A!A+A+A!A+A!A+0A+A!A+A!A+0A+A+AA+AAA+AAAA+AAAAA+AAAAAA' -a='A' -i=1 --margin=0.01 -A=0.25,0.1 -H=L -e=0.1 -J='*,4,0;'
%%
%%
\begin{center}
%
{\includegraphics*[width=35mm, viewport={0 247 595 805}]{d4444-r85-var1-motif.pdf}}%
\hspace*{8mm}% layout
{\includegraphics*[width=35mm, viewport={0 247 595 805}]{d4444-r85-var1-motif-area.pdf}}%
%
\end{center}
\caption{\label{fig:d4444-r85-var1-motif}
%
Motif of the curve.
Line drawing (left) and area drawing (right).
The curve starts at the upper left and ends at the lower right.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d4444-r85-var1-tile-plus.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=4 -w=2 -e=0 -m='A AAAAAA+A!A0A+A!A+A+A!A+A+A!A+A+A!A+A+A!A+A!A+0A+A!A+A+A!A+A+A!A+A+A!A+A!A+0A+A!A+A+A!A+A+A!A+A!A+0A+A!A+A+A!A+A!A+0A+A!A+A!A+0A+A+AA+AAA+AAAA+AAAAA+AAAAAA' -a='(4,A+)' -k=-4 -J='A,4,0;' -i=1 -@=1 --margin=0.01 -r=A
%%
%% zrender -d=4 -w=2 -e=0 -m='A AAAAAA+A!A0A+A!A+A+A!A+A+A!A+A+A!A+A+A!A+A!A+0A+A!A+A+A!A+A+A!A+A+A!A+A!A+0A+A!A+A+A!A+A+A!A+A!A+0A+A!A+A+A!A+A!A+0A+A!A+A!A+0A+A+AA+AAA+AAAA+AAAAA+AAAAAA' -a='(4,A+)' -k=-4 -J='A,4,0;' -i=1 -@=0 --margin=0.01 -r=-90
%%
%%
\begin{center}
%
{\includegraphics*[width=95mm, viewport={0 247 595 837}]{d4444-r85-var1-tile-plus-decomp.pdf}}%
\hspace*{3mm}% layout
%
\begin{subfigure}[b]{30.5mm}
{\includegraphics*[width=30mm, viewport={0 247 595 842}]{d4444-r85-var1-tile-plus.pdf}}
\vspace*{4mm}% V
\end{subfigure}
%
%\begin{subfigure}[b]{20mm}
%\fbox{\includegraphics*[width=20mm, viewport={0 247 595 842}]{d4444-r85-var1-tile-plus.pdf}}
%\fbox{\includegraphics*[width=20mm, viewport={0 247 595 842}]{d4444-r85-var1-tile-plus.pdf}}
%\end{subfigure}
%
\end{center}
\caption{\label{fig:d4444-r85-var1-tile-plus}
The second iterate of the CCW prototile \tileS{A+}{4} (left),
decomposed into 85 small copies of its first iterate (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d488-x-const-b-r5-var1-tile-minus.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%% was:
%% zrender -d=8 -a='(4,A+B+)' -m='A Abbbb!BABBA!ABA  B B  b b' -T='A!A,B!b,b!B,A+B,A-b,B+A,B--B,b++b,b-A' -w=20 -l -e=0.1 -k=+8 -i=0 -@=1 -J='A,8,0;B,8,0;b,4,0'
%%% now is
%% zrender -d=8 -a='(2,A!)' -m='A Abbbb!BABBA!ABA  B B  b b' -T='A!A,B!b,b!B,A+B,A-b,B+A,B--B,b++b,b-A' -w=20 -l -e=0.1 -k=+8 -i=0 -@=1 -J='A,8,0;B,8,0;b,4,0'
%% zrender -d=8 -a='(2,A!)' -m='A Abbbb!BABBA!ABA  B B  b b' -T='A!A,B!b,b!B,A+B,A-b,B+A,B--B,b++b,b-A' -w=20 -l -e=0.1 -k=+8 -i=1 -@=1 -J='A,8,0;B,8,0;b,4,0'
%% zrender -d=8 -a='(2,A!)' -m='A Abbbb!BABBA!ABA  B B  b b' -T='A!A,B!b,b!B,A+B,A-b,B+A,B--B,b++b,b-A' -w=20 -l -e=0.1 -k=+8 -i=3 -@=1 -J='A,8,0;B,8,0;b,4,0' -r=-52
%%
\begin{center}
%
{\includegraphics*[width=25mm, viewport={150 247 450 842}]{d488-x-const-b-r5-var1-tile-minus-it1.pdf}}%
{\includegraphics*[width=40mm, viewport={80 247 515 842}]{d488-x-const-b-r5-var1-tile-minus-it2.pdf}}%
%{\includegraphics*[width=43mm, viewport={0 247 595 842}]{d488-x-const-b-r5-var1-tile-minus-it3.pdf}}%
{\includegraphics*[width=55mm, viewport={50 257 595 815}]{d488-x-const-b-r5-var1-tile-minus-it4.pdf}}%
\hspace*{0mm}% layout
%
\end{center}
\caption{\label{fig:d488-x-const-b-r5-var1-tile-minus}
The CW tile \tileS{A!}{2},
first (left), second (middle), and fourth (right) iterate.
Coloring by the orientations of the edges in the first iterate.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d488-x-const-b-r5-var1.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=8 -a='A' -m='A Abbbb!BABBA!ABA  B B  b b' -T='A!A,B!b,b!B,A+B,A-b,B+A,B--B,b++b,b-A' -w=20 -e=0.1 -L=0.5 -i=0 -@=1 --zoom=0.95 -A=0.3,0.1 -H=L --letters-mv=0.45,0.15
%% zrender -d=8 -a='A' -m='A Abbbb!BABBA!ABA  B B  b b' -T='A!A,B!b,b!B,A+B,A-b,B+A,B--B,b++b,b-A' -w=20 -l -e=0.1 -A -L=0.5 -k=+8 -i=0 -@=1 --zoom=0.95  -J='A,8,0;B,8,0;b,4,0' --letters-mv=0.45,0.15
%%
%% zrender -d=8 -a='A' -m='A Abbbb!BABBA!ABA  B B  b b' -T='A!A,B!b,b!B,A+B,A-b,B+A,B--B,b++b,b-A' -w=20 -l -e=0.1 -k=+8 -i=1 -@=1 --zoom=0.95 -J='A,8,0;B,8,0;b,4,0'
%% zrender -d=8 -a='A' -m='A Abbbb!BABBA!ABA  B B  b b' -T='A!A,B!b,b!B,A+B,A-b,B+A,B--B,b++b,b-A' -w=20 -l -e=0.1 -k=+8 -i=2 -@=1 --zoom=0.95 -J='A,8,0;B,8,0;b,4,0'
%%
\begin{center}
%
%\begin{subfigure}[b]{25mm}
%\end{subfigure}
{\includegraphics*[width=32mm, viewport={100 267 495 802}]{d488-x-const-b-r5-var1-it1.pdf}}%
{\includegraphics*[width=32mm, viewport={100 267 495 802}]{d488-x-const-b-r5-var1-it1-solid.pdf}}%
%\hspace*{3mm}% layout
%
{\includegraphics*[width=32mm, viewport={90 267 495 802}]{d488-x-const-b-r5-var1-it2-solid.pdf}}%
{\includegraphics*[width=32mm, viewport={90 267 495 802}]{d488-x-const-b-r5-var1-it3-solid.pdf}}
%
\end{center}
\caption{\label{fig:d488-x-const-b-r5-var1}
From left to right:
motif as line and as area drawing,
second and third iterates as area drawing.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d488-x-grid-graph-2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=8 -a='A!(4,A+B+)' -m='A Abbbb!BABBA!ABA  B B  b b' -T='A!A,B!b,b!B,A+B,A-b,B+A,B--B,b++b,b-A' -w=15 -k=+8 -A=0.2,0.1 -e=0 -i=0 -@=3 --zoom=5.2 --shift-x=-0.05 -J='A,8,0;B,8,0;b,4,0'
%%
\begin{center}
%
\fbox{\includegraphics*[width=60mm, viewport={0 367 595 842}]{d488-x-grid-graph-dir-solid.pdf}}%
%
\end{center}
\caption{\label{fig:d488-x-grid-graph-2}
Area drawing of the grid colored by orientation of edges.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d488-x-grid-graph.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=8 -a='A!(4,A+B+)' -m='A Abbbb!BABBA!ABA  B B  b b' -T='A!A,B!b,b!B,A+B,A-b,B+A,B--B,b++b,b-A' -w=15 -l=',A,Bb' -L=0.5 -e=0 -i=0 -@=3 --zoom=5.2 --shift-x=-0.05 -A=0.25,0.15 -H=L --letters-mv=0.45,0.15
%%
%% zrender -d=8 -a='A!(4,A+B+)' -m='A Abbbb!BABBA!ABA  B B  b b' -T='A!A,B!b,b!B,A+B,A-b,B+A,B--B,b++b,b-A' -w=15 -l=',A,B,b' -A=0.2,0.1 -L=0.5 -e=0 -i=0 -@=3 --zoom=5.2 --shift-x=-0.05 -J='A,8,0;B,8,0;b,4,0' --letters-mv=0.45,0.15 -B=5
%%
%%% zrender -d=8 -a='A!(4,A+B+)' -m='A Abbbb!BABBA!ABA  B B  b b' -T='A!A,B!b,b!B,A+B,A-b,B+A,B--B,b++b,b-A' -w=15 -k=+8 -A=0.2,0.1 -e=0 -i=0 -@=3 --zoom=5.2 --shift-x=-0.05 -J='A,8,0;B,8,0;b,4,0'
%%
\begin{center}
%
\fbox{\includegraphics*[width=60mm, viewport={0 367 595 842}]{d488-x-grid-graph.pdf}}%
\hspace*{5mm}% layout
\fbox{\includegraphics*[width=60mm, viewport={0 367 595 842}]{d488-x-grid-graph-solid.pdf}}%
% \hspace*{0.5mm}% layout
% \fbox{\includegraphics*[width=42.5mm, viewport={0 367 595 842}]{d488-x-grid-graph-dir-solid.pdf}}%
%
\end{center}
\caption{\label{fig:d488-x-grid-graph}
%Grid where all edges are double edges.
The $(4.8.8)$-grid with double edges,
line drawing (left, blue for \texttt{A}, otherwise red)
and area drawing
(right, blue for \texttt{A}, red for \texttt{B}, green for \texttt{b}).\IMAGENAME%
%, and area drawing colored by orientation of edges (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d488-x-r13-2-var0-curve-tiling.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%% zrender -d=8 -a='B' -T='A!A,B!b,b!B,A+B,A-b,B+A,B--B,b++b,b-A' -w=15 -k=+8 --colors-pick=1,8 -m='A ABbbbbABAABABbABA  b bbbBAb  B BABABbbbABbABBAB' -J='A,8,0;B,8,0;b,4,0' -i=2 --grid=12,12 -r=A --zoom=1.4 --shift-y=-0.02
%%
\begin{center}
%
\fbox{\includegraphics*[width=100mm, viewport={0 547 595 842}]{d488-x-r13-2-var0-curve-tiling.pdf}}%
\hspace*{0mm}% layout
%
\end{center}
\caption{\label{fig:d488-x-r13-2-var0-curve-tiling}
%
Tiling the plane by the curves, coloring by orientation.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d488-x-r13-2-var0-motifs.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=8 -a=':A:' -T='A!A,B!b,b!B,A+B,A-b,B+A,B--B,b++b,b-A' -w=15 -l=',A,b,B' --fancy-print-maps -e=0.1 -L=0.4 -A=0.3,0.1 -H=L --letters-mv=0.45,0.2 -m='A ABbbbbABAABABbABA b bbbBAb B BABABbbbABbABBAB'
%% zrender -d=8 -a=':b:' -T='A!A,B!b,b!B,A+B,A-b,B+A,B--B,b++b,b-A' -w=15 -l=',A,b,B' --fancy-print-maps -e=0.1 -L=0.4 -A=0.3,0.1 -H=L --letters-mv=0.45,0.2 -m='A ABbbbbABAABABbABA b bbbBAb B BABABbbbABbABBAB'
%% zrender -d=8 -a=':B:' -T='A!A,B!b,b!B,A+B,A-b,B+A,B--B,b++b,b-A' -w=15 -l=',A,b,B' --fancy-print-maps -e=0.1 -L=0.4 -A=0.3,0.1 -H=L --letters-mv=0.45,0.2 -m='A ABbbbbABAABABbABA b bbbBAb B BABABbbbABbABBAB'
%%
\begin{center}
%
{\includegraphics*[width=40mm, viewport={50 300 505 790}]{d488-x-r13-2-var0-motifs-A.pdf}}%
{\includegraphics*[width=29mm, viewport={25 247 569 802}]{d488-x-r13-2-var0-motifs-b.pdf}}%
{\includegraphics*[width=43mm, viewport={50 277 585 802}]{d488-x-r13-2-var0-motifs-B.pdf}}%
\hspace*{0mm}% layout
%
%
\end{center}
\caption{\label{fig:d488-x-r13-2-var0-motifs}
%
Motifs for curves
\texttt{A} (left),
\texttt{b} (middle), and
\texttt{B} (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d666-ABC-grid.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -T='A+B,A!A,A-C, B+C,B!B,B-A, C+A,C!C,C-B' --const-maps -e=0.1 -w=15 -a='A' -l=',A,B,C' -A --grid=10,10 -i=0 --zoom=1.5 --shift-y=-0.03 -A=0.3,0.1 -H=L -L=0.4 --letters-mv=0.45,0.15
%%
%% zrender -d=6 -T='A+B,A!A,A-C, B+C,B!B,B-A, C+A,C!C,C-B' --const-maps -e=0.1 -w=15 -a='A' -l=',A,B,C' -A --grid=10,10 -i=0 --zoom=1.5 --shift-y=-0.03 -J='*,6,0' -B=3,0.7
%%
\begin{center}
%
\fbox{\includegraphics*[width=60mm, viewport={0 450 595 842}]{d666-ABC-grid.pdf}}%
\hspace*{3mm}% layout
\fbox{\includegraphics*[width=60mm, viewport={0 450 595 842}]{d666-ABC-grid-area.pdf}}%
%
%
\end{center}
\caption{\label{fig:d666-ABC-grid}
%
%\jjTodo{ use -B also in other area drawing of grids }
A coloring of the hexagon grid with three colors.
Line drawing (left) and area drawing (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d666-ABC-r13-var01-motifs.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -T='A+B,A!A,A-C, B+C,B!B,B-A, C+A,C!C,C-B' -m='A A+B+C+A+B!B+C+A-C!C+A-C+A+B-A  B B+C+A+B+C!C+A+B!B-A+B+C-B  C C+A+B+C+A!A+B!B+C+A-C' -e=0.12 -w=15 -a=':A:' -l=',A,B,C' -i=1 -A=0.3,0.1 -H=L -L=0.4 --letters-mv=0.45,0.15
%% zrender -d=6 -T='A+B,A!A,A-C, B+C,B!B,B-A, C+A,C!C,C-B' -m='A A+B+C+A+B!B+C+A-C!C+A-C+A+B-A  B B+C+A+B+C!C+A+B!B-A+B+C-B  C C+A+B+C+A!A+B!B+C+A-C' -e=0.12 -w=15 -a=':B:' -l=',A,B,C' -i=1 -A=0.3,0.1 -H=L -L=0.4 --letters-mv=0.45,0.15
%% zrender -d=6 -T='A+B,A!A,A-C, B+C,B!B,B-A, C+A,C!C,C-B' -m='A A+B+C+A+B!B+C+A-C!C+A-C+A+B-A  B B+C+A+B+C!C+A+B!B-A+B+C-B  C C+A+B+C+A!A+B!B+C+A-C' -e=0.12 -w=15 -a=':C:' -l=',A,B,C' -i=1 -A=0.3,0.1 -H=L -L=0.4 --letters-mv=0.45,0.15
%%
%%
\begin{center}
%
{\includegraphics*[width=43mm, viewport={50 307 595 710}]{d666-ABC-r13-var01-motifs-A.pdf}}%
{\includegraphics*[width=43mm, viewport={50 337 595 740}]{d666-ABC-r13-var01-motifs-B.pdf}}%
{\includegraphics*[width=35mm, viewport={50 290 595 790}]{d666-ABC-r13-var01-motifs-C.pdf}}%
\hspace*{0mm}% layout
%
\end{center}
\caption{\label{fig:d666-ABC-r13-var01-motifs}
%
First iterates of the curves
\texttt{A} (left),
\texttt{B} (middle), and
\texttt{C} (right).
Each curve starts at the bottom and ends at the top right
as indicted.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d666-ABC-r13-var01-tiles-minus.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%% zrender -d=6 -T='A+B,A!A,A-C, B+C,B!B,B-A, C+A,C!C,C-B' -m='A A+B+C+A+B!B+C+A-C!C+A-C+A+B-A  B B+C+A+B+C!C+A+B!B-A+B+C-B  C C+A+B+C+A!A+B!B+C+A-C' -e=0.1 -w=5 -a='(2,A!)' -l=',A,B,C' -i=1 -A -i=0 -J='*,6,0' -@=1 -i=3
%% zrender -d=6 -T='A+B,A!A,A-C, B+C,B!B,B-A, C+A,C!C,C-B' -m='A A+B+C+A+B!B+C+A-C!C+A-C+A+B-A  B B+C+A+B+C!C+A+B!B-A+B+C-B  C C+A+B+C+A!A+B!B+C+A-C' -e=0.1 -w=5 -a='+(2,B!)' -l=',A,B,C' -i=1 -A -i=0 -J='*,6,0' -@=1 -i=3
%% zrender -d=6 -T='A+B,A!A,A-C, B+C,B!B,B-A, C+A,C!C,C-B' -m='A A+B+C+A+B!B+C+A-C!C+A-C+A+B-A  B B+C+A+B+C!C+A+B!B-A+B+C-B  C C+A+B+C+A!A+B!B+C+A-C' -e=0.1 -w=5 -a='++(2,C!)' -l=',A,B,C' -i=1 -A -i=0 -J='*,6,0' -@=1 -i=3
%%
%%
\begin{center}
%
{\includegraphics*[width=41mm, viewport={100 247 500 822}]{d666-ABC-r13-var01-tiles-minus-AA.pdf}}%
{\includegraphics*[width=45mm, viewport={0 247 595 842}]{d666-ABC-r13-var01-tiles-minus-BB.pdf}}%
{\includegraphics*[width=37mm, viewport={0 247 595 842}]{d666-ABC-r13-var01-tiles-minus-CC.pdf}}%
\hspace*{0mm}% layout
%
\end{center}
\caption{\label{fig:d666-ABC-r13-var01-tiles-minus}
%
Mutual self-similarity of the CW tiles
\tileS{A!}{2} (left, small copies blue),
\tileS{B!}{2} (middle, small copies red), and
\tileS{C!}{2} (right, small copies green).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d666-grid-graph.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%% zrender -d=6 -m='A A+A+A+A+A!A+A+A!A-A+A+A-A ' -e=0 -w=10 -a='(6,A+)' -i=0 -@=2 -A=0.3,0.15 --zoom=3 --no-text -H=L
%%
%% zrender -d=6 -m='A A+A+A+A+A!A+A+A!A-A+A+A-A ' -e=0 -w=5 -a='(6,A+)' -k=+6 -i=0 -@=2 -A=0.2,0.1 -J='A,6,0;' --zoom=3 --no-text
%%
\begin{center}
%
\fbox{\includegraphics*[width=64mm, viewport={0 447 595 842}]{d666-grid-graph.pdf}}%
\hspace*{1mm}% layout
\fbox{\includegraphics*[width=64mm, viewport={0 447 595 842}]{d666-grid-graph-solid.pdf}}%
%
\end{center}
\caption{\label{fig:d666-grid-graph}
The hexagon grid with double edges (left).
In the area drawing (right) each edge corresponds to the
triangular area left of it, coloring by orientation.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d666-r109-var1-motif.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -m='A A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A+A!A+A+A+A!A+A+A+A+A+A!A+A+A+A!A+A+A+A+A+A-A+A!A+A-A-A+A-A+A-A+A!A+A-A+A-A+A-A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A-A+A-A+A-A+A-A+A-A+A-A ' -e=0 -k=+6 -w=7 -a=':A:' -i=0 -@=1 --margin=0.01 -A=0.3,0.1 -H=L -e=0.1 -k=0
%%
%% zrender -d=6 -m='A A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A+A!A+A+A+A!A+A+A+A+A+A!A+A+A+A!A+A+A+A+A+A-A+A!A+A-A-A+A-A+A-A+A!A+A-A+A-A+A-A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A-A+A-A+A-A+A-A+A-A+A-A ' -e=0 -k=+6 -w=7 -a='A' -i=0 -@=1 --margin=0.01 -A=0.3,0.1 -H=L -e=0.1 -k=0 -J='A,6,0;'
%%
\begin{center}
%
{\includegraphics*[width=60mm, viewport={0 337 595 747}]{d666-r109-var1-motif.pdf}}%
\hspace*{3mm}%
{\includegraphics*[width=60mm, viewport={0 337 595 747}]{d666-r109-var1-motif-area.pdf}}%
%
\end{center}
\caption{\label{fig:d666-r109-var1-motif}
%
First iterate of a curve of order 109.
It starts at the bottom and ends at the top.
Line drawing (left) and area drawing (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d666-r109-var1-tile-digon.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -m='A A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A+A!A+A+A+A!A+A+A+A+A+A!A+A+A+A!A+A+A+A+A+A-A+A!A+A-A-A+A-A+A-A+A!A+A-A+A-A+A-A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A-A+A-A+A-A+A-A+A-A+A-A ' -e=0 -k=+6 -w=3 -a='++(2,A!)' -i=1 -@=1 -A -J='A,6,0;' --margin=0.01
%%
%% zrender -d=6 -m='A A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A+A!A+A+A+A!A+A+A+A+A+A!A+A+A+A!A+A+A+A+A+A-A+A!A+A-A-A+A-A+A-A+A!A+A-A+A-A+A-A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A-A+A-A+A-A+A-A+A-A+A-A ' -e=0 -k=+6 -w=3 -a='++(2,A!)' -i=1 -@=0 -A -J='A,6,0;'
%% zrender -d=6 -m='A A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A+A!A+A+A+A!A+A+A+A+A+A!A+A+A+A!A+A+A+A+A+A-A+A!A+A-A-A+A-A+A-A+A!A+A-A+A-A+A-A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A-A+A-A+A-A+A-A+A-A+A-A ' -e=0 -k=+6 -w=3 -a='++++(2,A!)' -i=1 -@=0 -A -J='A,6,0;' --margin=0.1
%% zrender -d=6 -m='A A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A+A!A+A+A+A!A+A+A+A+A+A!A+A+A+A!A+A+A+A+A+A-A+A!A+A-A-A+A-A+A-A+A!A+A-A+A-A+A-A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A-A+A-A+A-A+A-A+A-A+A-A ' -e=0 -k=+6 -w=3 -a='++++++(2,A!)' -i=1 -@=0 -A -J='A,6,0;' --margin=0.03 # scale!
%%
%%
\begin{center}
%
{\includegraphics*[width=109mm, viewport={0 350 595 733}]{d666-r109-var1-tile-digon-decomp.pdf}}%
%\hspace*{0.5mm}%
%
\begin{subfigure}[b]{21mm}
{\includegraphics*[width=20mm, viewport={0 247 595 842}]{d666-r109-var1-tile-digon-it1-r0.pdf}}
{\includegraphics*[width=20mm, viewport={0 247 595 842}]{d666-r109-var1-tile-digon-it1-r2.pdf}}
{\includegraphics*[width=20mm, viewport={0 247 595 842}]{d666-r109-var1-tile-digon-it1-r4.pdf}}
\vspace*{2mm}% V
\end{subfigure}
%
\end{center}
\caption{\label{fig:d666-r109-var1-tile-digon}
Second iterate of the digon tile \tileS{A!}{2} (left),
decomposed into 109 smaller copies of itself (first iterate)
appearing in three orientations (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d666-r109-var1-tile-plus-it1.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -m='A A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A+A!A+A+A+A!A+A+A+A+A+A!A+A+A+A!A+A+A+A+A+A-A+A!A+A-A-A+A-A+A-A+A!A+A-A+A-A+A-A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A-A+A-A+A-A+A-A+A-A+A-A ' -e=0 -k=+6 -w=5 -e=0.1 -a='(6,A+)' -i=1 -A='0.35,0' --margin=0.01 -H=L
%%
%% zrender -d=6 -m='A A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A+A!A+A+A+A!A+A+A+A+A+A!A+A+A+A!A+A+A+A+A+A-A+A!A+A-A-A+A-A+A-A+A!A+A-A+A-A+A-A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A-A+A-A+A-A+A-A+A-A+A-A ' -e=0 -k=+6 -w=3 -a='(6,A+)' -i=1 -J='A,6,0;' --margin=0.01
%%
\begin{center}
%
{\includegraphics*[width=50mm, viewport={0 270 595 822}]{d666-r109-var1-tile-plus-lines.pdf}}
\hspace*{5mm}% H
{\includegraphics*[width=50mm, viewport={0 270 595 822}]{d666-r109-var1-tile-plus-solid.pdf}}
%
\end{center}
\caption{\label{fig:d666-r109-var1-tile-plus-it1}
First iterate of the CCW prototile \tileS{A+}{6}.
Line drawing (left) and area drawing (right).
Coloring by orientation of the curves.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d666-r109-var1-tile-plus.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -m='A A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A+A!A+A+A+A!A+A+A+A+A+A!A+A+A+A!A+A+A+A+A+A-A+A!A+A-A-A+A-A+A-A+A!A+A-A+A-A+A-A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A-A+A-A+A-A+A-A+A-A+A-A ' -e=0 -k=+6 -w=3 -a='(6,A+)' -i=1 -@=1 -A -J='A,6,0;' --margin=0.01 -r=-18
%%
%%
\begin{center}
%
%{\includegraphics*[width=109mm, viewport={0 247 595 842}]{d666-r109-var1-tile-plus-decomp.pdf}}%
{\includegraphics*[width=129mm, viewport={0 280 595 805}]{d666-r109-var1-tile-plus-decomp.pdf}}%
\hspace*{0mm}% layout
%
%\begin{subfigure}[b]{20.5mm}
%{\includegraphics*[width=20mm, viewport={0 247 595 842}]{d666-r109-var1-tile-plus.pdf}}
%\vspace*{12mm}% V
%\end{subfigure}
%
\end{center}
\caption{\label{fig:d666-r109-var1-tile-plus}
Second iterate of the CCW prototile \tileS{A}{6},
decomposed into 109 smaller copies of its first iterate.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%% zrender -d=6 -m='A A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A+A!A+A+A+A!A+A+A+A+A+A!A+A+A+A!A+A+A+A+A+A-A+A!A+A-A-A+A-A+A-A+A!A+A-A+A-A+A-A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A+A+A+A!A-A+A-A+A-A+A-A+A-A+A-A ' -e=0 -k=+6 -w=3 -a='(6,A+)' -i=1 -A -J='A,6,0;' --margin=0.01

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d666-r19-it.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -m='A A+A-A+A+A!A-A+A+A!A+A+A!A+A+A+A+A+A-A ' -a='A' -t='++!!!!!!,--' -@=1 -i=3 -J='A,6,0;'
%%
\begin{center}
%
{\includegraphics*[width=90mm, viewport={0 332 595 738}]{d666-r19-it.pdf}}%
%
\end{center}
\caption{\label{fig:d666-r19-it}
Fourth iterate, coloring by orientation of edges in the motive.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d666-r19-it1.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%  zrender -d=6 -m='A A+A-A+A+A!A-A+A+A!A+A+A!A+A+A+A+A+A-A ' -e=0.1 -w=17 -a='A' -H=L -t='++!!!!!!,--' -A=0.3,0.1 -@=1 -i=0
%%
%% zrender -d=6 -m='A A+A-A+A+A!A-A+A+A!A+A+A!A+A+A+A+A+A-A ' -e=0.1 -w=7 -a=':A:' -H=L -t='++!!!!!!,--' -A=0.4,0.1 -@=1 -i=1
%%
\begin{center}
%
{\includegraphics*[width=40mm, viewport={70 247 530 782}]{d666-r19-it1.pdf}}%
\hspace*{8mm}% layout
{\includegraphics*[width=55mm, viewport={50 265 545 802}]{d666-r19-it2.pdf}}%
%
%
\end{center}
\caption{\label{fig:d666-r19-it1}
First (left) and second (right) iterates of the curve.
Starts and ends are marked.
Coloring by orientation of the edges in the motif.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d666-r25-var1-digon-solid.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -m='A A+A+A!A+A+A+A+A+A-A+A!A+A+A!A+A+A+A+A!A-A-A+A+A-A ' -e=0.1 -w=10 -a='(2,A!)' -k=+2 -i=1 -A=0.2 --margin=0.03 -J='*6,0' -r=60
%%
%% zrender -d=6 -m='A A+A+A!A+A+A+A+A+A-A+A!A+A+A!A+A+A+A+A!A-A-A+A+A-A ' -e=0.1 -w=10 -a='(2,A!)' -k=+2 -i=3 -A=0.2 --margin=0.03 -J='*6,0' -r=-60
%%
\begin{center}
%
{\includegraphics*[width=55mm, viewport={0 360 595 717}]{d666-r25-var1-digon-solid-it1.pdf}}%
\hspace*{5mm}% layout
{\includegraphics*[width=55mm, viewport={0 360 595 717}]{d666-r25-var1-digon-solid-it.pdf}}%
%
\end{center}
\caption{\label{fig:d666-r25-var1-digon-solid}
%
Area drawings of the
first (left) and third (right)
iterate of the digon tile \tileS{A!}{2}.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d666-r25-var1-outline.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%% zrender -d=6 -m='A A+A-A+A+A+A+A-A-A-A-A+A-A ' -e=0 -w=10 -a='(6,A+)' -k=+6 -i=1 -A=0.33 -H=L --margin=0.03
%%
%% zrender -d=6 -m='A A+A+A!A+A+A+A+A+A-A+A!A+A+A!A+A+A+A+A!A-A-A+A+A-A ' -e=0.1 -w=10 -a='(6,A+)' -k=+6 -i=1 -A=0.33,0.1 -H=L --margin=0.03
%%
\begin{center}
%
{\includegraphics*[width=50mm, viewport={0 267 595 822}]{d666-r25-var1-outline.pdf}}%
\hspace*{5mm}% layout
{\includegraphics*[width=50mm, viewport={0 267 595 822}]{d666-r25-var1-outline-filled.pdf}}%
%
\end{center}
\caption{\label{fig:d666-r25-var1-outline}
Border of the CCW tile \tileS{A+}{6} (left)
and tile filled with a curve of order 25 (right).
First iterates, coloring by orientation of the curves.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/d666-r25-var1-tile-solid.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%% zrender -d=6 -m='A A+A+A!A+A+A+A+A+A-A+A!A+A+A!A+A+A+A+A!A-A-A+A+A-A ' -e=0.1 -w=10 -a='(6,A+)' -k=+6 -i=1 -A=0.2 --margin=0.03 -J='*6,0'
%%
%% zrender -d=6 -m='A A+A+A!A+A+A+A+A+A-A+A!A+A+A!A+A+A+A+A!A-A-A+A+A-A ' -e=0.1 -w=10 -a='(6,A+)' -k=+6 -i=3 -A=0.2 --margin=0.03 -J='*6,0' -r=-60
%%
\begin{center}
%
{\includegraphics*[width=55mm, viewport={0 247 595 827}]{d666-r25-var1-tile-solid-it1.pdf}}%
\hspace*{5mm}% layout
{\includegraphics*[width=55mm, viewport={0 247 595 827}]{d666-r25-var1-tile-solid-it.pdf}}%
%
\end{center}
\caption{\label{fig:d666-r25-var1-tile-solid}
Area drawings of the first (left)
and third (right) iterate of the tile \tileS{A+}{6}.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/dekking-2-omg.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=4 -T='A+B,A-D,B-A,B+C,C-B,C+D,D+A,D-C' -m='A A+B-A  B B-A+B-A+B-A+B-A+B  C C+D-C+D-C+D-C+D-C  D D-C+D  ' -a='A+B+C+D' --comment=' id = 49   #simple' -l  -w=15 -e=0.15 -@=0 -i=1 -L=0.5 -A=0.3,0.1 -r=-45
%%
\begin{center}
%
{\includegraphics*[width=64.5mm, viewport={0 487 595 600}]{dekking-2-omg-it1.pdf}}%
\hspace*{0mm}% layout
%
\end{center}
\caption{\label{fig:dekking-2-omg}
%
First iterate of the tile \tileS{A+B+C+D+}{1}
of a curve-set
without any constant letter
that is not plane-filling.
Coloring by curves of the first iterate.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/easy-grids-dir.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=4 -a='F' -T='F+F,F-F' -w=10 --const-maps --grid=12,12 -r=A --zoom=1.4 --shift-y=-0.02 -A=0.2,0.12
%% zrender -d=3 -a='F' -T='F+F,F-F' -w=10 --const-maps --grid=12,12 -r=A --zoom=1.8 --shift-y=-0.02 -A=0.2,0.15
%% zrender -d=6 -a='F' -T='F+F,F--F' -w=10 --const-maps --grid=15,15 -r=A --zoom=1.4 --shift-y=-0.02 -A=0.2,0.15
%% zrender -d=12 -a='A' -T='A++A,A---B,B---A,B++++B' -w=10 --const-maps --grid=15,15 -r=A --zoom=1.4 --shift-y=-0.02 -A=0.2,0.15
%%
%%% hexagon grid:
%%% zrender -d=6 -a='F' -T='F+F,F-F' -w=10 --const-maps --grid=15,15 -r=A --zoom=1.4 --shift-y=-0.02
%%
\begin{center}
%
\fbox{\includegraphics*[width=30mm, viewport={250 500 595 842}]{easy-grids-dir-4444.pdf}}%
\hspace*{2mm}% layout
\fbox{\includegraphics*[width=30mm, viewport={250 500 595 842}]{easy-grids-dir-333333.pdf}}%
\hspace*{2mm}% layout
\fbox{\includegraphics*[width=30mm, viewport={250 500 595 842}]{easy-grids-dir-3636.pdf}}%
\hspace*{2mm}% layout
\fbox{\includegraphics*[width=30mm, viewport={250 500 595 842}]{easy-grids-dir-3464.pdf}}%
%
\end{center}
\caption{\label{fig:easy-grids-dir}
%
Directed grids,
from left to right:
square grid $(4^4)$,
triangle grid $(3^6)$,
trihexagonal grid $(3.6.3.6)$, and
the $(3.4.6.4)$-grid.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/easy-grids.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=4 -a='F' -T='F+F,F-F' -w=10 --const-maps --grid=12,12 -r=A --zoom=1.4 --shift-y=-0.02
%% zrender -d=3 -a='F' -T='F+F,F-F' -w=10 --const-maps --grid=12,12 -r=A --zoom=1.4 --shift-y=-0.02
%% zrender -d=6 -a='F' -T='F+F,F--F' -w=10 --const-maps --grid=15,15 -r=A --zoom=1.4 --shift-y=-0.02
%% zrender -d=12 -a='A' -T='A++A,A---B,B---A,B++++B' -w=10 --const-maps --grid=15,15 -r=A --zoom=1.4 --shift-y=-0.02
%%
%%% hexagon grid:
%%% zrender -d=6 -a='F' -T='F+F,F-F' -w=10 --const-maps --grid=15,15 -r=A --zoom=1.4 --shift-y=-0.02
%%
\begin{center}
%
\fbox{\includegraphics*[width=30mm, viewport={250 500 595 842}]{easy-grids-4444.pdf}}%
\hspace*{2mm}% layout
\fbox{\includegraphics*[width=30mm, viewport={250 500 595 842}]{easy-grids-333333.pdf}}%
\hspace*{2mm}% layout
\fbox{\includegraphics*[width=30mm, viewport={250 500 595 842}]{easy-grids-3636.pdf}}%
\hspace*{2mm}% layout
\fbox{\includegraphics*[width=30mm, viewport={250 500 595 842}]{easy-grids-3464.pdf}}%
%
\end{center}
\caption{\label{fig:easy-grids}
%
Tessellations of the plane with their vertex configurations,
from left to right:
square tiling $(4^4)$,
triangle tiling $(3^6)$,
trihexagonal tiling $(3.6.3.6)$, and
the tiling $(3.4.6.4)$.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/folding-r09-it1.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%% zrender -m='L L+R+L-R+L+R-L+R-L R R+L-R+L-R-L+R-L-R' -d=4 -e=0.1 -L=0.4 -A -l=',L,R' -@=1 -r=A -i=0 -w=15 -a='L'
%% zrender -m='L L+R+L-R+L+R-L+R-L R R+L-R+L-R-L+R-L-R' -d=4 -e=0.1 -L=0.4 -A -l=',L,R' -@=1 -r=A -i=0 -w=15 -a='R'
%%
\begin{center}
%
{\includegraphics*[width=37mm, viewport={0 310 595 760}]{folding-r09-it1-L.pdf}}%
\hspace*{10mm}% layout
{\includegraphics*[width=37mm, viewport={0 310 595 760}]{folding-r09-it1-R.pdf}}%
%
\end{center}
\caption{\label{fig:folding-r09-it1}
%
First iterates of a folding curve of order 9,
curve for \texttt{L} (left) and curve for \texttt{R} (right).
Note that either is the reversal of the other.
Coloring by letters.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/folding-r09-lattice-tile.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -m='L L+R+L-R+L+R-L+R-L R R+L-R+L-R-L+R-L-R' -d=4 -e=0.1 -A -r=A -a='(2,L+R+)' -J -i=4 --colors-pick=1,4 -@=0 -i=4 -t='+,-'
%% zrender -m='L L+R+L-R+L+R-L+R-L R R+L-R+L-R-L+R-L-R' -d=4 -e=0.1 -A -r=A -a='(2,L+R+)' -J -i=4 --colors-pick=1,4 -@=1 -i=4 -t='+,-'
%%
\begin{center}
%
{\includegraphics*[width=64.5mm, viewport={0 247 595 842}]{folding-r09-lattice-tile-left.pdf}}%
{\includegraphics*[width=64.5mm, viewport={0 247 595 842}]{folding-r09-lattice-tile-right.pdf}}%
%
\end{center}
\caption{\label{fig:folding-r09-lattice-tile}
%
The tile \tileS{L+R+}{2}, colored by orientation of the curves contained (left).
It can be decomposed into 9 small copies of itself of the same orientation,
it is a lattice tile (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/folding-r09-non-filling.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -i=3 -m='L L-R+L+R-L  R R+L-R-L+R' -d=4 -e=0 -A -k=-1 -L -@=0 -r=A -i=1 -w=15 -a='(2,L+R+)'
%% zrender -i=3 -m='L L-R+L+R-L  R R+L-R-L+R' -d=4 -e=0 -k=-1 -@=0 -r=A -i=3 -w=8 -a='(2,L+R+)'
%%
\begin{center}
%
{\includegraphics*[width=64.5mm, viewport={0 247 595 842}]{folding-r09-non-filling-it1.pdf}}%
\hspace*{0mm}% layout
{\includegraphics*[width=64.5mm, viewport={0 247 595 842}]{folding-r09-non-filling-it3.pdf}}%
%
\end{center}
\caption{\label{fig:folding-r09-non-filling}
%
First (left) and third (right) iterates of the tile \tileS{L+R+}{2} for
a folding curve that is self-avoiding but not plane-filling.
Note the two squares inside the first iterate that are not traversed.
Coloring by curves of the first iterate.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/folding-r09-plane-filling.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -i=3 -m='L L+R-L-R-L+R+L+R-L  R R+L-R-L-R+L+R+L-R' -d=4 -e=0.1 -A -k=-1 -L -@=0 -r=A -i=1 -w=15 -a='(2,L+R+)'
%% zrender -i=3 -m='L L+R-L-R-L+R+L+R-L  R R+L-R-L-R+L+R+L-R' -d=4 -e=0.2 -k=-1 -@=0 -r=A -i=3 -w=4 -a='(2,L+R+)'
%%
\begin{center}
%
{\includegraphics*[width=64.5mm, viewport={0 247 595 842}]{folding-r09-plane-filling-it1.pdf}}%
\hspace*{0mm}% layout
{\includegraphics*[width=64.5mm, viewport={0 247 595 842}]{folding-r09-plane-filling-it3.pdf}}%
%
\end{center}
\caption{\label{fig:folding-r09-plane-filling}
%
First (left) and third (right) iterates of the tile \tileS{L+R+}{2} for
a folding curve that is self-avoiding and plane-filling.
Coloring by curves of the first iterate.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/folding-r09-shapes.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%% zrender -i=3 -m='L L+R+L-R+L+R-L+R-L R R+L-R+L-R-L+R-L-R' -d=4 -e=0.1 -A -k=-1 -@=1 -r=A -i=4 -w=15 -a='L' -J
%% zrender -i=3 -m='L L+R+L-R+L+R-L+R-L R R+L-R+L-R-L+R-L-R' -d=4 -e=0.1 -A -k=-1 -@=1 -r=A -i=4 -w=15 -a='(2,L+R+)' -J
%%
\begin{center}
%
{\includegraphics*[width=64.5mm, viewport={0 247 595 842}]{folding-r09-shapes-curves.pdf}}%
\hspace*{0mm}% layout
{\includegraphics*[width=64.5mm, viewport={0 247 595 842}]{folding-r09-shapes-tiles.pdf}}%
%
\end{center}
\caption{\label{fig:folding-r09-shapes}
%
Left: shape of either curve (\texttt{L} or \texttt{R}),
right: shape of either tile (\tileS{L+R+}{2} or \tileS{L-R-}{2}).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/folding-r09-tile-numsys.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -m='L L+R+L-R+L+R-L+R-L R R+L-R+L-R-L+R-L-R' -d=4 -e=0.1 -L=0.4 -A=0.2,0.1 -@=1 -i=0 -w=15 -a='(2,L+R+)' --colors-pick=1,1
%%
%% zrender -m='L L+R+L-R+L+R-L+R-L R R+L-R+L-R-L+R-L-R' -d=4 -a='(2,L+R+)' -J -i=4 --colors-pick=1,1 -i=5
%%
%%
\begin{center}
%
{\includegraphics*[width=35mm, viewport={100 247 495 822}]{folding-r09-tile-numsys-tile-it1.pdf}}%
\hspace*{3mm}% layout
{\includegraphics*[width=35mm, viewport={100 247 495 822}]{folding-r09-tile-numsys-tile.pdf}}%
\hspace*{3mm}% layout
\fbox{\includegraphics*[width=35mm, viewport={150 0 850 1007}]{folding-r09-tile-numsys.png}}%
%
%
%
\end{center}
\caption{\label{fig:folding-r09-tile-numsys}
%
First (left) and fifth (middle) iterate of the CCW tile
and the fundamental region of the
corresponding numeration system (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/grid-colorings-1.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=4 -a='A' -T='A+A,A-B,B+B,B-A,' --grid=10.0,10.0 --const-maps --comment='ct=2, c=2' -L=0.4 -l -w=10 -A=0.2,0.1 -i=0 --text-start-y=0.8 --font-size=18 --no-text --add-text='ct=2  col=2  tv=[2, 2]   patch: 2 x 2' --add-text='T+: (A)^4 (B)^4' --add-text='T-: (AB)^2' --colors-pick='1,2'
%%
%% zrender -d=4 -a='A' -T='A+B,A-B,B+A,B-A,' --grid=10.0,10.0 --const-maps --comment='ct=3, c=2' -L=0.4 -l -w=10 -A=0.2,0.1 -i=0 --text-start-y=0.8 --font-size=18 --no-text --add-text='ct=3  col=2  tv=[1, 1]   patch: 2 x 2' --add-text='T+: (AB)^2' --add-text='T-: (AB)^2'  --colors-pick=1,2
%%
\begin{center}
%
%\fbox{\includegraphics*[width=40mm, viewport={70 447 525 772}, page=1]{zout-2x2-uniq.pdf}}%
%\hspace*{2mm}% layout
%\fbox{\includegraphics*[width=60mm, viewport={70 467 525 772}, page=2]{zout-2x2-uniq.pdf}}%
\fbox{\includegraphics*[width=60mm, viewport={70 467 525 772}]{grid-colorings-2A.pdf}}%
\hspace*{7mm}% layout
%\fbox{\includegraphics*[width=60mm, viewport={70 467 525 772}, page=3]{zout-2x2-uniq.pdf}}%
\fbox{\includegraphics*[width=60mm, viewport={70 467 525 772}]{grid-colorings-2B.pdf}}%
%

%
\end{center}
\caption{\label{fig:grid-colorings-1}
%
The two colorings using two colors:
$\vec{s}=[2,\,2]$ (left) and
$\vec{s}=[1,\,1]$ (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/grid-colorings-2.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%%
%%
\begin{center}
%
\fbox{\includegraphics*[width=60mm, viewport={70 467 525 772}, page=4]{zout-2x2-uniq.pdf}}%
\hspace*{7mm}% layout
\fbox{\includegraphics*[width=60mm, viewport={70 467 525 772}, page=5]{zout-2x2-uniq.pdf}}%
%

%
\end{center}
\caption{\label{fig:grid-colorings-2}
%
Two colorings using four colors:
$\vec{s}=[2,\,2]$ (left) and
$\vec{s}=[2,\,1]$ (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/grid-colorings-3.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%%
%%
\begin{center}
%
\fbox{\includegraphics*[width=60mm, viewport={70 467 525 772}, page=6]{zout-2x2-uniq.pdf}}%
\hspace*{7mm}% layout
\fbox{\includegraphics*[width=60mm, viewport={70 467 525 772}, page=7]{zout-2x2-uniq.pdf}}%
%

%
\end{center}
\caption{\label{fig:grid-colorings-3}
%
Two colorings using four colors:
$\vec{s}=[2,\,2]$ (left) and
$\vec{s}=[1,\,1]$ (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/grid-colorings-4.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%%
%%
\begin{center}
%
\fbox{\includegraphics*[width=60mm, viewport={70 467 525 772}, page=8]{zout-2x2-uniq.pdf}}%
\hspace*{7mm}% layout
\fbox{\includegraphics*[width=60mm, viewport={70 467 525 772}, page=1]{zout-5-colors.pdf}}%
%

%
\end{center}
\caption{\label{fig:grid-colorings-4}
%
A coloring using four colors with $\vec{s}=[2,\,2]$ (left)
and the unique coloring using five colors with $\vec{s}=[5,\,5]$ (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/hexagon-grid.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=6 -a='F' -T='F+F,F-F' -w=10 --const-maps --grid=15,15 -r=A --zoom=1.4 --shift-y=-0.02
%%
\begin{center}
%
\fbox{\includegraphics*[width=50mm, viewport={150 550 595 837}]{hexagon-grid-4444.pdf}}%
\hspace*{2mm}% layout
%
\end{center}
\caption{\label{fig:hexagon-grid}
%
The tiling of the plane with hexagons.
The vertex configuration is $(6^3)$,
three edges are incident to each point.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/nofit-manta-triangle-tiles.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=3 -m='F F+F-F-F0F+F+F-F0F  H H+F-F-F+H0H ' -w=7 -a='(3,F+)' -e=0.12 --colors-pick=0,12 -@=0 -i=4 -k=+1 -J
%% zrender -d=3 -m='F F+F-F-F0F+F+F-F0F  H H+F-F-F+H0H ' -w=7 -a='(3,H+)' -e=0.12 --colors-pick=0,12 -@=0 -i=4 -k=+1 -J
%%
\begin{center}
%
{\includegraphics*[width=60mm, viewport={20 257 575 820}]{nofit-manta-triangle-tiles-FFF.pdf}}%
{\includegraphics*[width=60mm, viewport={20 257 575 820}]{nofit-manta-triangle-tiles-HHH.pdf}}%
\hspace*{0mm}% layout
%
\end{center}
\caption{\label{fig:nofit-manta-triangle-tiles}
%
Fourth iterates of the tiles \tileS{F+}{3} (left)
and \tileS{H+}{3} (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/nofit-manta-triangle.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=3 -m='F F+F-F-F0F+F+F-F0F  H H+F-F-F+H0H ' -w=15 -a='(1,F+)' -k=-1 -L=0.4 -A=0.2,0.1 -e=0.1 --colors-pick=1,12 -i=1
%% zrender -d=3 -m='F F+F-F-F0F+F+F-F0F  H H+F-F-F+H0H ' -w=15 -a='(1,H+)' -k=-1 -L=0.4 -A=0.2,0.1 -e=0.1 --colors-pick=1,12 -@=1 -i=0 -l
%%
%% zrender -d=3 -m='F F+F-F-F0F+F+F-F0F  H H+F-F-F+H0H ' -w=10 -a='(1,F+)' -A=0.2,0.1 -e=0.12 --colors-pick=1,12 -@=2 -i=0 -l
%% zrender -d=3 -m='F F+F-F-F0F+F+F-F0F  H H+F-F-F+H0H ' -w=10 -a='(1,H+)' -A=0.2,0.1 -e=0.12 --colors-pick=1,12 -@=2 -i=0 -l
%%
\begin{center}
%
\begin{subfigure}[b]{31mm}
{\includegraphics*[width=30mm, viewport={90 397 500 692}]{nofit-manta-triangle-F.pdf}}
{\includegraphics*[width=30mm, viewport={90 397 500 692}]{nofit-manta-triangle-H.pdf}}%
\end{subfigure}
\hspace*{0mm}% layout
%
{\includegraphics*[width=40mm, viewport={40 247 550 842}]{nofit-manta-triangle-F-it.pdf}}
{\includegraphics*[width=40mm, viewport={40 247 550 842}]{nofit-manta-triangle-H-it.pdf}}
%
\end{center}
\caption{\label{fig:nofit-manta-triangle}
%
Motif for \texttt{F} (top left)
and \texttt{H} (bottom left).
Second iterate for \texttt{F} (middle) and \texttt{H} (right).
Edges \texttt{F} are blue and edges \texttt{H} are red.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/nofit-r07-ex00-F.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=3 -m='F F+F-F-G+F+F-F  G G+G-G-G+G+G-G' -a=F -e=0.12 -@=1 -i=0 -w=20 -l=,F,G -L=0.4 -A
%% zrender -d=3 -m='F F+F-F-G+F+F-F  G G+G-G-G+G+G-G' -a=F -e=0.12 -@=2 -i=0 -w=15 -l=,F,G -L=0.4 -A
%% zrender -d=3 -m='F F+F-F-G+F+F-F  G G+G-G-G+G+G-G' -a=F -e=0.1 -@=5 -i=0 -w=5 -l=,F,G -J -r=-80
%%
%%
\begin{center}
%
\begin{subfigure}[b]{30mm}
{\includegraphics*[width=30mm, viewport={50 357 545 662}]{nofit-r07-ex00-F-it1.pdf}}
{\includegraphics*[width=30mm, viewport={70 340 530 742}]{nofit-r07-ex00-F-it2.pdf}}
\end{subfigure}
\hspace*{0mm}% layout
%
{\includegraphics*[width=90mm, viewport={25 370 570 695}]{nofit-r07-ex00-F-it.pdf}}%
%
%
\end{center}
\caption{\label{fig:nofit-r07-ex00-F}
%
First (top left), second (bottom left),
and fifth (right) iterate of curve~\texttt{F}.
Coloring by individual edges,
blue for \texttt{F} and red for \texttt{G}.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/nofit-r07-ex00-shape.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=3 -m='F F+F-F-F+F+F-F' -a=F -A -w=20 -e=0.1 -i=0 -@=1 -k=+1
%% zrender -d=3 -m='F F+F-F-F+F+F-F' -a=F -A -w=20 -e=0.1 -i=4 -@=1 -k=+1 -J -r=-80
%%
\begin{center}
%
{\includegraphics*[width=35mm, viewport={90 347 505 630}]{nofit-r07-ex00-shape-motif.pdf}}%
\hspace*{5mm}% layout
{\includegraphics*[width=65mm, viewport={20 347 595 700}]{nofit-r07-ex00-shape-it5.pdf}}%
%
\end{center}
\caption{\label{fig:nofit-r07-ex00-shape}
%
Motif (left) and self-similarity (right) of a curve of order 7.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/nofit-r07-ex01-F.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=3 -m='F F0F+F+G-F-F0F  G G+G-G-G+G+G-G' -a=F -e=0.12 -@=1 -i=0 -w=20 -l=,F,G -L=0.4 -A
%% zrender -d=3 -m='F F0F+F+G-F-F0F  G G+G-G-G+G+G-G' -a=F -e=0.3 -@=2 -i=0 -w=15 -l=,F,G -L=0.4 -A
%% zrender -d=3 -m='F F0F+F+G-F-F0F  G G+G-G-G+G+G-G' -a=F -e=0.3 -@=4 -i=0 -w=5 -l=,F,G -r=-66
%%
%%
\begin{center}
%
\begin{subfigure}[b]{30mm}
{\includegraphics*[width=30mm, viewport={50 357 545 662}]{nofit-r07-ex01-F-it1.pdf}}
{\includegraphics*[width=30mm, viewport={70 340 530 742}]{nofit-r07-ex01-F-it2.pdf}}
\end{subfigure}
\hspace*{0mm}% layout
%
{\includegraphics*[width=90mm, viewport={25 370 570 700}]{nofit-r07-ex01-F-it.pdf}}%
%
%
\end{center}
\caption{\label{fig:nofit-r07-ex01-F}
%
First (top left), second (bottom left, rounded turns),
and fourth (right) iterate of curve~\texttt{F}.
There is always a nonzero turn between successive edges \texttt{G} (red)
but not always for \texttt{F} (blue).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/r5-dragon.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -d=4 -m='F F+F+F-F-F' -a='F' -k=-1 -i=1 -w=20 -A -e=0.05 -r=-90
%%
%% zrender -d=4 -m='F F+F+F-F-F' -a='F' -k=-1 -i=6 -J -r=-50
%%
\begin{center}
%
{\includegraphics*[width=40mm, viewport={0 350 595 720}]{r5-dragon-it1.pdf}}%
\hspace*{5mm}% layout
{\includegraphics*[width=50mm, viewport={0 350 595 720}]{r5-dragon-it.pdf}}%
%
\end{center}
\caption{\label{fig:r5-dragon}
%
First (left) and sixth (right) iterate of a curve of order 5
on the square grid without double edges.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/r7-x3-set-numsys.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -T='A0A,B0B,C0C, A+B,B+C,C+A, A-C,B-A,C-B' -d=3 -m='A ABABCBCBABA  B BCCCB  C CAAAC' -e=0 -w=3 -a='A+B+C' -@=1 --colors-pick=1,3 -t='0,-' -i=4 -J -r=-18
%%
%% other tile (is same shape, rotated by 180 degrees):
%% zrender -T='A0A,B0B,C0C, A+B,B+C,C+A, A-C,B-A,C-B' -d=3 -m='A ABABCBCBABA  B BCCCB  C CAAAC' -e=0 -w=3 -a='A-C-B-' -@=1 --colors-pick=1,3 -t='0,+' -i=4 -J -r=-18
\begin{center}
%
{\includegraphics*[width=64.5mm, viewport={0 247 595 822}]{r7-x3-set-numsys.pdf}}%
\hspace*{1mm}% layout
{\includegraphics*[width=61.5mm, viewport={0 0 1000 1007}]{r7-x3-set-numsys.png}}%
%
\end{center}
\caption{\label{fig:r7-x3-set-numsys}
%
Self-similarity of the prototile \tileS{A+B+C+}{1} (left)
and fundamental region of the corresponding numeration system (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/r7-x3-set-tile.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%% zrender -T='A0A,B0B,C0C, A+B,B+C,C+A, A-C,B-A,C-B' -d=3 -m='A ABABCBCBABA  B BCCCB  C CAAAC' -e=0.15 -w=20 -a='A+B+C' --colors-pick=1,3 -k=-1 -@=0 -i=1 -L -A -r=-60
%% zrender -T='A0A,B0B,C0C, A+B,B+C,C+A, A-C,B-A,C-B' -d=3 -m='A ABABCBCBABA  B BCCCB  C CAAAC' -e=0.15 -w=20 -a='A+B+C' --colors-pick=1,3 -t='0,-' -@=1 -i=0 -L -A -r=-60
%%% zrender -T='A0A,B0B,C0C, A+B,B+C,C+A, A-C,B-A,C-B' -d=3 -m='A ABABCBCBABA  B BCCCB  C CAAAC' -e=0.15 -w=20 -a='A+B+C' --colors-pick=1,3 -t='0,-' -@=1 -i=0 -L -A -J -r=-60
%%
%%
\begin{center}
%
{\includegraphics*[width=40mm, viewport={0 280 595 842}]{r7-x3-set-tile-curve-1.pdf}}%
\hspace*{15mm}% layout
{\includegraphics*[width=40mm, viewport={0 280 595 842}]{r7-x3-set-tile-curve-2.pdf}}%
%
%
\end{center}
\caption{\label{fig:r7-x3-set-tile}
%
First iterate of the prototile \tileS{A+B+C+}{1}, colored by curves (left).
The same, colored to separate triangles (right).\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/sausage-problem.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%% zrender -d=4 -a='(2,L+R+)' -m='L L+R-L  R R' -e=0.1 -L -A -k=-1 -w=20 -@=0 -i=1 --zoom=0.7
%% zrender -d=4 -a='(2,L+R+)' -m='L L+R-L  R R' -e=0.1 -L=0.6 -A -k=-1 -w=10 -@=0 -i=3
%%
%%
\begin{center}
%
{\includegraphics*[width=50mm, viewport={0 332 595 780}]{sausage-problem-it1.pdf}}%
\hspace*{10mm}% layout
{\includegraphics*[width=50mm, viewport={0 285 595 812}]{sausage-problem-it3.pdf}}%
%
\end{center}
\caption{\label{fig:sausage-problem}
%
First (left) and third (right) iterate of the tile \tileS{L+R+}{2}
for the curve-set with maps \Lmap{L}{L+R-L} and \Lmap{R}{R}.
Coloring by the curves of the first iterate.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> figures/zout-2x3-max-cols-ed.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[h!tbp]
%%
%%
%%
%%
\begin{center}
%
%\fbox{\includegraphics*[width=64.5mm, viewport={0 247 595 842}]{zout-2x3-max-cols-ed.pdf}}%
\fbox{\includegraphics*[width=64.5mm, viewport={30 286 565 801}]{zout-2x3-max-cols-ed.pdf}}%
\hspace*{0mm}% layout
%
\end{center}
\caption{\label{fig:zout-2x3-max-cols-ed}
%
$(2,3)$-patches on the square grid,
separated by the diagonal light blue lines.
Each of the 24 edges in a patch has a
unique color and equivalent letter.\IMAGENAME%
}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Emacs:
%%% Local Variables:
%%% MyRelDir: "./figures"
%%% pdf-file: "../main"
%%% End:


==> new-double-edges.tex <==

%\FloatBarrier
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{The $(3.3.3.3.6)$-grid (TODO)}
%% file = 00lsys-d33336.txt
%
%Here we use turns by 60 degrees ($2\pi/6$).
%
%\IMAGE{d33336-grid}
%%% note flags for B are *right*
%%
%Figure~\ref{fig:d33336-grid} shows the grid where only
%the edge corresponding one letter (\texttt{B}) is a double edge.
%There are three edge classes.
%
%The area right to an edge \texttt{B}
%is assigned to it.
%%
%The CCW prototiles are
%\tileS{A+}{6},
%\tileS{C++}{3}, and
%\tileS{B!}{2}.
%The only CW prototile is \tileS{A--B--C--}{1},
%it appears in six orientations.
%
%\jjTodo{ order 12 curve }
%  name = d33336-r12
% zrender -d=6 -a='(6,A+)---B!B--C++C++C--A--B' -m='A AAABBCCABBCAAA  B BCCCABBCCCAAB  C CCABBABBC' -A -L -k=-1 -e=0.1 -T='A+A, A--B, B!B, B0A, B--C, C++C, C--A'

%\jjTodo{ Koch shaped curve ? ; nope, not again }
% zrender -d=6 -a='A+A+A+A+A+A--B!B--C++C++C--A--B' -m='A A+A--B!B--C++C--A--B!B--C--A+A+A+A B B C C++C--A--B!B--C++C++C--A--B!B--C ' --comment='# id =1 #simple' -l -k=-1 -w=3 -e=0.2 -@=0 -i=1 -A=0.2,0.1 -H=R


%\FloatBarrier
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{The $(3.3.4.3.4)$-grid (TODO)}
%
%\jjTODO{ file = 00lsys-d33434.txt ; note flags for B are right }


%\FloatBarrier
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{The $(4.6.12)$-grid (TODO)}
%%% file 00lsys-d4612.txt
%
%\IMAGE{d4612-grid}
%
%\jjTODO{ note flags for C and c are at right }
%
%There are four edge classes
%
%\jjTodo{ r31-abc-var1, see below }
%% zrender -d=12 -a='A' -m='A AcCBCcAcCBCcAcCBCBAcCBCBABAcCBCcA  B BCcAcCBCcAcCBCcAcAcCBCcAcAcCBCBABABAcABAcCBAB  C CBCcAcCBAcCBABC  c cAcABABAcCBCcAcCBCcABABCBCcABAc' -T='C!c,c!C,A+B,B+A,A--c,c--A,B---C,C---B' -e=0.2 -w=1 -i=2 -@=1 --fancy-print-maps -J -l=',A,B,C,c' -B=5

%
%\jjTODO{ transitions, prototiles }
%
%\jjTODO{ just c and C bidirectional }
%
%\IMAGE{d4612-grid-graph}
%\IMAGE{d4612-outline}
%
%Figure~\ref{fig:d4612-outline}
%\jjTODO{ 6-symm, line drawing not perfect }
%
%
%\IMAGE{d4612-lattice-tile}


%\IMAGE{d4612-lattice-tile-r31-abc-var1}
%
%\IMAGE{d4612-r31-abc-var1-tiling}
%\IMAGE{d4612-r31-abc-var1-tiling-alt}
%
%\jjTODO{ tiles-minus! }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%*{Just letter \texttt{B} non-constant}
%
%\IMAGE{d4612-lattice-tile-r13-var2-it1}
%\IMAGE{d4612-lattice-tile-r13-var2}
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%{Just letter \texttt{A} constant}
%
%\IMAGE{d4612-r13-bc-var1-tiles-plus}
%\IMAGE{d4612-lattice-tile-r13-bc-var1}
%\IMAGE{d4612-r13-bc-var1-tiling-alt}
%\IMAGE{d4612-r13-bc-var1-tiling}


%%% Emacs:
%%% Local Variables:
%%% mode: latex
%%% MyRelDir: "."
%%% TeX-master: "./main"
%%% makefile-dir: "./"
%%% frame-title-format: "CS: double-edges [attic]"
%%% End:

